Some classical formul{\ae} for curves and surfaces

The goal of this text is to present the computation by Salmon, in the second half of the XIXth century, of various numbers enumerating planes with a prescribed tangency pattern with a sufficiently general surface $S$ in $\mathbf{P}^3$ (or, equivalently, of hyperplane sections of $S$ with prescribed singularities). Emblematic among these are the number of tritangent planes, and the number of planes cutting out a curve with a tacnode.

==> formulae.tex <==
\chaptitle{Some classical formul{\ae} for curves and surfaces}
\chapauthor{Thomas Dedieu}

\setcounter{chapter}{11}
\startchap
\label{13.th-classic}

% WARNING
% redefinition of \:
\def\:{\!:\!}

\newcommand{\no}{n\textsuperscript{o}}
\newcommand{\nos}{n\textsuperscript{os}}

\newcommand{\rs}{\mathrm{s}}
\newcommand{\rc}{\mathrm{c}}

% macros specifiques pour ce texte : formule Salmon
\newcommand{\TC}{\mathrm{TC}}

\renewcommand{\He}{\mathrm{He}}
\newcommand{\Kn}{\mathrm{Kn}}

\newcommand{\II}{I\kern -.1em I}

\newcommand{\taylordisc}{\smash
{(\raisebox{-.8mm}{\textpmhg{a}}\kern -.7mm)}}
% in case one wants to go back to normal use:
% \newcommand{\taylordisc}{\eqref{taylor-discr}}

\def\Qc{{\mathcal{Q}}}
\newcommand{\AZ}[1][\Z]{A_{#1}}
\newcommand{\x}{\mathbf{x}}
\renewcommand{\a}{\mathbf{a}}
\newcommand{\balpha}{{\boldsymbol\alpha}}
\newcommand{\IZ}[1][\Z]{\mathfrak{I}_{#1}}
\newcommand{\wt}{\operatorname{weight}}
\newcommand{\conorm}[1]{\mathcal{C}_{#1}}
\newcommand{\tconorm}[1]{\tilde{\mathcal{C}}_{#1}}

%\DeclareMathOperator{\Polar}{\mathrm{D}}
\newcommand{\Polar}{\mathrm{D}}
\newcommand{\dD}{\mathrm{D}}
% \newcommand{\polar}[2]{\Polar_{#1}#2}
\newcommand{\polar}[2]{\mathrm{D} _{#1} #2}
% ATTENTION
% macros polarité redéfinies ci-dessous
% \newcommand{\polar}[2]{\mathrm{D} _{#1} #2}
\let\obspolar\polar
\renewcommand{\polar}[2]{\mathrm{D} ^{#1} #2}
  
\newcommand{\Osc}{\mathrm{Osc}}
\newcommand{\Tan}{\mathrm{Tan}}

\newcommand{\appbnd}[2]{\mathcal{B}^{#1} #2}
\newcommand{\circum}[2]{\mathcal{C}^{#1} #2}
\newcommand{\polcone}[2]{\mathcal{D}^{#1} #2}

% \let\oldflat\flat
% \def\flat#1{\vphantom{#1}^\oldflat \kern -.1em #1}

\renewcommand{\O}{\mathcal{O}}

\setdefaultenum{(i)}{}{}{}
\setdefaultitem{---}{}{}{}



% \begin{abstract}
% The goal of this text is to present the computation by Salmon,
% in the second half of the XIXth century,
% of various numbers enumerating planes with a prescribed
% tangency pattern with a sufficiently general
% surface $S$ in $\mathbf{P}^3$
% (or, equivalently, of hyperplane sections of $S$ with prescribed
% singularities).
% Emblematic among these are the number
% of tritangent planes,
% and the number
% of planes cutting out a curve with a tacnode.
% \end{abstract}

% These notes have been taken on the occasion of the seminar
% \emph{Degenerazioni e enumerazione di curve su una superficie}
% run at Roma Tor Vergata 2015--2017.

\vspace{-1em}

\startcontents[13.th-classic]
\renewcommand{\tocdataformat}[1]{\null}
\printcontents[13.th-classic]{}{1}[2]{}


\bigskip


\def\scheck#1{\smash{\check{#1}}}
%\def\scheck#1{{\check{#1}}}

% \subsection{Introduction}
% %  and description of contents}

The goal of this text is to present the computation by Salmon,
in the second half of the XIXth century
(now a little less than two-hundred years ago),
of various numbers enumerating planes with a prescribed
tangency pattern with a smooth, and sufficiently general,
surface $S$ in $\P^3$
(or, equivalently, of hyperplane sections of $S$ with prescribed
singularities).
Emblematic among these are the number $\scheck t$
of tritangent planes,
given in \ref{p:tritangent},
and the number $\scheck \beta$
of planes cutting out a curve with a tacnode,
given in \ref{p:beta-flecnodal}.

The aforementioned numbers are the degrees of various loci in the dual
projective space $\scheck \P^3$ (the points of which correspond to
planes in $\P^3$), among which the closures of the various equisingular
strata of the dual surface $\dual S$
(the points of the latter correspond to planes tangent to $S$).
The results we present feature not only the computation of these
degrees, but also the description of the intricate geometry of these
loci and their counterparts on $S$.
Among these loci, one finds the parabolic curve of $S$
(the locus of points at which the tangent plane cuts out a
cuspidal curve; it corresponds to the cuspidal double curve of
$\dual S$), the node-couple curve
(the locus of points at which the tangent plane is also tangent at
another point; it corresponds to the ordinary double curve of
$\dual S$),
and the flecnodal curve
(the locus of points $p$ at which the tangent plane cuts out a curve
with one local branch with a flex at $p$; its counterpart on $\dual S$
is not visible in terms of equisingular strata).
A fundamental aspect of this geometry is the duality relation between
$S$ and its dual, and more generally between the loci in each of them.

Salmon's arguments are specific to hypersurfaces, and based on the
manipulation of polynomials and elimination theory.
For instance, he determines relatively explicit polynomials cutting
out the node-couple and flecnodal curves on $S$ (the parabolic curve
is cut out by the Hessian determinant).
He also makes an essential use of polars,
which for hypersurfaces may be defined in terms of polynomial
calculus, as we recall in Appendix \ref{S:polarity}.
His method to compute the number $\scheck t$ of tritangent planes,
which we present in Sections \ref{s:polcone-cusps} and
\ref{s:app-dual-tritg}, is as follows.
Let $\varpi$ be a general point of $\scheck \P^3$, and consider the
intersection of $\dual S$ with its first and second polars with
respect to $\varpi$. It is supported on the locus of points
$\varkappa$ such that the line $\vect {\varpi, \varkappa}$ has
intersection multiplicity at least three with $\dual S$ at
$\varkappa$, which of course comprises the triple points of $\dual S$,
and among those the points corresponding to tritangent planes.
Then, a fine analysis of this intersection
provides a set of relations involving the enumerative numbers we are
interested in
(but not only them),
see Theorem \ref{th:cusp-edg},
and it turns out we are able to compute sufficiently many of the
quantities in these relations in some other way
(for instance, the aforementioned number $\scheck \beta$ is obtained by
intersecting the parabolic and flecnodal curves on $S$)
so that we can finally find $\scheck t$. 

We also present, still following Salmon, the computation of
enumerative numbers related to the 
already mentioned loci, but not directly to the enumeration of hyperplane
sections with prescribed singularities.
For instance, we find the number of apparent double points of the
cuspidal and ordinary double curve of $\dual S$,
namely $g_\He = \scheck h$ and $g_\Kn = \scheck k$ given in
\ref{p:H-dev-num} and \ref{p:g_Kn}, respectively.
In fact, we study (in Section \ref{S:He-Kn})
the two developable surfaces in $\P^3$ dual to the
cuspidal and ordinary double curves of $\dual S$, and compute their
numerical characters.
This involves
a fine study of the local geometry of $S$ along its
parabolic curve
(see Section \ref{s:He-dev}),
which complements the aforementioned description of
the geometry of $S$ and its duality with $\dual S$.
This also comprises an analysis analogous to that described above for
the enumeration of tritangent planes, in which one considers this time
the intersection of $\dual S$ and its first polar with respect to
$\varpi$ with another hypersurface derived from $\dual S$ and relative
to $\varpi$, such that the intersection is supported on the locus of
points $\varkappa$ such that the line
$\vect {\varpi, \varkappa}$ has intersection multiplicity
with $\dual S$ greater than
one both at $\varkappa$ and at some other point.

The last Section \ref{S:enriques}
is dedicated to relatively more recent formulas
(from the first half of the XXth century, now a little less than
one-hundred years ago),
following the presentation given by Enriques in his landmark book
\cite{enriques}.
The main novelty is that they involve new invariants from a different
nature
(Salmon's formulas are all in term of the degree $n$ of the surface
only),
such as the arithmetic genus, and are applicable to surfaces
in $\P^3$ with ordinary singularities, so that in practice they apply
to any general three-dimensional linear subsystem of a very ample
linear system on a smooth surface.
This study includes in particular proofs of the Noether formula for the
arithmetic genus of a smooth surface, and the classical postulation
formula.

Appendix \ref{ap:dev} contains a presentation of developable surfaces
in $\P^3$ in classical terms, following Edge's beautiful book
\cite{edge}. It features Plücker formulas for curves in $\P^3$, that
are necessary for the computations in Section \ref{S:He-Kn}.
Perhaps more importantly, it is the occasion to describe the duality
relations between a curve in $\P^3$ and its dual, following the guiding
thread of this text. This all has been generalized, in modern times,
to curves in a projective space of arbitrary dimension by
Piene \cite{piene-duality}, and her results are included as well.

Appendix \ref{S:asympt} proposes an application of a basic topological
formula counting singular curves in a pencil,
see \cite[Section \tref{s:pencil}]{10.th-panoramico},
to the proof of a duality statement, namely that the orthogonality
correspondence takes asymptotic tangent lines of a surface in $\P^3$
to asymptotic tangent lines of its dual.

For the two central Sections \ref{S:zero-strata}
and \ref{S:He-Kn}, I have followed rather closely
Salmon's magnificent book \cite{salmon2}, in its fifth edition of
1915
(I have not dug in earlier text of his, or prior
versions of this book).
I have done my best to add explanations and justifications
wherever I felt this was needed
(and this is a lot of places, if I may be so bold).
Yet a blind spot of the present text is that it leaves the question of
the validity of Salmon's formulas aside: they apply to a smooth
surface under suitable transversality conditions, and we make all
along the blanket assumption that a sufficiently general surface
indeed verifies the latter transversality conditions, but do not prove
it; see Paragraph \ref{p:transversality} for some references on this
question.

Salmon's formulas have been revisited in several modern texts
already, in particular by Piene \cite{piene-someformulas}, using her
theory of polars \cite{piene-polars}.
Besides, the title of this text is a nod at the title of
\cite{piene-someformulas}, itself a nod at a series of papers by
Roth. 
There is also a proof by
Ronga \cite{ronga-13}, based on the use of
multiple-point formulas: these ideas are discussed in
\cite{14.th-vainsencher}.
Witaszek's thesis \cite{witaszek} is very complete and valuable,
concentrated on the study of very general quartic surfaces.
I have done my best to quote all relevant works on the topic. While I
certainly have quoted all those that I took inspiration from, I claim
by no means to have been encyclopedic. There are undoubtly many
references missing (in particular, I have intentionally left aside
some of the older material). May their authors and, more importantly,
the interested readers forgive me.

Let me quote G.C.~Rota to conclude this introduction:
<<~Le teorie vanno e vengono ma le formule restano.~>>\footnote
{<<~The theories may come and go but the formulas remain.~>>
  Quote and translation stolen from Ottaviani's
  Five lectures on projective invariants.
}


\paragraph*{Thanks}
I am grateful to Ragni Piene for her observations on a preliminary
version of this text.


\paragraph*{General notation}
\phantomsection
\addcontentsline{toc}{subsection}{General notation}
The exponent (and sometimes the superscript) $\vee$ denotes the dual,
in the sense of vector spaces and projective spaces, or of projective
geometry (see Section \ref{s:proj-dual}).
The symbol $\perp$ denotes the orthogonal with respect to the pairing
between linear functionals and vectors as well as, most often,
the induced notion between points in two dual projective spaces
(we will usually dodge the difference between vector spaces
and projective spaces, thus trading off slight abuses for lighter
notations and, hopefully, clarity).
Thus, if $p$ is a point in $\P^N$, then $\orth p$ is the hyperplane in
the dual projective space $\check \P^N$ whose points correspond to all
hyperplanes of $\P^N$ that contain $p$; and if $H$ is a hyperplane of
$\P^N$, $\orth H$ is the corresponding point of $\check \P^N$.
For any subset $A \subset \P^N$, $\vect {A}$ denotes the span of $A$;
thus, if $p$ and $q$ are two distinct points, $\vect{p,q}$ is the line
spanned by $p$ and $q$.

For a vector space $V$, we denote by $\P(V)$ the projective space of
all vector lines of $V$.
If $W$ is a linear subspace of $V$, we use the shorthand
$\P(V)/\P(W)$ for the projective space $\P(V/W)$,
so that if $\Lambda$ is a linear subspace of some projective space
$\P^N$, 
then $\P^N/\Lambda$ denotes the corresponding quotient projective space.
We will then usually denote by $\pi_\Lambda: \P^N \dashrightarrow
\P^N/\Lambda\cong \P^m$ the projection from $\Lambda$.
We may abuse notation and denote, for any linear subspace $F$ of
$\P^N/\Lambda$, by $\pi_\Lambda^{-1}(F)$ the largest linear subspace
of $\P^N$ surjecting onto $F$.

If $p$ is a point of a scheme $X$, we denote by $\TC_pX$ the tangent
cone of $X$ at $p$; if $p$ is a smooth point of $X$, we denote by
$T_pX$ its tangent space at $p$; if moreover $X$ is seen as lying in
some projective space, then $\T_pX$ denotes its projective tangent
space at $p$.

If $X$ is a degree $n$
hypersurface in some projective space $\P^N$, we denote
by $\polar {p^k} X$ its $k$-th polar with respect to the point $p$; it
is a degree $n-k$ hypersurface.

The notation 
$O(d)$
denotes a linear combination of monomials which all have
degree at least $d$.

The letter $n$ is reserved throughout the text to the degree of a
hypersurface, with the (hopefully only) exception of Appendix
\ref{S:calculus} .




\section{Background material}
\label{S:background}

\subsection{Projective duality}
\label{s:proj-dual}

The theme of this text is the enumeration of
hyperplanes with a prescribed tangency pattern with a smooth surface
in $\P^3$.
To get started, let us recall the basics of
projective duality, that we will use repeatedly in the course of the
text. 
For a more complete introduction, see \cite[Chap.~1]{tevelev}.

\begin{definition}
Let $X$ be a variety in $\P^N$. The \emph{dual variety} of $X$ is the
Zariski closure $\dual X$ in the dual projective space $\check \P^N$
of the set of points $\varpi \in \check \P^N$ such that the hyperplane
$\orth \varpi \subset \P^N$ is tangent to $X$ at one of its smooth
points. 
\end{definition}

A central result is the following \emph{reflexivity theorem}.
For an algebraic proof, see \cite{kleiman-aarhus}
(which also features a detailed history of this result),
or \cite[Example~16.20]{harris-13}.
For a proof using symplectic geometry, see \cite[Chap.~1]{GKZ}.

\begin{theorem}
\label{t:reflexivity}
Let $X$ be a variety in $\P^N$. One has $\dual {(\dual X)} =X$. 
More precisely, let $p$ and $\varpi$ be smooth points of $X$ and
$\dual X$ respectively: The hyperplane $\orth \varpi \subset
\P^N$ is tangent to $X$ at $p$ if and only if the hyperplane $\orth p
\subset \check \P^N$ is tangent to $\dual X$ at $\varpi$.
\end{theorem}

\noindent
This may be refined in the following way.
For a proof, see \cite{katz}, or \cite[\S 14.1]{claire}.

\begin{theorem}
\label{t:sm-odp}
Suppose $X$ is smooth and its dual is a hypersurface. 
A point $\varpi \in \dual X$ is smooth if and only if the hyperplane
$\varpi \subset \P^N$ is tangent to $X$ in a unique point $p$, and 
$\orth \varpi \cap X$ has an ordinary double point at $p$.
\end{theorem}

The general philosophy is that the singularity of the dual in a point
$\varpi$ reflects the tangency scheme of the hyperplane $\orth \varpi$
with $X$.
I shall loosely refer to any result incarnating this philosophy as a
\emph{biduality statement}.
For instance, when $X$ itself is a smooth hypersurface one has the
following result, see \cite[Prop.~11.24]{dimca}.

% \bigskip
% More generally one can describe the tangent cone of the dual variety
% at any point in similar terms. For this, we refer to
% \cite[Prop.~11.24]{dimca}. 

\begin{theorem}
\label{t:dimca-tgcone}
Let $X$ be a smooth hypersurface in $\P^N$, and let
$\varpi \in \dual X$ be such that the singular locus of 
$\orth \varpi \cap X$ consists of finitely many points
$p_1,\ldots,p_r$. 
Then the tangent cone to $\dual X$ at $\varpi$ is the union of all
hyperplanes $\orth {p_1},\ldots, \orth p_r$, each counted with
multiplicity $\mu(X,\varpi,p_i)$, the Milnor number of the singularity
of $\orth \varpi \cap X$ at $p_i$.
\end{theorem}

The following result
(see \cite[Tm.~1.21]{tevelev})
says that linear projections and taking linear
sections are dual operations. 
Recall from elementary linear algebra that if
$W$ is a linear subspace of a vector space $V$, then the transpose of
the projection $V\to V/W$ canonically identifies with the injection
$\orth W \hookrightarrow \dual V$.
% $\Lambda$ is a linear subspace of $\P^N$, then the projection 
% $\P^N/\Lambda\dashrightarrow \P^N/\Lambda$
% canonically identifies with the inclusion $\orth \Lambda \subset
% \check \P^N$ 

\begin{proposition}
\label{prop:dual-sec-proj}
Let $X$ be a variety in $\P^N$, and $\Lambda$ be a general linear
subspace of codimension $m+1$ in $\P^N$. Consider the projection
from $\Lambda$, 
\[
\pi_\Lambda: \P^N \dashrightarrow \P^N/\Lambda\cong \P^m.
\]
{\setlength\parindent{0mm}
\begin{asparaenum}[\normalfont i)]
\item 
If $m>\dim(X)$ and $\restr {\pi_\Lambda} X$ is an isomorphism to
its image, then
$\dual {\pi_\Lambda(X)} = \orth \Lambda \cap \dual X$.
\item 
If $m=\dim(X)$, let $B\subset \P^m$ be the branch divisor of $\restr
{\pi_\Lambda} X$. One has $\dual B = \orth \Lambda \cap \dual X$.
\item If $m < \dim(X)$, let $\tilde X \to X$ be the blow-up of $X$ at
$\Lambda \cap X$, and $\tilde \pi_\Lambda: \tilde X \to \P^m$ be the
morphism induced by $\pi_\Lambda$.
Let $\Delta \subset \P^m$ be the discriminant of $\tilde
\pi_\Lambda$. One has $\dual \Delta = \orth \Lambda \cap \dual X$.
\end{asparaenum}}
\end{proposition}


\subsection{Projective duality for hypersurfaces
and polarity}

When $X$ is a hypersurface, much information on $\dual X$ may
be obtained by studying the defining equation of $X$ using polynomial
calculus.
We gather here a few facts relevant for us, and refer to
\cite[Chap.~1]{dolgachev} for a much more complete treatment.
A key technical tool is polarity, the main results of which are
included in Appendix~\ref{S:polarity}.

In this section, we always assume that $X$ is a hypersurface in
$\P^N$, defined by a degree $n$ homogeneous polynomial $F$ in a
system of homogeneous coordinates $(x_0:\ldots:x_N)$.

\paragraph{}
\label{p:eq-tg-hp}
Let $q=(q_0:\ldots:q_N)$ be a smooth point of $X$.
By Euler's formula, the
equation of the tangent hyperplane to $X$ at $q$ is
\begin{equation*}
\partial _0 F(q) \cdot x_0 + \cdots + \partial _N F(q) \cdot x_N
=\dD _qF(x_0,\ldots,x_N)
=\polar {(x_0,\ldots,x_N)} F (q)
=0,
\end{equation*}
in the notation of \ref{notation:polarity}.
In particular, the point $p=(x_0:\ldots:x_N)$ 
sits on $\T_qX$
if and only if
$q$ sits in the degree $n-1$ hypersurface $\polar p X$.

\paragraph{}
\label{p:appbnd-I}
Suppose for simplicity that $X$ is smooth.
It may be seen from \ref{p:eq-tg-hp} that
for all $p \in \P^N$,
the intersection $\polar p X \cap X$ is the locus of those points
$q\in X$ such that
% $q$ sits on the tangent hyperplane $\T_p X$.
the line $\vect {p,q}$ is tangent to $X$ at $q$.
Thus, $\polar p X \cap X$ is the ramification divisor of the
projection $\pi_p:X \to \P^{N-1}$.
It is called the \emph{apparent boundary} of $X$ as
seen from the point $p$;
I will denote it by $\appbnd p X$.
The cone projecting the apparent boundary from $p$ is
called the \emph{circumscribed cone};
I will denote it by $\circum pX$.
When $X$ is singular, the circumscribed cone is the closure of the set of all lines passing through $p$ and tangent
to $X$ at a smooth point; we will use this definition in Paragraph
\ref{p:polar-cones}. 

\paragraph{Gauss map and degree of the dual}
\label{p:-deg-dual-polars}
Since there is a unique tangent hyperplane at each smooth point of
$X$, there is a dominant rational map
\[
\gamma_X: X \dashrightarrow \dual X
\]
called the \emph{Gauss map}.
If $\dual X$ is a hypersurface, it follows from \ref{t:sm-odp} that
the Gauss map is birational.

It follows from \ref{p:eq-tg-hp} that the Gauss map of $X$ is the
restriction to $X$ of 
the map defined on $\P^N$ by the $N$-dimensional linear system of all
first polars of $X$,
\ie of all $\polar p X$, $p\in \P^N$.
This is a linear subsystem of $|\O_{\P^N}(n-1)|$, and it is base point
free if and only if $X$ is smooth.

This gives a way to compute the degree of the dual of
$X$, which is also called the \emph{class} of $X$. If $X$ is smooth,
one finds that the degree of $\dual X$ equals $n(n-1)^{N-1}$. If $X$ is
singular, this has to be corrected by taking into account the base
locus of the linear system of first polars, which is supported on the
singular locus of $X$.
One may prove the Plücker formula $(P_1)$ of \ref{p:classic-Pluecker}
in this way.
More generally, Teissier \cite[Appendice II]{teissier-simultanee}
has obtained a formula for the class of any hypersurface with isolated
singularities;
the reader may also consult
\cite[Section 1.2.3]{dolgachev}.
The same formula has been proved by Laumon \cite{laumon}, with a
method close in spirit to the topological method described in
\cite[Section \tref{s:pencil}]{10.th-panoramico}.
This formula has been generalized to hypersurfaces with arbitrary
singularities by Piene \cite{piene-polars}.

\paragraph{}
\label{p:hessian-flexes}
Assume that $X$ is smooth. The Hessian hypersurface $\Hess(X)$
(see Appendix \ref{app:hess})
cuts out on $X$ the locus of those points $p\in X$ 
such that the tangent section $\T_pX \cap X$ has a singularity at $p$
worse than an ordinary double point. The intersection $X \cap
\Hess(X)$ is the ramification divisor of the Gauss map $\gamma_X: X
\to \dual X$.


\bigskip
Before I close this section, let me mention that there exists a notion
of polars for varieties in a projective space that are not necessarily
hypersurfaces.
See, for instance,
\cite{piene-polars}
and
\cite{teissier-afst}.
Using these one may compute the class of varieties in projective space
other than hypersurfaces, see, \eg
\cite{piene-polars}
and
\cite{urabe-pluecker}.


\subsection{Pl{\"u}cker formulae for plane curves}
\label{s:pluecker}

As a first and fundamental application of the previous results, let us
explain the classical Pl{\"u}cker formulae for plane curves. 

\paragraph{}
Let $C \subset \P^2$ be a plane curve. It has a finite number of
bitangent lines (\ie lines tangent to $C$ in two distinct points) and
inflection points, which give rise respectively to nodes and cusp of
the dual curve $\dual C \subset \check \P^2$: this can be seen for
instance with Theorem \ref{t:dimca-tgcone}. In general there are no
lines with a larger tangent scheme with $C$, so that nodes and cusps
are the only singularities of $\dual C$.

The reflexivity theorem \ref{t:reflexivity} suggests to
look for formulae linking numerical characters of $C$ and $\dual C$ in
a symmetric fashion. In this perspective one should allow $C$ to have
nodes and cusps.


\paragraph{Pl{\"u}ckerian characters of a plane curve}
\label{p:pluecker-notation}
We consider a plane curve $C \subset \P^2$ such that both $C$ and its
dual $\dual C \subset \check \P^2$ have only ordinary double points
(nodes) and ordinary cusps as singularities. We call:
\begin{mycpctitem}
\item $n$ the degree of $C$;
\item $\check n$ the degree of $\dual C$;
\item $\beta$ the number of bitangents of $C$, which is also the
  number of nodes of $\dual C$;
\item $\iota$ the number of flexes of $C$, which is also the
  number of cusps of $\dual C$;
\item $\delta$ the number of nodes of $C$, which is also the
  number of bitangents of $\dual C$;
\item $\kappa$ the number of cusps of $C$, which is also the
  number of flexes of $\dual C$.
\end{mycpctitem}


\paragraph{Pl{\"u}cker formulae for plane curves}
\label{p:classic-Pluecker}
One has the following relations for a curve $C$ as in 
\ref{p:pluecker-notation}.
\begin{alignat*}{6}
  & (P_1)
  & \quad &
  \check n &= n(n-1) -2\delta - 3\kappa;
  & \hspace{12mm} &
  (\check P_1)
  & \quad &
  n &= \check n(\check n -1)-2\beta-3\iota;
  \\
  & (P_2)
  &&
  \iota &= 3n(n-2) -6\delta -8\kappa;
  && (\check P_2)
  &&
  \kappa &= 3\check n(\check n-2) -6\beta -8\iota,
\end{alignat*}
For a more symmetric version one may prefer to write
$\check \delta$ and $\check \kappa$ for $\beta$ and $\iota$,
respectively. 

We sketch the proof, as it is emblematic of our approach in this text,
and refer to \cite{fischer} for a detailed implementation.

One first computes the class of a plane curve with nodes and cusps,
following \ref{p:-deg-dual-polars}: this will give the two relations on
the first line by applying the computation to both $C$ and $\dual C$.
Let $p\in \P^2$ be a general point. It follows from Theorem
\ref{t:pol-sing} that the first polar $\polar p C$ passes through all
nodes and cusps of $C$, is smooth at these points, and has general
tangent line at the nodes and tangent line equal to the reduced
tangent cone of $C$ at the cusps. Hence $\polar p C$ intersects $C$
with multiplicity $\geq 2$ at the nodes and $\geq 3$ at the cusps, and
in fact these are the actual intersection multiplicities. The relation
follows. 

Then one computes the number of flexes of $C$ by considering its
intersection with its Hessian (see \ref{p:hessian-flexes}): this will
give the two relations on the second row.
Again, one has to substract the contribution of $C \cap \Hess(C)$
corresponding to the singularities of $C$ and not to actual
inflection points.
If $q$ is a node of $C$, then the Hessian curve also has an ordinary
double point at $q$, with tangent cone equal to that of $C$.
If $q$ is a cusp of $C$, then the Hessian curve has a triple point
with two local branches at $q$, 
one smooth with general tangent, and one cuspidal
with tangent cone equal to that of $C$.
It follows that $C$ intersects its Hessian with multiplicity $\geq 6$
at the nodes and $\geq 8$ at the cusps, and again these are the actual
intersection multiplicities, hence the formula.


\paragraph{Generators for the Plücker relations}
The four relations in \ref{p:classic-Pluecker} generate a codimension
three complete intersection ideal,
\ie the Plücker formulae reduce to three formulae only, with the
Koszul type relations as the only relations among them.
Indeed, the following relation holds:
\[
  P_1 + \check P_1 = \frac 1 3 (P_2 + \check P_2),
\]
so that any three among $P_1,P_2,\check P_1, \check P_2$ generate all
Plücker relations.
It is arguably an endless game to search for a preferred set of
three generators for the Plücker relations; 
the three relations below form an appealing generating set:
\begin{alignat*}{2}
  (P'_1) & &
  3n - \kappa &= 3 \check n - \iota
  \\
  (P'_2) & \qquad &
  n(n-2)+\check n(\check n-2) &= 2\delta+3\kappa +2\beta+3\iota
  \\
  (P'_3) & &
  18(\delta-\beta)
  &= (\kappa-\iota)(\kappa-\iota+6\check n-27).
\end{alignat*}
They are indeed relations as
\begin{align*}
  P'_1 &= 3P_1-P_2 = -3\check P_1+\check P_2
  \\
  P'_2 &= P_1 + \check P_1 = \frac 1 3 (P_2 + \check P_2)
  \\
  P_3' &= 3 \, \bigl[3(n+\check n)+\kappa-\iota-3\bigr] \, P_1
         - \bigl[ 3(n+\check n)+\kappa-\iota \bigr] \, P_2
         +9 \, \check P_1,
\end{align*}
and they indeed generate the Plücker relations as
\begin{equation*}
  \left(\begin{matrix}
      P_1 \\ P_2 \\ \check P_1 \\ \check P_2
    \end{matrix}\right)
  =
  \left(\begin{matrix}
      \frac{1}{6}(n+\check n)+\frac{1}{18}(\kappa-\iota)
      &\frac{1}{2}&-\frac{1}{18}\\[1mm]
      \frac{1}{2}(n+\check n) +\frac{1}{6}(\kappa-\iota)-1
      &\frac{3}{2}&-\frac{1}{6}\\[1mm]
      -\frac{1}{6}(n+\check n)-\frac{1}{18}(\kappa-\iota)
      &\frac{1}{2}&\frac{1}{18}\\[1mm]
      -\frac{1}{2}(n+\check n)-\frac{1}{6}(\kappa-\iota)+1
      &\frac{3}{2}&\frac{1}{6}\\
     \end{matrix}\right)
\left(\begin{matrix}
     P'_1 \\ P'_2 \\ P'_3
\end{matrix}\right).
\end{equation*}




\paragraph{Smooth plane curves}
\label{p:pluecker-sm-plane}
When the plane curve $C$ is smooth one has $\delta=\kappa=0$,
so one is left with four Plückerian characters and three independent
Plücker relations.
The two characters $\check n$ and $\iota$ are expressed in terms of
$n$ by the relations $P_1$ and $P_2$, and one finds in addition:
\begin{equation*}
\textstyle
  \beta = \frac 1 2
                        n (n - 2) (n - 3) (n + 3).
\end{equation*}


\paragraph{The genus formula}
The Plücker formulae usually come adjoined with the following
relation, gotten from the fact that the two curves $C$ and $\check C$,
being birational, 
have the same geometric genus. Computing their respective geometric
genera by means of the adjunction formula, one gets:
\begin{equation*}
  \tfrac 1 2 (n-1)(n-2) -\delta -\kappa
  = \tfrac 1 2 (\check n-1) (\check n-2) - \beta -\iota.
\end{equation*}
The latter relation may in fact be obtained from the Plücker
relations: it is
\[
  \tfrac 1 2 (-P_1-2\check P_1 + \check P_2)
  = -\tfrac 1 2\,\bigl[  \tfrac 1 3 (n+\check n) + \tfrac 1 9
  (\kappa-\iota) -1 \bigr]\, P'_1
  +\tfrac 1 {18}\, P'_3.
\]


\bigskip
The condition that a plane curve and its dual both have nodes and
cusps as their only singularities poses some delicate questions.
We refer to \cite{kulikov-shustin} for recent results.
Finally, let me mention \cite{kulikov-afst}, in which the author
introduces a concept of virtual numbers of nodes and cusps, which
allows him to give symmetric Plücker formulas valid for curves with
arbitrary singularities.



\section{Double curves of the dual of a surface in $\P^3$}
\label{S:basic-dual}


We now start our study of surfaces in $\P^3$. 
Here we give a first description of the dual of a smooth surface in
$\P^3$, that will be refined later.


\subsection{Local geometry of a surface in $\P^3$ and its dual}

We first take the occasion to introduce some necessary notions on the
local geometry of a surface in $\P^3$.
Let $S$ be a surface in $\P^3$.

\paragraph{Parabolic points}
A \emph{parabolic point} of $S$ is a point $p\in S$ such that
the Hessian of $S$ at $p$ vanishes (see \ref{p:hessian}).

Equivalently, the polar quadric of $S$ at $p$,
viz. $\dD_{p^2} S$, is singular, in the sense that it is either a singular
quadric indeed, or the whole $\P^3$.
If $p$ is a smooth point of $S$, then
the first (resp.\ second) possibility is equivalent to the tangent
hyperplane section 
$S \cap \T_pS$ having a double point at $p$ with tangent cone a double
line (resp. multiplicity strictly larger than $2$ at $p$).
Thus, in general, the tangent hyperplane section of $S$ at a
parabolic point $p$ will have a cusp at $p$.

If the Hessian of $S$ does not vanish identically on $S$
(this is the case if and only if the dual of $S$ is a surface, see
\ref{p:hess-dev}),
we shall call
the curve $S\cap \Hess(S)$ the \emph{parabolic curve} of $S$,
or indifferently the \emph{Hessian curve},
and denote it by $\He(S)$.


\paragraph{Asymptotic tangent lines}
\label{p:asympt-tg}
A line $\Lambda \subset \P^3$ is
an \emph{asymptotic tangent} of $S$ at the point $p \in S$ if
$\Lambda$ and $S$ have intersection multiplicity at least $3$ at $p$.

By Theorem \ref{t:polars-tglines},
the asymptotic tangent lines at $p$ are the lines contained in the
intersection $\T_pS \cap \dD_{p^2}S$ of the tangent hyperplane and the
polar quadric of $S$ at $p$
(note that  $\T_pS = \dD_pS$ and $\dD_{p^2} S$ are tangent at $p$ by
Theorem \ref{t:pol-sing}).
Thus, there are two distinct asymptotic tangent
lines at $p$ if $p$ is not a parabolic point,
and one double asymptotic tangent
lines at $p$ if $p$ is a parabolic point and the polar quadric
$\dD_{p^2}S$ is not the whole $\P^3$.
If $\dD_{p^2}S$ is the whole $\P^3$, then all lines in $\T_pS$
passing through $p$ are asymptotic tangents.

If the polar quadric $\dD_{p^2}S$ is not the whole $\P^3$, then the
sum of the asymptotic tangent lines at $p$ is the tangent cone at $p$
of the tangent hyperplane section $\T_pS \cap S$.

\smallskip
\subparagraph{Flex tangent lines}
The asymptotic tangent lines may also be called
\emph{flex tangent lines}.
Let $H \subset \P^3$ be a hyperplane containing $p \in S$.
The curve $H \cap S$ has a flex
% \footnote
% {we say that a plane curve $C$ has a \emph{flex}
%   at $p$ if there exists a line
%   $\Lambda \subset \P^2$ having intersection multiplicity at least $3$
%   with $C$ at $p$.}
at $p$ if and only if the plane $H$
contains an asymptotic tangent line of $S$ at $p$, as an elementary
local computation shows.


\smallskip
\subparagraph{A duality statement for asymptotic tangents}
\label{p:biduality-flex-tg}
For all smooth $p\in S$,
if $\Lambda \subset \P^3$ is an asymptotic tangent line of $S$ at $p$,
then the line  $\orth \Lambda \subset \check \P^3$ is an asymptotic
tangent line of $\dual S$ at $\orth [\T_pS]$.

This is proved in 
\cite[\tref{p:vanishing-2nd-polar}]{16.th+l-redres}, and in
Appendix \ref{S:asympt};
see also 
Proposition \ref{prop:invol-at-tg}.


\paragraph{Codimension one singular loci of the dual}
\label{codim1-sing}
Let $S$ be a general surface in $\P^3$.
Then its dual $\dual S$ is singular along the two curves
parametrizing, respectively, bitangent hyperplanes of $S$,
and hyperplanes tangent to $S$ at a parabolic point.

I will call the former the \emph{ordinary double curve} of
$\dual S$.
The surface $\dual S$ indeed has an ordinary double point at its
generic point by Theorem \ref{t:dimca-tgcone}.
The two local sheets of $\dual S$ along the ordinary double curve
correspond to deformations of bitangent hyperplanes preserving either
one of the two tangency points.
The \emph{node-couple curve} $\Kn(S) \subset S$ is the closure of the
locus of points $p\in S$ such that $\T_pS$ is a bitangent plane.
Thus, the Gauss map realizes $\Kn(S)$ as a double cover of the
ordinary double curve of $\dual S$.

I will call \emph{cuspidal double curve} of
$\dual S$ the image of the parabolic curve of $S$ by the Gauss map.
The surface $\dual S$ indeed has an $A_2$ double point at its
generic point, as follows from the fact that the ramification divisor
of the birational map $S \dashrightarrow \dual S$ is the parabolic
curve, see \cite[Proposition 1.2.1]{dolgachev}.

We will make throughout the text the blanket assumption that the
codimension one singular loci of the dual surface $\dual S$ amount
eaxctly to its ordinary and cuspidal double curves, to which we will
refer as the \emph{double curves} of $\dual S$.
We refer to Paragraph \ref{p:transversality} for a discussion of this
assumption. 



\subsection{Degrees of the double curves}
\label{s:double-curves}


This section is dedicated to formulae that give the degrees of the
ordinary and cuspidal double curves of the dual of a surface $S$ in
$\P^3$; the main result is Corollary \ref{c:deg-dbl-curves}.
These formulae have been given a modern proof in
\cite{iversen} (see, in particular, Section VII.1 therein).

The underlying idea is that the double curves of the dual
$\dual S$ amount to
behaviours occuring in codimension two in the linear system of
hyperplane sections of $S$,
hence these behaviours are visible in a general codimension one linear
subsystem; therefore, one should be able to find all the relevant
information after projecting $S$ from a general point.


\paragraph{Setup}
Let $S$ be a smooth, degree $n$, surface in $\P^3$. 
For all $p \in \P^3$, we let $\appbnd pS$ be the apparent boundary
of $S$ from $p$ (since $S$ is smooth, this is the curve
$S \cap \polar p {S}$), and consider
the plane curve $B_p \subset \P^2$ image of $\appbnd p S$ by the projection
$\pi_p:\P^3 \dashrightarrow \P^2$ from the point $p$;
it is the branch divisor of the projection
$\restr {\pi_p}S: S \to \P^2$.

The main result of \cite{CF}
(see also \cite{kulikov-kulikov})
asserts that for general $p$,
the curve $B_p$ has only nodes and cusps
as singularities
(see \cite{gruson-peskine} for a general result valid in all
dimensions), 
and it is irreducible.
In addition, we shall assume that the dual plane curve
$\dual {B_p}$ has only nodes and cusps as singularities as well: since
$\dual {B_p}$ is isomorphic to $\orth p \cap \dual S$, this is
equivalent to the assumption that the codimension one singular loci of
$\dual S$ are as described in \ref{codim1-sing}.



\paragraph{Pl{\"u}ckerian characters of the branch curve}
\label{p:pluecker-branch}
Let $\nu$ be the degree of the branch curve $B_p \subset \P^2$,
$\check \nu$ be its class, and $\delta$, $\kappa$, $\beta$, $\iota$ be
its other Pl{\"u}ckerian characters as in \ref{p:classic-Pluecker}.
These numbers may all be expressed as polynomials in the degree of
$S$: 
% \begin{mycpctitem}
% \setlength{\itemsep}{1mm}
% \item $\nu=n(n-1)$~;
% \item $\check \nu = n(n-1)^2$~;
% \item $\delta=\frac 1 2 n(n-1)(n-2)(n-3)$~;
% \item $\kappa=n(n-1)(n-2)$~;
% \item $\iota=4n(n-1)(n-2)$~;
% \item $\beta=\frac 1 2 n(n-1)(n-2)(n^3-n^2+n-12)$.
% \end{mycpctitem}
\begin{alignat*}{2}
  \nu &=n(n-1)
  & \qquad\qquad
  \check \nu &= n(n-1)^2
  \\
  \delta &= \tfrac 1 2 n(n-1)(n-2)(n-3)
  &
  \beta &= \tfrac 1 2 n(n-1)(n-2)(n^3-n^2+n-12)
  \\
  \kappa &= n(n-1)(n-2)
  &
  \iota &= 4n(n-1)(n-2).
\end{alignat*}


\paragraph{}
\label{p:key-and-quick}
Let me first outline a quick proof of these formulae, based on the
two facts that, on the one hand, $B_p$ is the birational
projection from $p$ of the apparent boundary $\appbnd p S$, and on the
other hand, it is the plane dual of the section of $\dual S$ by the
plane $\orth p \subset \check \P^3$.

This implies that: i) the degree and
class of $B_p$ equal the degrees of $\appbnd p S$ and $\dual S$
respectively, which gives the formulae for $\nu$ and $\check \nu$ (see
\ref{p:pluecker-branch-geom} below):
ii)
the geometric genus of $B_p$ equals that of $\appbnd p S$, which is
easy to compute since the latter is a complete intersection. We can
then derive all remaining characters using the Pl{\"u}cker formulae
for plane curves. This is carried out
in a more general context in Section \ref{s:enriques-2dim}.

\medskip
Since $B_p$ is a general hyperplane section of $\dual S$, the above
formulae give the following.

\begin{corollary}
\label{c:deg-dbl-curves}
The numbers of binodal and cuspidal curves in a general net of
hyperplane sections of $S$ are respectively
\[
\textstyle
\frac 1 2 n(n-1)(n-2)(n^3-n^2+n-12)
\quad \text{and}
\quad
4n(n-1)(n-2).
\]
These numbers are the degrees of the ordinary and cuspidal double
curves of $\dual S$ respectively.
\end{corollary}

\paragraph{}
\label{p:pluecker-branch-geom}
Let me now give a description of the Plückerian
characters in \ref{p:pluecker-branch} in terms of the tangent
hyperplanes to $S$.
It gives a way to compute these characters directly
(although for $\beta$ I don't know of an elementary way to do it),
regardless of the quick proof
given in \ref{p:key-and-quick}.

\medskip
\subparagraph{Degree of $B_p$}
The curve $B_p$ is the projection of the circumscribed curve
$\appbnd p S = S \cap \polar p S$ from the outer point $p$.
Therefore,
$\deg(B_p) = \deg(\appbnd p S) = \deg(S) \cdot \deg (\polar p S)$.

\medskip
\subparagraph{Class of $B_p$}
The curve $\dual B_p \subset \check \P^2$ is the hyperplane section of
$\dual S$ by $\orth p$.
Indeed, for all $q\in B_p$, the hyperplane
$\pi_p^{-1}(\T_qB_p)$ is tangent to $S$ at some point $q' \in \appbnd p S$
and contains $p$;
conversely, if $H \subset \P^3$ contains $p$ and is tangent to $S$ at
some point $q'$, then $q' \in \appbnd p S$ and $\pi_p(H)$ is the tangent
line to $B_p$ at $\pi_p(q')$.

\noindent
This implies that
$\deg(\dual B_p) = \deg(\dual S) = \deg(S) \cdot \deg (\polar p S)^2$.

\medskip
\subparagraph{Nodes of $B_p$} 
\label{sp:nodes-Bp}
The nodes of $B_p$ are the points of $B_p$ with two distinct preimages
in $\appbnd p S$, hence they correspond  to
unordered pairs of distinct points $q,q' \in \appbnd p S$ such that
$p,q,q'$ are aligned.
Since $\appbnd p S$ is the curve of points $q \in S$ such that the line
$\vect{p,q}$ is tangent to $S$ at $q$,
the nodes of $B_p$ correspond to
the bitangent lines to $S$ passing by $p$.
The number of such lines may be computed in a natural way using
discriminants;
this is explained in 
\cite[Section \tref{s:bitg-lines}]{16.th+l-redres}.

\medskip
\subparagraph{Flexes of $B_p$}
Since $B_p$ is the branch curve of the projection of $S$ from $p$,
it has a flex at a point $q$ if and only if
the hyperplane $\pi_p^{-1}(\T_qB_p)$ cuts out a curve
with a cuspidal singularity on $S$.


This may be seen with the following local computation.
Let $q$ be an inflection point of $B_p$, and $q' \in \appbnd p S$ be
such that $\pi_p(q')=q$.
%the double point in its pull-back to $S$.
Locally around $q'$, $S$ may be described as a double cover of a
neighbourhood of $q$ in $\P^2$, 
hence
as a hypersurface $z^2=f(x,y)$ in affine coordinates $(x,y,z)$, such
that the projection from $p$ is $(x,y,z) \mapsto (x,y)$ and
$f(x,y)=0$ is an equation of $B_q$ locally at $q$. 
Assume that the tangent line $\T_qB_p$ is $y=0$.
Then the section of $S$ by its tangent plane at $q'$ is the
hypersurface $z^2=f(x,0)$ in affine coordinates $(x,z)$, and since $q$
is a flex of $B$, $f(x,0)$ vanishes to the third order at $0$, hence
the curve  $z^2=f(x,0)$ has a cusp at the origin, as we wanted to
show. 
The converse is proved in the same fashion.

It follows that the number of flexes of $B_p$ is the number of
hyperplanes passing through $p$ and tangent to $S$ at a
parabolic point. This is the number of intersection points of
$\appbnd p S$ with the parabolic curve, \ie
$\deg(S)\cdot\deg(\polar p S)\cdot\deg(\Hess(S))$.


\medskip
\subparagraph{Cusps of $B_p$}
\label{p:cusps-Bp}
The cusps of $B_p$ correspond to the points $q \in \appbnd p S$ such that the
line $\vect{p,q}$ is tangent to $\appbnd p S$ at $q$,
see Lemma \ref{l:proj-spcurv}.
By Lemma \ref{l:proj-flex-tg} below,
this happens if and only if the line $\vect{p,q}$ is an
asymptotic tangent of $S$ at $q$.
Therefore, the number of cusps of $B_p$ is
$\deg(S) \cdot \deg (\polar p S) \cdot \deg (\polar {p^2} S)$.

\medskip
\subparagraph{Bitangents of $B_p$}
\label{r:couple-nodal}
A line $\Lambda \subset \P^2$ is bitangent to $B_p$ if and only if
the plane $\pi_p^{-1}(\Lambda) \subset \P^3$ is bitangent to $S$.
In \cite[\S 605--607]{salmon2} Salmon constructs
from the equation of $S$,
by rather elaborate elimination theory,
a polynomial which cuts out on $S$ the locus of tangency
points of all bitangent planes of $S$.
This polynomial has degree $(n-2)(n^3-n^2+n-12)$,
and from this one deduces the number of bitangent planes of $S$ that
pass through a given general point, and
therefore the number of bitangent lines of $B_p$,
see Theorem \tref{t:node-couple}
and Corollary \tref{c:node-couple}
in \cite{16.th+l-redres}.
This construction by Salmon is the main topic of
\cite{16.th+l-redres}.



\begin{lemma}
\label{l:proj-flex-tg}
Let $q \in \appbnd p S$.
The line $\vect{p,q}$ is tangent to $\appbnd p S$ at $q$ if and only if it
is an asymptotic tangent of $S$ at $q$.
\end{lemma}

This may be proved in several ways that I deem interesting.
One may first of all do it by a local computation: this is done in
\cite[Prop.~3.9]{CF},
and I will leave it as an exercise.
I shall now give two other proofs.


\begin{proof}[Proof of \ref{l:proj-flex-tg}
by polarity]
% to illustrate the power of this formalism.
%Since $q \in \appbnd p S$,
By assumption,
$q \in \polar p S$, and the line
$\vect{p,q}$ is tangent to $S$ at $q$.
Then, the line $\vect {p,q}$ is an asymptotic
tangent of $S$ at $q$ if and only if $q \in \polar {p^2} S$,
which by polar symmetry
is equivalent to $p \in \polar {q^{n-2}} S$.
On the other hand, being tangent to $S$, the line
$\vect{p,q}$ is tangent to $\appbnd p S$ at $q$ if and only if
it is tangent to $\polar p S$, which is equivalent to
$p \in \polar {q^{n-2}} (\polar p S)$
(note that $\polar p S$ is a degree $n-1$ hypersurface).
Now, $\polar {q^{n-2}} (\polar p S) = \polar p (\polar {q^{n-2}} S)$,
and the two conditions
$p \in \polar {q^{n-2}} S$
and $p \in \polar p (\polar {q^{n-2}} S)$
are equivalent by the Euler formula, see
\ref{p:polar-self-conjug}.
\end{proof}


\begin{proof}[Proof of \ref{l:proj-flex-tg}
  by duality]
We shall use the duality statement that the orthogonal of an
asymptotic tangent to $S$ at $q$ is an asymptotic tangent to $\dual S$
at $\orth [\T_qS]$,
see \ref{p:biduality-flex-tg}.

Thus, in the conditions of the lemma,
the line $\vect{p,q}$
is an asymptotic tangent of $S$ at $q$
if and only if
the line $\orth {\vect{p,q}}$
is an asymptotic tangent of $\dual S$ at $\orth [\T_qS]$.
Since the plane $\orth p$ contains the line $\orth {\vect{p,q}}$,
this is equivalent to the hyperplane section
$\orth p \cap \dual S$ having a flex along the line
$\orth {\vect{p,q}}$
at the point $\orth [\T_qS]$.
In turn, since the projection $B_p$ of $\appbnd p S$ from $p$ is dual
as a plane curve to $\orth p \cap \dual S$, this is equivalent to
$B_p$ having a cusp at the projection of $q$ from $p$,
and the latter condition is equivalent, as we have already noted, to
the line $\vect{p,q}$ being tangent to $\appbnd p S$ at $q$.
\end{proof}


Let $q \in \appbnd p S$ be a smooth point.
We have seen above that, on the one hand,
$B_p$ has a flex at $\pi_p(q)$ if and only if
$q$ is a parabolic point of $S$, and then the tangent
$\T_q(\appbnd p S)$ is the unique asymptotic tangent of $S$ at $q$,
and on the other hand,
$B_p$ has a cusp at $\pi_p(q)$ if and only if
the line $\vect {p,q}$ is the tangent $\T_q(\appbnd p S)$, and this
happens if and only if $\vect{p,q}$ is an asymptotic tangent at $q$.
With this respect, it is interesting to note the following.

\begin{lemma}
Let $q \in \appbnd p S$ be a smooth point.
The tangent line $\T_q(\appbnd p S)$
% to $\appbnd p S$ at $q$
is an asymptotic tangent of
$S$ at $q$ if and only if either $q$ is a parabolic point,
or $\vect{p,q}$ is an asymptotic tangent at $q$.
In the latter case, 
$\vect{p,q}$ is the tangent line $\T_q(\appbnd p S)$.
\end{lemma}

\begin{proof}
First note that since $q$ is a smooth point of $\appbnd p S$, the
linear spaces $\T_qS$ and $\T_q(\polar p S)$ intersect along a line.
This implies that $\T_q(\polar p S)$ has dimension $2$, and since it
equals $\polar {q^{n-2}} {\polar p S}
= \polar p {\polar {q^{n-2}} S}$,
the polar quadric of $S$ at $q$ is not the whole $\P^3$.

Assume that $q$ is parabolic.
Then $\polar {q^{n-2}} S$ is a quadric cone, smooth at $q$
by Theorem \ref{t:pol-sing},
and $S$ has a unique flex tangent line at $q$,
which is the line
$L =
\T_q (\polar {q^{n-2}} S) \cap \polar {q^{n-2}} S
= \T_q S \cap \polar {q^{n-2}} S$
spanned by $q$ and the vertex of the cone $\polar {q^{n-2}} S$.
The tangent line $\T_q(\appbnd p S)$
equals
$\T_qS \cap \T_q(\polar p S)$,
so we only need to show that the line $L$ is contained in
$\T_q(\polar p S)$.
Now, since $\T_q(\polar p S)
= \polar p {\polar {q^{n-2}} S}$, it contains the singular point of
the cone $\polar {q^{n-2}} S$, hence also the whole line $L$.

If, on the other hand, $\vect {p,q}$ is an asymptotic tangent at $q$,
then it equals $\T_q(\appbnd p S)$ by Lemma \ref{l:proj-flex-tg}
above, and we are done in this case.

Conversely, assume that the line $L = \T_q(\appbnd p S)$
is an asymptotic tangent at $q$, but $\vect{p, q}$ is not.
Thus $p$ is off $L$,
and $L$ is contained in the quadric $\polar {q^{n-2}} S$.
Then, for all $r \in L$, the tangent space $\T_r (\polar {q^{n-2}} S)$
contains $L$, but also $p$ because
$r \in L \subset \polar p ({\polar {q^{n-2}}S})$.
It follows that the plane $\vect{p,L}$ is tangent to
$\polar {q^{n-2}} S$ at all points $r\in L$,
and this implies that
$\polar {q^{n-2}} S$ is a cone, \ie
$q$ is a parabolic point of $S$.
\end{proof}



\section{Zero-dimensional strata of the dual surface}
\label{S:zero-strata}

In this section we study some zero-dimensional strata of the dual of a
general smooth surface $S$ in $\P^3$;
in particular, we compute the number of tritangent planes of $S$,
see \ref{p:tritangent}.
The general strategy is to look at the
cuspidal edges of the polar cone of $\dual S$ with respect to a
general point of $\check \P^3$; the main result in this direction is
Theorem \ref{th:cusp-edg}.
The ordinary double edges of this cone
are studied in Section \ref{S:He-Kn}.

\subsection{Local models}

In Section \ref{s:polcone-cusps}
below we shall study a batch of formulae valid for surfaces in $\P^3$
with a given class of singularities that are modeled on those of the
dual of a general enough smooth surface.
Here we describe these singularities.
A discussion about why these should be the appropriate singularities
may be found in Paragraph \ref{p:transversality}
below.


\paragraph{Swallowtails}
\label{p:swallowtail}
We define the \emph{swallowtail\/\footnote
{in french, <<~queue d'arronde~>>, one of seven elementary catastrophes
  in Thom's theory.}
singularity}
(also referred to in this text as ``point of type $\beta$'')
as the singularity at the origin of the discriminant locus in the
semi-universal deformation space of an $A_3$ curve singularity, also
known as an ordinary tacnode.

The semi-universal deformation of the tacnode
is the family of curves over the affine space $\A^3_{a,b,c}$,
of dimension $3$ and with coordinates $(a,b,c)$,
defined in $\A^2_{x,y}\times \A^3_{a,b,c}$ by the equation:
\begin{equation}
\label{eq:tacnode-deform}
y^2=x^4+ax^2+bx+c.
\end{equation}
For more details, please see \cite{02.edoardo}.
The semi-universal deformation space of the tacnode is this
$\A^3_{a,b,c}$, and the \emph{discriminant locus} therein
is the locus over which the curves in the family defined by
\eqref{eq:tacnode-deform}
For all $(a,b,c)$, the curve in $\A^2_{x,y}$ defined by
Equation \eqref{eq:tacnode-deform}
is singular if and only if the polynomial in $x$ on the
right-hand-side has a double root. Therefore
the equation of the discriminant locus is given by the classical
discriminant of a univariate degree $4$ polynomial, \ie
\begin{equation}
\label{eq:swallowtail}
\Disc(x^4+ax^2+bx+c)
= 256 c^3 - 128 a^2 c^2 + 144 a b^2 c - 27 b^4  + 16 a^4c - 4 a^3 b^2.
\end{equation}
From this equation we see that the swallowtail
singularity is a locally irreducible triple point, with tangent cone a
triple plane.

Alternatively, the discriminant locus is the image of the map
\[
  (u,v) \longmapsto (x-u)^2(x-v)(x+2u+v)
\]
(note that the absence of $x^3$ term on the right-hand-side of
\eqref{eq:tacnode-deform} is equivalent to the sum of the four roots
of the polynomial in $x$ being $0$).
It follows that the equation of the discriminant locus may
be obtained
by eliminating $u$ and $v$ from the equations
\[
\left\{
  \begin{aligned}
a &= -3u^2-2uv-v^2 \\
b &= 2u^3+4u^2v+2uv^2 \\
c &= -2u^3v-u^2v^2
  \end{aligned}
\right.
% \iff
% x^4+ax^2+bx+x = (x-u)^2(x-v)(x+2u+v)
\]
gotten by computing the coefficients of $(x-u)^2(x-v)(x+2u+v)$.

Similarly,
the locus in the semi-universal deformation space of the tacnode over
which the curves in the family defined by \eqref{eq:tacnode-deform}
have a cusp is the image of the map
$(u,v) \mapsto (x-u)^3(x+3u)$, hence its equations may be found 
by eliminating $u$ and $v$ from the equations
\[
a = -6u^2; \quad
b = 8u^3 ; \quad
c = -3u^4.
% \left\{
%   \begin{aligned}
% a &= -6u^2 \\
% b &= 8u^3 \\
% c &= -3u^4
%   \end{aligned}
% \right.
\]
This gives the ideal of equations 
\begin{equation}
(a^2+12c,
8a^3+27b^2),
\end{equation}
from which we see that the locus in consideration is an irreducible
curve with a planar ordinary cusp at the origin, the generic point of
which is a cuspidal double point of the discriminant locus.
We shall call this curve the \emph{cuspidal double curve} of the
swallowtail singularity.

In turn, the locus over which the curves
in the family defined by \eqref{eq:tacnode-deform}
have two nodes is the image of the map
$(u,v) \mapsto (x-u)^2(x+u)^2$, hence its equations may be found 
by eliminating $u$ and $v$ from the equations
\[
a = -2u^2;\quad
b = 0 ; \quad
c = u^4;
% \left\{
%   \begin{aligned}
% a &= -2u^2 \\
% b &= 0 \\
% c &= u^4
%   \end{aligned}
% \right.
\]
this gives the ideal of equations 
\begin{equation}
(b,
a^2-4c),
\end{equation}
from which we see that the locus in consideration is a smooth irreducible
curve, the generic point of
which is an ordinary double point of the discriminant locus.
We shall call this curve the \emph{ordinary double curve} of the
swallowtail singularity.

Finally,
one finds that the tangent cone of the intersection of the cuspidal
and ordinary double curves is defined by the ideal
$(b,c,a^2)$ , so these two curves intersect with multiplicity $2$.


\paragraph{Type $\gamma$ singularity}
\label{p:type-gamma}
Similarly to what we have done for the swallowtail in
\ref{p:swallowtail} above, we define
the \emph{singularity of type $\gamma$} as the singularity at the
origin of the discriminant locus in the semi-universal deformation
space of the multisingularity $(A_1,A_2)$ consisting of a node and an
ordinary cusp.

The semi-universal deformations of a node
and a cusp are respectively given by
\begin{equation}
\label{eq:type-gamma}
y^2 = x^2+a
\qquad \text{and}
\qquad
y^2 = x^3+bx+c,
\end{equation}
and we consider the disjoint union of their pull-back to the product
$\A^1_a\times \A^2_{b,c}$.
The equation of the discriminant is merely the product of the two
discriminants, \ie 
\begin{equation}
\Disc(x^2+a)\cdot \Disc(x^3+bx+c)
= a \cdot (4b^3+27c^2).
\end{equation}
At the origin, the discriminant locus has two local sheets, one smooth
and one with a cuspidal double curve, and the two meet transversely.

The locus in $\A^1_a\times \A^2_{b,c}$ above which the curve defined by
\eqref{eq:type-gamma} has a cusp
parametrizes those deformations of the multisingularity $(A_1,A_2)$
along which the node
smoothes and the cusp is maintained. Its has equations
\[
b=c=0.
\]
It is a smooth curve, which we will call 
the \emph{cuspidal double curve} of the
type $\gamma$ singularity. 

The locus in $\A^1_a\times \A^2_{b,c}$ above which the curve defined by
\eqref{eq:type-gamma} has two nodes
parametrizes those deformations of the multisingularity $(A_1,A_2)$
along which the node
is maintained and the cusp deforms to a node, which has equations
\[
a=4b^3+27c^2=0.
\]
It is a curve with a planar ordinary cusp at the origin, which we will
call 
the \emph{ordinary double curve} of the
type $\gamma$ singularity. 
It is the intersection curve of the two sheets of the discriminant
surface. 

\paragraph{Type $t$ singularity}
\label{p:type-t}
Finally, we define
the \emph{singularity of type $t$} as the singularity at the
origin of the discriminant locus in the semi-universal deformation
space of the multisingularity $(A_1,A_1,A_1)$ consisting of three nodes.

Thus we consider three copies of the semi-universal deformations of a
node, 
\begin{equation}
\label{eq:type-t}
y^2 = x^2+a
\qquad \text{and}
\qquad
y^2 = x^2+b
\qquad \text{and}
\qquad
y^2 = x^2+c,
\end{equation}
and look at the disjoint union of their pull-back to the product
$\A^1_a\times \A^1_{b} \times \A^1_c$.
The equation of the discriminant is the product of the three
discriminants, \ie 
\begin{equation}
\Disc(x^2+a)\cdot \Disc(x^2+b)\cdot \Disc(x^2+c)
= abc.
\end{equation}
The discriminant locus has three smooth local sheets meeting
transversely at the origin.

The locus in $\A^1_a\times \A^1_{b} \times \A^1_c$
above which the curve defined by
\eqref{eq:type-t} has two nodes is the union of the three coordinate
lines $\A^1_a \times \0\times \0$, $\0 \times \A^1_b \times\0$,
and $\0\times\0\times \A^1_c$;
it is defined by the ideal of equations
$(ab, ac, bc)$, and has a triple point at the origin.
Yet again, we shall call it the ordinary double curve of the type $t$
singularity. 

The locus in $\A^1_a\times \A^1_{b} \times \A^1_c$
above which the curve defined by
\eqref{eq:type-t} has a cusp
is empty.



\subsection{Polar cones and their cuspidal edges}
\label{s:polcone-cusps}

In this section we describe the cuspidal edges of the polar cone of a
surface in $\P^3$ which has the same kind of singularities as the dual
of a sufficiently general smooth surface. We shall call this class of
singularities d-ordinary singularities, since (plain) ordinary
singularities classically refer to the kind of singularities found on
a sufficiently general projection to $\P^3$ of a smooth surface in
$\P^5$ (or 
in $\P^N$ for any $N\geq 5$),
see \ref{p:setup-enr-dim3}.

The central result is Theorem \ref{th:cusp-edg}, which is the keystone
of the computation of the number of tritangent planes in the next
section. 

\paragraph{Surfaces with d-ordinary singularities}
\label{p:d-ord-sings}
We say that a surface $X \subset \P^3$ has
\emph{d-ordinary singularities} if it has 
a curve $B$ of ordinary double points,
a curve $C$ of simple cuspidal double points,
and no other singularities except from those arising from the
singularities of the curves $B$ and $C$, by which we mean:
\begin{mycpctitem}
\item $\beta$ intersection points between $B$ and $C$
at which $C$ is cuspidal (and $B$ is smooth), at which $X$ has a type $\beta$ (\ie
swallowtail) singularity 
as in \ref{p:swallowtail} above;
\item $\gamma$ intersection points between $B$ and $C$ at which $B$ is
  cuspidal (and $C$ is smooth), at which $X$ has a type $\gamma$
  singularity 
as in \ref{p:type-gamma} above;
\item $t$ the number of triples points of the ordinary double curve
  $B$, at which $X$ has a type $t$ singularity as in \ref{p:type-t}
  above. 
\end{mycpctitem}
Moreover, we let $b$ and $c$ denote the degrees of the curves $B$ and
$C$ respectively.


\bigskip
We now consider, for the rest of the present
Section \ref{s:polcone-cusps},
a surface $X \subset \P^3$ with d-ordinary singularities,
with the notation as in \ref{p:d-ord-sings}
above.

Let $p$ be a general point of $\P^3$.
It follows from a local computation, see Theorem \ref{t:pol-sing},
that the first polar $\polar p X$
contains simply the curves $B$ and $C$, with tangent cone equal to
that of $X$ at the generic point of $C$. Therefore, the intersection
$X\cap \polar p X$ contains $B$ and $C$ with multiplicities $2$ and $3$
respectively, and we need to refine the definition of apparent boundary
given in \ref{p:appbnd-I}.


\paragraph{Polar cones of a surface with d-ordinary singularities}
\label{p:polar-cones}
We let the \emph{polar cone} $\cD^pX$ of $X$ with
respect to $p$ be the cone projecting from $p$ over the
curve $X \cap \polar p X$.
It contains the two cones projecting $B$ and $C$ from $p$ with
multiplicities $2$ and $3$ respectively, and we let
the \emph{circumscribed cone} $\cC^pX$ be the cone residual to these
two cones in the polar cone;
it is the closure of the set of all lines passing through $p$ and tangent
to $X$ at a smooth point.
Finally, we denote by $\appbnd p X$ the curve 
$(X \cap \cC^pX)_\red$, which we call the \emph{apparent boundary}.

We let $a$ be the degree of $\cC^pX$. Then,
the degree of the polar cone $\cD^pX$ reads
\begin{equation}
\label{eq:deg-polar-cone}
n(n-1) = a +2b +3c.  
\end{equation}



\paragraph{Cuspidal edges of the polar cone}
\label{p:cusp-edg-polar-cone}
We now introduce more notation, and list various kinds of points that
will appear in the 
intersection $X \cap \polar p X \cap \polar {p^2} X$, together with
the singular points listed in \ref{p:d-ord-sings}.
The lines joining $p$ to the points of
$X \cap \polar p X \cap \polar {p^2} X$ are
the cuspidal edges of the polar cone $\cD^pX$, in analogy with what
happens when $X$ is smooth, see Paragraph \ref{p:cusps-Bp}.

We set:
\begin{mycpctitem}
\item $\kappa$ the number of cuspidal edges of the circumscribed cone
$\cC^p X$; 
\item $\rho$ the number of intersection points between the
  apparent boundary $\appbnd p X$ and the ordinary
  double curve $B$;
\item $\sigma$ the number of intersection points between the
  apparent boundary $\appbnd p X$
  and the cuspidal double curve $C$.
\end{mycpctitem}
We shall introduce some more notation later in
\ref{p:dble-edg-polar-cone}, but it
is not relevant for the present considerations.


\bigskip
Salmon gives the following set of formulae
\cite[\S 610]{salmon2},
which describes separately the intersections with the second polar 
$\polar {p^2} X$ of the three components of the polar cone $\cD^pX$.


\newcommand{\hieroA}[1]
{\smash{\raisebox{1.3mm}{\pmglyph{\HDiv}}
\kern -6mm \raisebox{-.6mm}{\pmglyph{\HIix}}
%\kern -1.3mm .
#1}}
\newcommand{\refCuspEdg}{({\protect\hieroA{}\kern -1.9mm)}}
\newcommand{\refCuspEdgA}{(\hieroA {\pmglyph{\HZi}})}%
\newcommand{\refCuspEdgB}{(\hieroA {\pmglyph{\HZiv}})}%
\newcommand{\refCuspEdgC}{(\hieroA {\pmglyph{\HZii}})}%
%
%
\begin{theorem}
\label{th:cusp-edg}
For $X \subset \P^3$ a surface with d-ordinary singularities and $p
\in \P^3$ a general point, and with the notation of
\ref{p:d-ord-sings} and \ref{p:cusp-edg-polar-cone}, one has:
\begin{align}
%\label{eq:A}
\tag{\hieroA {\pmglyph{\HZi}}}
a(n-2) &= \kappa + \rho +2\sigma \ ;\\
\tag{\hieroA {\pmglyph{\HZiv}}} 
b(n-2) &= \rho + 2\beta + 3\gamma +3t \ ;\\
\tag{\hieroA {\pmglyph{\HZii}}} 
c(n-2) &= 2\sigma + 4 \beta + \gamma.
\end{align}
\end{theorem}

He comments:
<<~The reader can see without difficulty that the points indicated in
these formul{\ae} are included in the intersections of
[$\polar {p^2}X$ with the three components of  $\cD^pX$];
but it is not so easy to see the reason for the numerical multipliers
which are used in the formul{\ae}. Although it is probably not
impossible to account for these constants by a priori reasoning, I
prefer to explain the method by which I was led to them
inductively.~>>
The latter method consists in considering the dual of a smooth cubic
surface, for which all the quantities may be directly computed, and
then in tuning the coefficients to make the formulae work.

The remainder of the present Section \ref{s:polcone-cusps} is dedicated
to the proof of the above theorem.
By Theorem \ref{t:polars-tglines}, the intersection
\[
  X \cap \polar p X \cap \polar {p^2} X
  = \bigl( \appbnd p X + 2B+3C \bigr)
   \cap \polar {p^2} X
\]
is supported on the locus $\mathfrak D$ of
points $q$ in $X$ such that the line $\vect {p,q}$ has intersection
multiplicity at least $3$ with $X$ at $q$.
The proof consists in the following two points.
(i) List the various kinds of points in the locus
$\mathfrak D$;
this indicates which terms (without the integer coefficients) 
appear on the right-hand-side of Formulae \refCuspEdg{};
the condition that $X$ has d-ordinary singularities leaves us with
finitely many possibilities.
(ii) For each of those, determine the corresponding
multiplicity in the intersection cycle
$X \cap \polar p X \cap \polar {p^2} X$; this will tell us the
integer coefficient with which each term on the right-hand-side of
\refCuspEdg{} appears.

The smooth points in the locus $\mathfrak D$ are the points of type
$\kappa$, see \ref{sp:cusp-edg-kappa} below.
Some special double points of $X$ lie in $\mathfrak D$, and these are
the points in the two intersections $\appbnd p X \cap B$ and $\appbnd
p X \cap C$. Finally, all triple points automatically lie in
$\mathfrak D$.
Thus the points appearing in $\mathfrak D$ are those of the types
$\kappa, \rho, \sigma, \beta, \gamma, t$.
The remainder of the proof consists in a case by case local study of
the polars of $X$ at all such points.

\medskip
\subparagraph{Type $\kappa$}
\label{sp:cusp-edg-kappa}
Cuspidal edges of $\cC^pX$ appear in correspondence with points $q \in
\appbnd p X$ such that the line $\vect {p,q}$ is tangent to
$\appbnd p X$, as has been explained in \ref{p:cusps-Bp},
and such points $q$ are simple points in the intersection
$\appbnd p X \cap \polar{p^2}X$ as in Lemma \ref{l:proj-flex-tg}.
For general $p$, these points lie on neither one of the double curves
of $X$.


\medskip
\subparagraph{Type $\rho$}
\label{sp:rho}
Points of type $\rho$ are those points $q$ lying on the ordinary
double curve $B$ such that the line $\vect {p,q}$ is
an honest tangent to one of the two smooth local sheets of $X$ at $q$;
let us call $X_q'$ this local sheet.
We claim that
(i) the first polar $\polar p X$ is smooth at $q$ with the same tangent
plane as $X_q'$, and its intersection with $X$ locally at $q$ consists
of $B$ and $\cC_pX$, the latter entirely
contained in $X_q'$,
and (ii)
the second polar $\polar {p^2} X$ is smooth at $q$ with general tangent
plane, hence it intersects both $B$ and $\cC_pX$ transversely at $q$.

Let us justify this claim by a specific local computation,
as it does not directly follow from Theorem \ref{t:pol-sing}.
We may assume that $q = (0:0:0:1)$ in a homogeneous system of coordinates
$(x:y:z:w)$, and $X$ is given locally at $q$ by the equation
\[
  f(x,y,z)= \bigl[x+g_2(x,y,z)+O(3)\bigr]
  \bigl[y+h_2(x,y,z)+O(3)\bigr] = 0
\]
in the affine chart $w=1$, where $g_2$ and $h_2$ are homogeneous
of degree $2$, and $O(3)$ denotes higher order terms.
Then we may take $p=(1:0:0:0)$, and thus $\polar p = \partial_x$.
Then,
\begin{multline*}
  \polar p f (x,y,z) =
  \bigl[x+g_2+O(3)\bigr]
  \bigl[\partial_x h_2+O(2)\bigr]
  + \bigl[1+\partial_x g_2+O(2)\bigr]
  \bigl[y+h_2+O(3)\bigr]
  \\= y + x\,\partial_x h_2
  +y\,\partial_xg_2 + h_2 + O(3)
\end{multline*}
and part (i) of the claim follows.
Finally, 
\begin{equation*}
  \polar {p^2} f (x,y,z) =
  2\,\partial_x h_2
  +x\,\partial_x^2 h_2
  +y\,\partial_x^2g_2 + O(2),
\end{equation*}
and part (ii) follows.


\medskip
\subparagraph{Type $\sigma$}
\label{p:sigma-cusp}
Points of type $\sigma$ are those points $q$ lying on the cuspidal
double curve $C$ such that the line $\vect {p,q}$ lies
in the tangent cone of the unique, cuspidal, local sheet of $X$ at $q$.
We claim that
(i) the first polar $\polar p X$ has a double point at $q$,
and the intersection of the tangent cones $\TC_qX$ and
$\TC_q(\polar p X)$ is a quadruple line supported on $\T_qC$;
moreover, (ii)
the second polar $\polar {p^2} X$ has a simple point at $q$, and
the intersection of its tangent plane with $[\TC_qX]_\red$ is the line
$\T_qC$.
By (i), since at $q$ the intersection of $\polar p X$ and $X$ is the
sum of $3C$ and $\appbnd p X$, 
the apparent boundary $\appbnd p X$ is smooth at $q$, and
tangent to the cuspidal edge $C$.
Thus, (ii) tells us that the second polar $\polar {p^2} X$ is tangent
 to both curves $C$ and $\cB^p X$ at $q$, which accounts for the
multiplicities 
$2$ of $\sigma$ in \refCuspEdgA{} and \refCuspEdgC.

As in \ref{sp:rho} above, we justify our claim by a local computation,
with similar notation.
We let
$q=(0:0:0:1)$, and consider the following equation for $X$ locally at
$q$ in the affine chart $w=1$:
\[
  f(x,y,z)= \bigl[ y+g_2(x,y,z)+O(3) \bigr]^2 +
  \bigl[ x +h_2(x,y,z) +O(3) \bigr]^3=0,
\]
where $g_2$ and $h_2$ are homogeneous of degree $2$.
We may again take $p=(1:0:0:0)$, and then
\[
  \polar p f = 2\,\partial_x g_2 \cdot y
  +3x^2 +O(3),
\qquad \text{and}
\qquad
\polar {p^2} f = 2\,\partial_x^2 g_2 \cdot y
+6x +O(2),
\]
which proves our claim.


\medskip
\subparagraph{Type $t$}
These are the points at which $X$ has three transverse smooth local
sheets.
We may directly apply Theorem~\ref{t:pol-sing}, to the effect that
at a type $t$ singular point $q$,
(i) the first polar 
$\polar p X$ has an ordinary double point at $q$,
and (ii) the second polar $\polar {p^2} X$ is smooth with general
tangent plane, hence intersects $B$ transversely at $q$.
This gives
the multiplicity $3$ for type $t$ in \refCuspEdgB{}, as $q$ is a triple
point of $B$. On the other hand, type $t$ points lie neither on
$\appbnd p X$ nor on $C$.

\medskip
\subparagraph{Type $\beta$}
\label{sp:type-beta}
These are triple points of $X$, with a local equation equivalent to
that in \eqref{eq:swallowtail}; in particular the tangent cone of $X$
at such a point is a triple plane.
Thus, it follows from Theorem~\ref{t:pol-sing} that if $q$ is a type
$\beta$ singular point, then
(i) the first polar $\polar p X$ has a double point at $q$ with tangent
cone a double plane supported on $(\TC_qX)_\red$, and
(ii) the second polar 
$\polar {p^2} X$ is smooth with tangent plane equal to
$(\TC_qX)_\red$.

The ordinary double curve $B$ is smooth at points of type $\beta$,
as we have seen in Paragraph \ref{p:swallowtail},
and the second polar is tangent to it. This accounts for the
multiplicity $2$ in \refCuspEdgA.
On the other hand, the cuspidal double curve $C$ has planar ordinary
cusps at points of type $\beta$, but it turns out that it intersects
$\polar {p^2} X$ 
with multiplicity $4$ at such points: indeed, in the notation of
\ref{p:swallowtail}, $C$ is defined by the ideal
$(a^2+12c,
8a^3+27b^2)$,
and the tangent cone of $\polar {p^2} X$ is the plane $c=0$.
This confirms the multiplicity of $\beta$
in \refCuspEdgB{}, and shows that
$(\TC_qX)_\red$ is the osculating plane of $C$ at swallowtail points
$q$. 



\medskip
\subparagraph{Type $\gamma$}
\label{sp:gamma}
These are triple points $q$ of
$X$, at which $X$ has two transverse local sheets, one smooth:
$X_q^\rs$, and the other cuspidal: $X_q^\rc$.  
The first polar $\polar p X$ has a double point at $q$, with tangent
cone the sum of $[\TC_q (X_q^\rc)]_\red$ and a general plane containing
the line $\TC_q (B)$.
The second polar $\polar {p^2} X$ is smooth at $q$, with tangent plane
a general plane containing the line $\TC_q (B)$.
Therefore it intersects $B$, which is cuspidal at $q$, with
multiplicity $3$, and it is transverse to $C$, which is smooth at
$q$. This amounts for the multiplicities $3$ and $1$ in \refCuspEdgB{}
and \refCuspEdgC{} respectively.

To clarify the situation, let us carry out the local computations
proving the above assertions. We
let $q=(0:0:0:1)$ and consider the two sheets $X_q^s$ defined
respectively by the equations
\[
z+O(2) = 0
\qquad \text{and}
\qquad
y^2+x^3+O(4) = 0.
\]
The curve $B$ is the intersection of these two sheets, it has a cusp
at $q$ with tangent cone defined by $z=y^2=0$. The curve $C$ is the
singular locus of $X_q^\rc$, it is smooth at $q$ with tangent line
defined by $y=x=0$.
We may take $p=(u_0:u_1:u_2:0)$. Then, by Theorem~\ref{t:pol-sing} the
tangent cones of $\polar p X$ and $\polar {p^2} X$ are defined
respectively by
\[
\polar p (zy^2) = y(2u_1z+u_2y)
\qquad \text{and}
\qquad
\polar {p^2} (zy^2) = 2u_1 (u_1 z +2u_2 y),
\]
which proves our claims.


\bigskip
\noindent
The proof of Theorem \ref{th:cusp-edg} is now complete.
\qed
\subsection{Application to the case when $X=S^\vee$}
% \subsection{Application to the case $X=\dual S$}
\label{s:app-dual-tritg}


%\paragraph{Description in the case $X=\dual S$}
We now let $S$ be a smooth, degree $n$, surface in $\P^3$,
and call \smash{$X = \dual S \subset \check \P^3$} its dual surface.
We shall explore in this situation
the geometric landscape described in Section \ref{s:polcone-cusps}
above.

\paragraph{}
\label{p:transversality}
We take for granted that if $S$ is general enough, then
$X$ has d-ordinary singularities
(see \ref{p:d-ord-sings}), and we assume that $S$ is indeed general
enough.

The principle behind this implication is that, since hyperplane
sections of $S$ form a $3$-dimensional system,
we expect that under suitable generality/transversality assumptions,
only (multi-)singularities imposing at most three conditions may occur
on hyperplane sections of $S$.
The condition that a given multi-singularity imposes at most three
conditions translates into the fact that its semi-universal
deformation space has dimension at most three
(for a general discussion of the expected codimension imposed by the
presence of a multi-singularity,
see \cite[Section \tref{s:ESloci}]{14.th-vainsencher}).
We expect moreover
that, still under the aforementioned generality assumptions,
for all $\orth H \in\check \P^3$, there is a submersion from an
analytic or étale neighbourhood of $\orth H$ in $\check \P^3$ to the
semi-universal deformation space of the multi-singularity of $H\cap
S$; this implies that, locally around $\orth H$, the dual $\dual S$
looks like the discriminant locus in the deformation space of the
multi-singularity of $H\cap S$.

For a proof that if $S$ is sufficiently general, then things happen
according to the above described expectations, see
\cite{bruce},
\cite{mccrory-shifrin},
and \cite{ronga-transversality}.
See also \cite{XuGeng} for a related result.


\begin{notation}
As a rule, we use the decoration with a duality symbol to indicate
that a symbol denotes a quantity associated with $X=\dual S$.
Thus, we set:
\begin{mycpctitem}
\item $\check n=
n(n-1)^2$, the degree of $X$.
\end{mycpctitem}
We use the notation introduced in Section \ref{s:polcone-cusps} for
the singularities of $X=\dual S$, with an additional ``$\vee$''
decoration. 
\end{notation}


\paragraph{}
The double curves $\check B$ and $\check C$
are the curves in $\dual S$ parametrizing the
bitangent and parabolic tangent planes to $S$, respectively.
The Gauss map of $S$ induces a
$2:1$ map $\Kn_S \to \check B$ from the node-couple curve $\Kn_S
\subset S$, and a birational map $\He_S \to \check C$ from the
Hessian curve $\He_S \subset S$.
We have seen in Corollary \ref{c:deg-dbl-curves}
%Section \ref{s:double-curves}
that the degrees of the two curves $\check B$ and $\check C$ in $\check
\P^3$ are:
\begin{mycpctitem}
\item $\check b=
\frac 1 2 n(n-1)(n-2)(n^3-n^2+n-12)$~;
%is the degree of the ordinary double curve of $\check S$;
\item $\check c=
4n(n-1)(n-2)$.
\end{mycpctitem}

\paragraph{}
\label{p:checkA}
In the context of Section \ref{s:polcone-cusps},
we need to choose a general point $\check p \in \check \P^3$
to consider the polar cone $\cD^{\check p}X$ and the apparent boundary
$\appbnd {\check p} X$.
This point $\check p$ corresponds to a hyperplane
$H_{\check p} =
\orth {\check p}$ in $\P^3$. The circumscribed cone
$\cC^{\check p} (\dual S) \subset \check \P^3$
is the dual of the plane curve
$H_{\check p} \cap S \subset \P^3$.
This gives:
\begin{mycpctitem}
\item $\check a=n(n-1)$.
\end{mycpctitem}
Note that with our values of $\check a, \check b, \check c$,
Formula \eqref{eq:deg-polar-cone}
holds indeed.

It also follows from the above description of
$\cC^{\check p} (\dual S)$ 
 that the cuspidal edges of type $\check \kappa$ of the
polar cone $\cD ^{\check p} \dual S$ are the lines
orthogonals to the osculating tangent lines of the plane curve
$H_{\check p} \cap S$ (\ie the orthogonals of the flex tangents of 
$H_{\check p} \cap S$). Thus,
\begin{mycpctitem}
\item $\check \kappa = 3n(n-2)$.
\end{mycpctitem}

\paragraph{}
The apparent boundary $\appbnd {\check p} {X}$
parametrizes points $\varpi \in X = \dual S$ such that
$\check p \in \T_\varpi X$,
\ie dually,
planes $\orth \varpi \subset \P^3$ tangent to $S$ at a
point $\orth [\T_\varpi X]$ lying on $H_{\check p}$.
It follows that the points of type $\check \rho$ (resp.\
$\check \sigma$) correspond to hyperplanes that are tangent to $S$ at
some point on $H_{\check p}$ and at some other point (resp.\ at some point on
$H _{\check p}$ which is parabolic). Thus,
$\check \rho$ (resp.\ $\check \sigma$) is the degree of the
intersection of $H _{\check p}$ with the node-couple curve $\Kn_S$
(resp.\ with the Hessian curve $\He_S$), and therefore:
\begin{mycpctitem}
\item $\check \rho = n(n-2)(n^3-n^2+n-12)$~;
\item $\check \sigma = 4n(n-2)$
\end{mycpctitem}
(for $\check \rho$, see \ref{r:couple-nodal};
$\check \sigma$ follows directly from the fact that $\He_S$ is the
complete intersection of $S$ and $\Hess(S)$).

\paragraph{}
\label{p:beta-gamma-t}
Points of type $\check \gamma$ correspond to planes $H$ tangent to $S$
at two points, one of which is parabolic; correspondingly the curve $H
\cap S$ has one cusp and one node. Points of type $\check \gamma$ are
honest points on $\check C$, in account of the cusp in $H\cap S$;
the presence of an additional, remote, node does not affect the local
geometry of the curve $\hat C$.
On the other hand, points of type $\check \gamma$ are cusps of
$\check B$: if one watches a general point of $\check B$ move towards
a point of type $\check \gamma$,
one sees a family of hyperplane sections of $S$ with
two nodes such that one the nodes degenerates to a cusp, and this is
the reason why points of type $\check \gamma$ are cuspidal points of
$\check B$, much in the same way as the curve in $\dual S$
corresponding to cuspidal tangent sections of $S$ is a cuspidal curve
of $\dual S$.
In less handwaving terms,
the local geometry of $\check B$ and $\check C$ at points of type
$\check \gamma$ is justified by the discussions in
\ref{p:type-gamma}
and \ref{p:transversality}.
The number $\check \gamma$ shall be derived indirectly in
\ref{p:2beta+gamma} below.

Points of type $\check \beta$ correspond to planes $H$ tangent to
$S$ at one point, such that the section $H \cap S$ has a tacnode
there. Indeed, points of type $\check \beta$ are cusps of $\check
C$, so that as a general point of $\check C$ moves towards a point of type
$\check \beta$, one must see a family of hyperplane sections of $S$ with
a cusp which degenerates to a tacnode. Going to a point of type $\check
\beta$ along $\check B$, one merely sees two nodes tending to a common
limit point, which is harmless for $\check B$, as indeed points $\check
\beta$ are smooth points of $\check B$.
The number $\check \beta$ will be derived in
\ref{p:beta-flecnodal} by considering the flecnodal locus in $S$.

Finally, points of type $\check t$ correspond to the famous
tritangent planes of $S$. Their number we shall
derive using formula (\hieroA {\pmglyph{\HZiv}}).


\paragraph{The flecnodal locus}
\label{p:flecnodal}
The \emph{flecnodal locus} is the locus of points
$q \in S$ such that there exists a line having intersection
multipliciy at least $4$ with $S$ at $q$.
It is a curve on $S$, and for a general point $q$ on this curve, the
tangent section $\T_qS\cap S$ has an ordinary double point at $q$,
such that one of the two local branches has a flex at $q$: the tangent
line to this branch is the one line having intersection multiplicity
$4$ with $S$ at $q$.

It has been shown by Salmon \cite[\S 588]{salmon2}
that the flecnodal curve is cut out on $S$
by a polynomial of degree $11n-24$, which we shall call the
\emph{flecnodal polynomial}. We describe his proof in
\cite[Section \tref{S:flecnodal}]{16.th+l-redres}.
A modern proof, and a generalization to arbitrary dimension,
is given in \cite{BASW}.
One can also find a brief account in
\cite[Section 8]{kollar-flecnodal},
and another generalization in \cite{alexeev-engel}.
Remarkably, the flecnodal polynomial vanishes modulo the equation of
$S$ if and only if $S$ is ruled
(note that the analogous vanishing property for the Hessian
characterizes developable ruled surfaces):
Salmon attributes this result to
Cayley; for a proof, see \cite[Section 8]{kollar-flecnodal},
or the references given in \cite{BASW}.

In \cite[\S 589--595]{salmon2}, Salmon gives the following explicit
formula for the flecnodal polynomial, which he attributes to Clebsch.
Let $F$ be an equation for $S$,
and denote by $\cH$ its Hessian matrix.
% and by $\H = \det(\cH) = \Hess(F)$ be its Hessian determinant.
Set
\[
  \Theta =
  \sum_{i,j}
  |\cH|_{i,j}
  \,\partial_i F \, \partial_j F,
  % \sum_{i,j}
  % \; \bigl|\, \cH \,\bigr|_{i,j}
  % \cdot \partial_i F \cdot \partial_j F,
\]
where $| \cH|_{i,j}$ denotes the cofactor formed by removing the $i$-th
row and the $j$-th column of $\cH$, \ie
$(-1)^{i+j}$ times the corresponding $3\times 3$
minor. 
Set
\[
  \Phi =
  - \sum_{i,j}\;
  \sum_{\substack{i_1<i_2 \\ j_1<j_2}}
  |\cH|_{i,j}
  \, |\cH|_{i_1i_2,j_1j_2}
  \, \partial_{ii_1i_2} F \, \partial_{jj_1j_2 }F
  % \; \bigl|\, \cH \,\bigr|_{i,j}
  % \cdot \bigl|\, \cH \,\bigr|_{i_1i_2,j_1j_2}
  % \cdot \partial_{ii_1i_2} F \cdot \partial_{jj_1j_2 }F
\]
where, in addition to the previous notation,
$|\cH|_{i_1i_2,j_1j_2}$ is $(-1)^{i_1+i_2+j_1+j_2}$ times the obvious
$2\times 2$ minor of $\cH$.
Then, the flecnodal polynomial is
\begin{equation}
\label{eq:flecnodal}
  \Theta-4 \Phi \,\Hess(F).
\end{equation}



\paragraph{Intersection of the parabolic and flecnodal curves}
\label{p:beta-flecnodal}
The points $q\in S$ such that the tangent section $\T_qS\cap S$ has a
tacnode at $q$ 
are the intersection points of the parabolic curve 
with the flecnodal curve.
Indeed, a point $q$ sits on the parabolic curve if and only if
$\T_qS\cap S$ has a double point at $q$ with degenerate tangent cone
(or a point of higher multiplicity), and it sits on the flecnodal
curve if and only if there is a line in the plane $\T_qS$ having
intersection multiplicity at least $4$ with the curve
$\T_qS\cap S$ at $q$.
With our blanket transversality assumption from
\ref{p:transversality}, this happens if and only if $\T_qS\cap S$ has
a tacnode at $q$.

The upshot of the above discussion is that the number $\check \beta$
is the 
number of intersection points of the parabolic and flecnodal curves,
which are cut out by polynomials of degrees $4(n-2)$ and $11n-24$,
respectively.
There is however one last subtlety, namely that the latter two curves
are everywhere tangent, see \ref{sp:He-Flec-touch}.
Therefore, one finds:
\begin{mycpctitem}
\item $\check \beta = 2n(n-2)(11n-24)$.
\end{mycpctitem}

\subparagraph{}\medskip
\label{sp:He-Flec-touch}
The fact that the parabolic and flecnodal curves are everywhere
tangent has been proved by Salmon \cite[\S 596]{salmon2};
a different proof has been given by McCrory and Shifrin
\cite{mccrory-shifrin}
in modern times.
In fact, Salmon even proves that the two surfaces cutting out the
parabolic and flecnodal curves on $S$ are everywhere tangent.

His argument is the following. Taking into account the expression
\eqref{eq:flecnodal} for the flecnodal polynomial, it suffices to show
that $\Theta$ is a square modulo the Hessian determinant $\Hess(F)$.
Now, it follows from a determinantal identity that for all $4$-tuples
$(c_i) \in \C^4$,
\[
  \Bigl( \sum
  |\cH|_{i,j}
  \,\partial_i F \, \partial_j F
  \Bigr)
  \Bigl( \sum
  |\cH|_{i,j}
  \, c_i \, c_j
  \Bigr)
  =
    \Bigl( \sum
  |\cH|_{i,j}
  \,\partial_i F \, c_j 
  \Bigr)^2
  \quad \mod \Hess(F).
\]
From the latter identity, Salmon deduces without further indication
that $\Theta$ is indeed a square modulo $\Hess(F)$.
I reckon that some additional arguments ought to be provided, but let
me not try to do it here.
Funnily enough, the squared factor on the right-hand-side of the last
identity has degree $7n-15$, a quantity that will show up later in a
seemingly unrelated manner, see \ref{p:H-dev-num}.




\paragraph{Intersection of the two double curves}
\label{p:2beta+gamma}
We now analyze the intersection of the
node-couple $\Kn_S$ and Hessian $\He_S$ curves on $S$.
For each point $q$ in their intersection, the tangent plane $\T_qS$
is either of type $\check \gamma$ or of type $\check \beta$,
and we shall see that the two curves are transverse if it is of type
$\check \gamma$, and tangent if it is of type $\check \beta$.

To a tangent plane of type $\check \gamma$ there corresponds a section
of $S$ with one node and one cusp, which gives two points on
$\Kn_S$, but only one of those lies on $\He_S$.
We add to our blanket transversality assumption that the two curves
are transverse at this point.

To a tangent plane of type $\check \beta$ there corresponds a
unique tangency point $q \in S$. 
On the one hand $q$ belongs to $\Kn_S$,
and it is a ramification point of the double cover
$\Kn_S \to \check B$, as $\T_qS \cap S$ may be seen as a bi-nodal
curve with the two nodes coalesced.
This implies that $T_q\Kn_S$ lies in the kernel of the differential of
the Gauss map of $S$ at $q$.
On the other hand $q$ is a ramification point of $\He_S \to \check C$ as
well, since $\check C$ has a cusp at $\orth {(\T_qS)}$, and this
implies that $T_q\He_S$ lies in the kernel of the differential of the
Gauss map of $S$ at $q$ (see also Lemma~\ref{pr:tg-to-Hess}). This
implies that the two curves $\Kn_S$ and $\He_S$ are tangent at $q$,
unless the differential of the Gauss map be $0$ at $q$, but this is
not the case by our blanket transversality assumption.

In the upshot, we find that
% \begin{align*}
% (K_S \cdot H_S) &= 2\beta + \gamma \\
% &= (n-2)(n^3-n^2+n-12)\cdot 4(n-2) \cdot n.
% \end{align*}
\begin{equation*}
\Kn_S \cdot \He_S
= 2\check \beta + \check \gamma.
\end{equation*}
Moreover, using the fact that both $\Kn_S$ and $\He_S$ are complete
intersections of $S$ and a hypersurface of known degree, we find
\begin{equation*}
\Kn_S \cdot \He_S
= (n-2)(n^3-n^2+n-12)\cdot 4(n-2) \cdot n.
\end{equation*}
We may now plug in the formula for $\check \beta$ obtained in
\ref{p:beta-gamma-t}, and obtain:
\begin{mycpctitem}
\item $\check \gamma = 4n(n-2)(n-3)(n^3+3n-16)$.\footnote
{There is a typo in the formula for $\check \gamma$ in \cite[\S
  630]{salmon2} ($n^3-3n-16$ instead of $n^3+3n-16$),
  which curiously enough goes back and forth between the various
  editions of the book, as Ragni Piene has pointed out to me.
The formula for $\check \gamma$ also appears in \cite[\S
612]{salmon2}, without the typo.}
\end{mycpctitem}


\paragraph{Formulae \refCuspEdg{} and the number
  of tritangent planes} 
\label{p:tritangent}
First of all let me mention that with the quantities we have been able
to find so far, formulae (\hieroA {\pmglyph{\HZi}}) and  (\hieroA
{\pmglyph{\HZii}}) are indeed verified (beware that $n$ should be
replaced by $\check n = n(n-1)^2$).

Formula  (\hieroA {\pmglyph{\HZiv}}) on the other hand yields the
number of tritangent planes to a smooth surface of degree $n$ in
$\P^3$:
\begin{mycpctitem}
\item $\check t=\frac 1 6 n(n-2)
(n^7-4n^6+7n^5-45n^4+114n^3-111n^2+548n-960)$.
\end{mycpctitem}



\section{Hessian and node-couple developables}
\label{S:He-Kn}


In this section we determine some more enumerative numbers related to
$0$-dimensional strata of a smooth surface $S \subset \P^3$ and its
dual, thus complementing the analysis carried out in the previous
Section \ref{S:zero-strata}.
These numbers are not immediately related to the enumeration of
hyperplane sections of $S$ with given singularities; for instance, we
determine the number of flexes of the cuspidal double curve
$\check C \subset \dual S$ (this is $\beta_\He$ in \ref{p:H-dev-num}),
and these
correspond to planes cutting out an honest tacnodal curve on $S$.
In general, we are concerned in this section with enumerative number
associated to the Hessian and node-couple developables (for the
definition, see Section \ref{s:dev-surf} below).

There are two main aspects to this study. On the one hand we shall
describe (in Section \ref{s:ord-dble-edges})
the ordinary double edges of the polar cone of a surface with
d-ordinary singularities, thus complementing the analysis of cuspidal
double edges in Section \ref{s:polcone-cusps} above.
On the other hand we will carry out
(in Section \ref{s:He-dev})
a detailed study of the geometry
of a surface along its parabolic curve, which I believe is interesting
for its own sake.



\subsection{Developables associated to curves on a surface}
\label{s:dev-surf}


We refer to Appendix \ref{ap:dev}
for the basics on developable surfaces in $\P^3$.

\paragraph{Developables associated to curves on a surface}
\label{p:dev-surf}
Let $Y$ be a curve traced on a surface $S \subset \P^3$.
Recalling that a developable surface in $\P^3$ merely amounts to a
one-dimensional family of planes,
one may
consider the developable surface $\Sigma_Y \subset \P^3$ corresponding
to the family of planes tangent to $S$ at points of $Y$.
In classical terms: this is the family of planes touching $S$ at
points of $Y$, and $\Sigma_Y$ is the surface
enveloped by the family of tangent planes to $S$ at points of $Y$.

Let $\gamma_S: S \dashrightarrow \dual S$ be the Gauss map of $S$. We
are considering the family of planes parametrized by the curve 
$\gamma_S(Y) \subset \check\P^3$.
By definition, the developable surface $\Sigma_Y$
is the dual surface $\dual {\gamma_S(Y)} \subset \P^3$ of the curve
$\gamma_S(Y) \subset \check\P^3$.
There exists a curve $\Gamma \subset \P^3$ such that 
$\Sigma_Y$ is the tangential surface $\Tan(\Gamma)$, but there is no
reason that $\Gamma$ should coincide with $Y$,
and neither that it should lie on $S$.

\paragraph{Hessian and node-couple developables}
The \emph{Hessian and node-couple developables} associated to a
smooth surface $S\subset \P^3$ are the developable surfaces $\Sigma_Y$
as in \ref{p:dev-surf} above with $Y$ the parabolic curve $\He(S)$ and
node-couple curve $\Kn(S)$, repectively.
They are the dual surfaces of the cuspidal and ordinary double curves
of $\dual S$, respectively, and
we will denote them by $\Sigma_\He$ and $\Sigma_\Kn$.

\begin{proposition}
The generators of the node-couple developable surface are the lines
joining pairs of conjugated points of the node-couple curve,
\ie the lines $\vect {p,q}$ such that there exists a plane
which is tangent to $S$ at both $p$ and $q$.
\end{proposition}

\begin{proof}
The node-couple developable is the dual of the curve
$\gamma_S(\Kn(S)) \subset \check \P^3$, so its generators are the
orthogonals of the tangents lines of $\gamma_S(K_S)$ (see
Section~\ref{s:dev-synth}).
Let $\varpi \in \gamma_S(K_S)$ be a general point.
There are two points $p,q \in S$ such that the plane
$H = \orth \varpi \subset \P^3$ is tangent to $S$ at both $p$ and $q$.
The tangent line
$\T_\varpi(\gamma_S(K_S))$ is the intersection of the
tangent planes to the two local sheets of $\dual S$ at $\varpi$,
respectively $\orth p$ and $\orth q$.
Therefore,
\[
\orth {\T_\varpi(\gamma_S(K_S))}
= \orth [\orth p \cap \orth q]{}
= \vect {p,q}.
\]
\end{proof}


We will determine the numerical characters of the node-couple
developable in Section \ref{s:chars-dev-dual}; we need the results of
Section \ref{s:ord-dble-edges} on the ordinary double edges of the
polar cone to do it.


In order to describe the generators of the developable $\Sigma_Y$ for
a general curve $Y$, we introduce the following device.


\paragraph{The involution $\iota_p$ on $\P(T_pS)$}
\label{p:invol-at-tg}
Let $p$ be a smooth, non-parabolic, point of a surface $S \subset
\P^3$.
There is a
self-map $\iota_p$ of the projective line $\P({T_pS})$
(indeed an involution by Proposition \ref{prop:invol-at-tg}
below),
which is defined as
follows. 
Let $u\in \P(T_pS)$ be a tangent direction at $p$.
The differential of the Gauss
map sends $u$ to a direction
$\gamma_S(u)$ in $\check \P^3$ tangent to $\dual S$ at
the point $\orth {(\T_pS)}$:
thus, $\gamma_S(u) \in \P\bigl(
T _{\orth {(\T_pS)}} \dual S
\bigr)$.
The tangent direction $\gamma_S(u)$ spans a line 
$\vect{\gamma_S(u)}$ such that
\[
  \orth {(\T_pS)}
  \,\subset\,
  \vect{\gamma_S(u)}
  \,\subset\,
  \T _{\orth {(\T_pS)}} \dual S.
\]
By biduality,
$\orth[\T _{\orth {(\T_pS)}} \dual S]{} \cong \{p\}$.
Therefore, the orthogonal of the line $\vect{\gamma_S(u)}$
is such that
\[
  p
  \,\in\,
  \orth {\vect{\gamma_S(u)}}
  \,\subset\,
  \T_pS,
\]
hence it defines a point $v \in \P( T_pS)$.
We define $\iota_p$ as the map $u\mapsto v$.

If one prefers, $u$ is
a point of $S$ infinitely near $p$.
Then $\gamma_S(u)$ is a point of $\dual S$ infinitely near the point 
$\orth {(\T_pS)}$.
Therefore, $\orth {\gamma_S(u)}$ is a tangent plane of $S$ infinitely
near the plane $\T_pS$.
The intersection of these two planes is a line
contained in $\T_pS$ and passing through $p$, and we let
$\iota_p(u)$ be its tangent direction at $p$.

We will consider the map $\iota_p$ indifferently
as a self-map of $\P({T_pS})$
or of the set of lines contained in $\T_pS$ and passing through $p$.

\begin{lemma}
\label{l:iota-dev!}
Let $Y$ be a curve traced on a surface $S \subset \P^3$,
and $p \in Y$ be a point which is non-parabolic on $S$.
Let $\Sigma_Y$ be the developable surface defined as in
\ref{p:dev-surf}.
Then $p$ sits on $\Sigma_Y$, and the generator of $\Sigma_Y$ through
$p$ is the line
$\iota_p(\T_pY)$.
\end{lemma}

\begin{proof}
By definition, $\Sigma_Y$ is the dual of the curve
$\gamma_S(Y) \subset \check \P^3$.
Therefore,
by the general theory of developable surfaces
(see Appendix \ref{ap:dev}),
the rulings of $\Sigma_Y$ are the orthogonals of the tangent lines of
$\gamma_S(Y)$.
The lemma then follows tautologically from the definition of $\iota_p$
in \ref{p:invol-at-tg}.
\end{proof}

\begin{proposition}
\label{prop:invol-at-tg}
The map $\iota_p$ is the orthogonality involution of $\P(T_pS)$
defined by the second fundamental form at $p$.
In particular, its fixed points are the tangent directions of the two
flex tangents of $S$ at $p$. 
\end{proposition}

Since $p$ is assumed to be non-parabolic, the second fundamental form
$\II_p$
at $p$ is a non-degenerate quadratic form on the tangent plane $T_pS$
(up to scalar multiplication), see Appendix \ref{app:hess}.
By definition, the orthogonality involution maps a vector line in
the vector plane $T_pS$ to its orthogonal with respect to $\II_p$,
which is another vector line in $T_pS$.

\begin{proof}
We consider homogeneous coordinates $(x:y:z:w)$ in $\P^3$, such that
$p=(0:0:0:1)$, and $\T_p S$ is the plane $z=0$. We write the equation
of $S$ in the form
% Locally at $p$, one may a consider $S$ in the affine space
% $\A^3_{xyz}$ with $p$ at the origin, and given by an of the form
\begin{equation*}
f(x,y,z,w)=
w^{n-1}z+w^{n-2}(ax^2+2rxy+by^2+2sxz+2tyz+cz^2)+ O(3)=0.
\end{equation*}
It follows from the local computation in \ref{p:Hess-II}
that the second fundamental form at $p$ is given by the matrix
\begin{equation}
\label{eq:II-p-baby}
  \begin{pmatrix}
a & r \\
r & b 
  \end{pmatrix}
\end{equation}
in the coordinates  $(x,y)$ on $T_pS$.
On the other hand,
the ``large'' Gauss map of $S$, defined on a Zariski open subset of
$\P^3$, maps the point $(x:y:z:w)$ to the transpose of  
\begin{equation*}
\begin{pmatrix}
\partial _x f \\ \partial _y f \\ \partial _z f \\ \partial _w f 
\end{pmatrix}
= \begin{pmatrix}
w^{n-2}(2ax +2ry+2sz)+\cdots \\ 
w^{n-2}(2rx+2by+2tz) + \cdots \\
w^{n-1} + w^{n-2}(2sx+2ty+2cz) + \cdots \\
(n-1)w^{n-2}z+\cdots
\end{pmatrix}.
\end{equation*}
We write it in the affine chart $w=1$; its differential at the origin
(\ie at $p$) is then
\begin{equation}
\label{eq:diff-gauss}
\begin{pmatrix}
2a\, dx +2r\, dy+2s\, dz \\
2r\, dx+2b\, dy+2t\, dz \\
2s\, dx+2t\, dy+2c\, dz  \\
(n-1)\,dz
\end{pmatrix}.
\end{equation}
Now, still in the affine chart $w=1$,
locally at $p$, $S$ is given by an
implicit function $z=\varphi(x,y)$ with vanishing differential at the
origin. In order to compute the differential of the ``small'' Gauss
map of $S$, defined on a Zariski open subset of $S$,
we need to compose the differential at the origin of
$(x,y)\mapsto (x,y,\varphi(x,y))$ with that of the ``large'' Gauss
map.
This amounts to set $dz=0$ in \eqref{eq:diff-gauss}.

The upshot is that the tangent plane to $S$ at the point infinitely
near $p$ in the direction $(u_0:u_1)$ is given by the equation
\begin{equation*}
(2au_0 +2ru_1)x
+(2ru_0+2bu_1)y
+(2su_0+2tu_1)z
=0.
\end{equation*}
Therefore its intersection with $\T_pS$ is given by 
\begin{equation*}
(2au_0 +2ru_1)x
+(2ru_0+2bu_1)y
=0,
\end{equation*}
hence $\iota_p$ is the involution
\begin{equation}
\label{involution-baby}
  \begin{pmatrix}
-r & -b \\
a & r 
  \end{pmatrix}
\in \PGL_2(\C)
\end{equation}
(it is indeed an involution because the trace of this matrix is $0$,
see \cite[Chap.~II, \S{D}]{samuel}).
By a straightforward computation
(in fact more or less the exact same computation that we have just
performed), this is the orthogonality involution
defined by the
bilinear form given by the matrix \eqref{eq:II-p-baby}, and this ends the
proof.
\end{proof}





\subsection{The Hessian developable surface}
\label{s:He-dev}

In this section we study the family of planes in $\P^3$ tangent to $S$
at its parabolic points, and the associated developable surface in
$\P^3$.  
We first need to adapt the observations of 
\ref{p:invol-at-tg} and \ref{prop:invol-at-tg}
to the case when $p$ is a parabolic point.

Let $p$ be a parabolic point of $S$. If $p$ is general, then the 
second fundamental form of $S$ at $p$ has rank $1$,
see Appendix \ref{app:hess},
hence the tangent section
$\T_pS\cap S$ has a degenerate double point at $p$,
and we call \emph{double asymptotic (or flex) tangent line} of $S$ at
$p$ the tangent cone $\TC_p(\T_pS\cap S)$.

\begin{proposition}
\label{pr:He-dev_I}
Let $p$ be a parabolic point of $S$ at which the second fundamental
form does not vanish.
Denote by $d\gamma_p$ the differential of the Gauss map of
$S$ at $p$, and by $\Lambda$ the double
asymptotic tangent line of $S$ at $p$.
Then:\\
(i) the kernel of $d\gamma_p$ is the tangent space at $p$ of
$\Lambda$;\\
(ii) the line in $\check \P^3$ passing through the point
$\orth {\T_pS}$ and going in the direction $\im(d\gamma_p)$ is the
orthogonal of $\Lambda$.
\end{proposition}


This tells, in particular, that if $p$ is a general parabolic point of
$S$, the map $\iota_p$ constructed in \ref{p:invol-at-tg} is
essentially a contraction of
$\P(T_pS)$ to its point corresponding to the double flex tangent line
of $S$ at $p$.


\begin{proof}
This follows from the computations carried out in the proof of
Proposition \ref{prop:invol-at-tg}.
Note that, in the notation
introduced there, we may assume $a=r=0$ since the
second fundamental form at $p$ has
rank $1$.
Then, we see from \eqref{eq:diff-gauss} that the kernel of $d\gamma$
is $y=0$, which is the reduced tangent cone of the tangent section
$\T_pS\cap S$ at $p$,
\ie the tangent space at $p$ of $\Lambda$.
In addition, we see from \eqref{involution-baby} that for 
$u=(u_0:u_1)$, the orthogonal of $\vect {d\gamma(u) }$ is $y=0$ if
$u_1\neq 0$ (and the whole $\T_pS$ is $u_1=0$). This proves (ii).
\end{proof}



\begin{remark}
Proposition \ref{pr:He-dev_I} is a biduality statement, the analog of 
\ref{p:biduality-flex-tg} for parabolic points.

Let $p$ be a general parabolic point. The line in $\check \P^3$
passing through the point $\gamma(p) = \orth {\T_pS}$
and going in the direction $\im (d\gamma_p)$ is the tangent line
$\T_{\orth {\T_pS}} \check C$ to the cuspidal double curve of $\dual S$ at
$p$, denoted by $\check C$.
Therefore, the proposition tells us that the orthogonal of 
the double flex tangent of $S$ at $p$ (denoted by $\Lambda$) is
the line $\T_{\orth {\T_pS}} \check C$.
We give another proof of this in Appendix \ref{S:asympt}.

Note that the double flex tangent $\Lambda$ is
the line of maximum contact with $S$ at $p$, and intersects $S$ with
multiplicity $3$,
and the tangent to the cuspidal edge,
$\T_{\orth {\T_pS}} \check C$,
is the line of maximum contact with $\dual S$ at the point
$\orth {\T_pS}$, and intersects $\dual S$ with multiplicity $4$ at
this point
(the intersection multiplicity
is $2$ for a general line, $3$ for a general line in the tangent cone,
and $4$ for the tangent of the cuspidal edge).
\end{remark}


\begin{figbox}
\includegraphics[height=20mm]{gauss-at-para}
\captionof{figure}{The Gauss map around the parabolic curve}
% {The image of a curve transverse to the double flex
% tangent is tangent to the cuspidal edge}
\end{figbox}


\begin{proposition}
\label{pr:tg-to-Hess}
Let $p$ be a parabolic point of $S$ at which the second fundamental
form does not vanish. The tangent line at $p$ to the
curve $S \cap \Hess(S)$ coincides with the double flex tangent line of
$S$ at $p$ if and only if the tangent section
$S \cap \T_pS$ has a tacnode at $p$ (or a worse singularity).
\end{proposition}

\begin{proof}%[Proof of Lemma \ref{pr:tg-to-Hess}]
Let us write the equation of $S$  in the form
\begin{equation*}
f(x,y,z,w)=
w^{n-1}z
+w^{n-2}\bigl(
{\textstyle \frac 1 2} y^2 + axz+byz+ 
{\textstyle \frac 1 2} c z^2 \bigr)
+w^{n-3}f_3(x,y,z)
+ O(4)=0,
%f_{\geq 4}(x,y,z,w)=0,
\end{equation*}
in a system of homogeneous coordinates $(x:y:z:w)$ such that
$p=(0:0:0:1)$
($n$ is the degree of $S$, and $f_{3}$ is homogeneous of degree $3$).
The tangent at $p$ to the Hessian curve is obtained by intersecting
$\T_p S$, that is, the plane $z=0$, with the tangent plane to the
Hessian, which we will find with formula \eqref{eq:hess-alt}. 

In the affine chart $w=1$, we have
\begin{align*}
\d x f &= az+ \d xf_3 + O(3) \\
\d y f &= y+bz+\d yf_3+O(3), \\
\d z f &= 1+ax+by+cz+ \d z f_3 + O(3)
\end{align*}
so that, up to a multiplicative constant, $\Hess(f)$ is
\begin{equation*}
\resizebox{\linewidth}{!}{%
$
\begin{vmatrix}
\frac{n}{n-1} (z+\frac 1 2 y^2 + \cdots) & 
az + \d xf_3 + \cdots & y+bz+ \d y f_3 + \cdots 
& 1+ax+by+cz+ \d z f_3 + \cdots 
\\
az + \d xf_3 + \cdots  
& \d x ^2 f_3 + \cdots & \d x \d y f_3 + \cdots
& a + \d x \d z f_3 + \cdots
\\ 
y+bz+ \d y f_3 + \cdots  
& \d x \d y f_3 + \cdots & 1 + \d y ^2 f_3 + \cdots 
& b + \d y \d z f_3 + \cdots
\\
1+ax+by+cz+ \d z f_3 + \cdots  
& a + \d x \d z f_3 + \cdots & b + \d y \d z f_3 + \cdots
& c + \d z ^2 f_3 + \cdots
\end{vmatrix}.
$
} % endresizebox
\end{equation*}
Plugging in $z=0$ and keeping for each entry only the terms of order
at most $1$, we obtain 
\begin{equation*}
\begin{vmatrix}
0 & 0 & y & 1+ax+by
\\
0 & \d x ^2 f_3  & \d x \d y f_3 
& a + \d x \d z f_3
\\ 
y
& \d x \d y f_3  & 1 + \d y ^2 f_3  
& b + \d y \d z f_3 
\\
1+ax+by
& a + \d x \d z f_3  & b + \d y \d z f_3 
& c + \d z ^2 f_3 
\end{vmatrix}.
\end{equation*}
The only linear term in this determinant is $\d x ^2 f_3$,
so the tangent line to $S \cap \Hess(S)$ has
equations
\begin{equation}
z = \d x ^2 f_3 = 0.
\end{equation}
Therefore,
it coincides with the double flex tangent line if and only if there is
no $x^3$ term in $f_3$, which is equivalent to the tangent section
of $S$ at $p$ having an equation of the form
\begin{equation*}
\frac 1 2 y^2 + y(a_{21}x^2+ a_{12}xy + a_{03}y^2) + O(4) = 0,
\end{equation*}
which is the local form of a tacnodal singularity.
\end{proof}


\begin{remark}
\label{rk:tacnodes-dev}
Let $p\in S$ be a point such that the tangent section $\T_pS\cap S$
has a tacnode at $p$
(in particular $p$ lies on the Hessian curve $\He(S)=S \cap \Hess(S)$).
It follows from
Proposition \ref{pr:tg-to-Hess} 
that the image of the Hessian curve $\He(S)$
by the Gauss map (\ie the cuspidal double curve of $\dual S$) has
a cusp at $\gamma_S(p)$.
(We had seen this fact already in \ref{p:swallowtail} and
\ref{sp:type-beta},
% that the cuspidal double curve itself has a cusp at $\gamma_S(p)$,
arguing that $\gamma_S(p)$ is a swallowtail of $\dual S$).

Indeed, if the second fundamental form has rank one at $p$, then
the kernel of the differential of the Gauss map at $p$
is the tangent space of the double flex
tangent of $S$ at $p$ by Proposition \ref{pr:He-dev_I},
and this coincides with the tangent space of $S \cap \Hess(S)$
by Proposition \ref{pr:tg-to-Hess}.
On the other hand, if the second fundamental form at $p$ is $0$, there
is nothing to prove.


\begin{proposition}
Let $p\in S$ be a point such that the tangent section $\T_pS\cap S$
has a tacnode at $p$.
The regression (\ie cuspidal) edge of the Hessian
developable $\Sigma_\He$ passes through $p$, and its osculating plane
there is $\T_pS$. In particular the two surfaces $\Sigma_\He$ and $S$
are tangent at $p$.
\end{proposition}

\begin{proof}
This follows from the fact,
which we have observed in \ref{sp:type-beta},
that $\orth p$ is the
osculating plane of the cuspidal double curve of $\dual S$,
which we will denote here by $C \subset \check \P^3$.
Note that it has a local parametrization of the form
$t\mapsto (t^2,t^3,t^4)$ at $p$, and has
intersection multiplicity $4$ with $\orth p$ at the point
$\orth [\T_pS]$, see \ref{p:swallowtail} and
\ref{sp:type-beta}.

Let $\Gamma \subset \P^3$ be the regression edge of $\Sigma_\He$.
By the general theory of developable surfaces, see
Appendix \ref{ap:dev}, $\Gamma$ parametrizes the osculating planes of
$C$. Thus, since $\orth p$ is an osculating plane of $C$,
$p=\orth [\orth p]$ sits on $\Gamma$.
Moreover, by the osc-duality for space curves, see again
Appendix \ref{ap:dev},
the osculating plane of $\Gamma$ at $p$ is the orthogonal of the point
at which $\orth p$ is osculating to $C$: the latter point is
$\gamma_S(p)=\orth [\T_pS]$, hence 
the osculating plane of $\Gamma$ at $p$ is $\T_pS$.
Finally, the tangent plane to $\Sigma_\He$ at $p$ is the osculating
plane of $\Gamma$ at $p$, which we have just seen is $\T_pS$.
\end{proof}
\end{remark}


\noindent
We may now give a direct geometric description of the Hessian
developable. 

\begin{theorem}
\label{t:geom-Hessdev}
The generators of the Hessian developable surface are the double flex
tangent lines at parabolic points of $S$. 
Its stationary planes are the tangent planes to $S$ at points where
the tangent section has a tacnode.
\end{theorem}

\begin{proof}
The identification of the generators follows from
Proposition \ref{pr:He-dev_I}
and Lemma \ref{l:iota-dev!} (which works fine even at parabolic
points).
That of the stationary planes follows from
Proposition \ref{pr:tg-to-Hess}, see also
Remark \ref{rk:tacnodes-dev}.
\end{proof}


The rest of this section is dedicated to the computation of the
numerical characters of the Hessian developable.


\begin{lemma}
Let $S,T$ be two surfaces in $\P^3$ of degrees $s,t$ respectively.
The degree of the ruled surface generated by the flex tangents of $S$
at the points of $S\cap T$ equals $st(3s-4)$.
\end{lemma}

Note that there is no reason that this ruled surface be developable in
general, although it is indeed when $T=\Hess(S)$.

\begin{proof}
Let $f,g$ be homogeneous equations of $S$ and $T$ respectively.
The ruled surface we are interested in is the projection on the first
factor of the incidence graph
\[
\bigl\{ 
(p,p') : p' \in S \cap T
\text{ and $p$ sits on a flex tangent of $S$ at $p'$}
\bigr\},
\]
which is the complete intersection in $\P^3 \times \P^3$ defined by
the following four bihomogeneous polynomials in the variables $(p,p')$:
$f(p')$, 
$g(p')$,
$\polar p f (p')$,
$\polar {p^2} f (p')$,
of bidegrees 
$(0,s)$,
$(0,t)$,
$(1,s-1)$,
and $(2,s-2)$respectively.

Our ruled surface is therefore the hypersurface in $\P^3$ 
defined by the homogeneous
equation obtained by eliminating the  variable $p'$,
\ie by the polynomial
\[
\Res _{s,t,s-1,s-2} \bigl( f,g, \polar p f, \polar {p^2} f \bigr),
\]
taken as a resultant of homogeneous polynomials in the variable $p'$,
with coefficients homogeneous polynomials in the variable $p$.
By a standard homogeneity property of the resultant,
see \cite[Theorem \tref{T:res}]{16.th+l-redres},
it is a homogeneous polynomial of degree
\begin{equation*}
\bigl[ 0 \times t(s-1)(s-2) \bigr]
+\bigl[ 0 \times s(s-1)(s-2)\bigr]
+\bigl[ 1 \times st(s-2)\bigr]
+\bigl[ 2 \times st(s-1) \bigr]
= st(3s-4)
\end{equation*}
in the variable $p$.
\end{proof}

\begin{corollary}
\label{c:rk-He-dev}
The degree of the Hessian developable surface equals
$2n(n-2)(3n-4)$.
\end{corollary}

% This quantity is called the \emph{rank} of the Hessian system in the
% classical terminology, cf.\ Appendix~\ref{ap:dev}.

\begin{proof}
We apply the above lemma with $T=\Hess(S)$.
This gives the degree $4n(n-2)(3n-4)$, which however has to be divided by
two, as the obtained equation is double in this case, being the two
flex tangents coincident at parabolic points.
\end{proof}


\paragraph{}
\label{p:cl-He-dev}
The class of the Hessian developable is the number of planes tangent
to $S$ at a parabolic point, and passing through a fixed general point
in $\P^3$. It is therefore the intersection number of $S$,
$\Hess(S)$, and $\polar {p'} S$ for a general $p' \in \P^3$, which
equals $4n(n-1)(n-2)$.

\paragraph{}
\label{p:stat-He-dev}
The number of stationary planes of the Hessian developable is, by 
Theorem~\ref{t:geom-Hessdev}, the number of points in the
intersection of the parabolic curve $S\cap \Hess(S)$ with the
flecnodal locus.
We have seen in \ref{p:beta-flecnodal} that this number is
$2n(n-2)(11n-24)$.

\paragraph{}
\label{p:H-dev-num}
We may now find the remaining characteristic numbers using the
formulae of Appendix~\ref{ap:dev}. 
We use the notation of
\ref{p:not-char-dev-I} and \ref{p:not-char-dev-II},
with an additional decoration '$\He$'
to avoid confusion;
see also the warning below.
We have found so far:
\begin{mycpctitem}
\item $r_\He = 2n(n-2)(3n-4)$,
  the degree (or rank) of the developable, see
  Corollary \ref{c:rk-He-dev};
\item $n_\He = 4n(n-1)(n-2)$,
  its class, see \ref{p:cl-He-dev};
\item $\alpha_\He = 2n(n-2)(11n-24)$,
  its number of stationary planes, see \ref{p:stat-He-dev}.
\end{mycpctitem}
Knowing three quantities is enough to derive all the others by
direct applications of the formulae in \ref{p:plucker-devI} and
\ref{p:plucker-devII}. 
This way one finds, as in \cite[\S 608]{salmon2}:
\begin{mycpctitem}
\item $m_\He = 4n(n-2)(7n-15)$, the degree of the regression edge of
  $\Sigma_\He$; 
% = n(n-2)(28n-60) 
\item $\beta_\He =10n(n-2)(7n-16)$, the number of flexes of the
  cuspidal double curve $\check C$ of $\dual S$;
% =n(n-2)(70n-160)
\item $g_\He=2 n (n - 2) (4 n^4  - 16 n^3  + 20 n^2  - 27 n + 39)$,
% $2g=n (n - 2) (16 n^4  - 64 n^3  + 80 n^2  - 108 n + 156)$
the number of apparent double points of $\check C \subset \dual S$;
\item $h_\He=2 n (n - 2) (196n^4  - 1232n^3  + 2580n^2  - 1861n + 137)$,
  % $2h=n(n-2)(784n^4  - 4928 n^3  + 10320 n^2  - 7444 n +548)$
  the number of apparent double points of the regression edge of
  $\Sigma_\He$.
\end{mycpctitem}

\subparagraph{Warning}\medskip
For ease of reference I have done my best to stick to Salmon's
notation, as other have done before me,
e.g., Piene \cite{piene-someformulas}, Ronga \cite{ronga-13}.
There are however some compatibility problems between the notation
of \ref{p:not-char-dev-I} and \ref{p:not-char-dev-II} for developable
surfaces,
and that of
\ref{p:d-ord-sings}, \ref{p:cusp-edg-polar-cone}, and
\ref{not:ord-edg-polar-cone}
for the singularities of the dual.
For instance, $\alpha_\He=\check \beta$,
both the number of stationary planes in the Hessian system
and of swallowtails of $\dual S$,
and $g_\He=\check h$, the number of apparent double points of the
cuspidal double curves of $\dual S$.

\subparagraph{References}\medskip
Some of these numbers have been computed by Kulikov in an interesting
series of two papers,
with intersection theoretic computations.
In particular, 
the number $\alpha_\He$ is computed in \cite{kulikov-calculus}
(``number of points $P_3$''),
and the number $\beta_\He$ is computed
(``number of points type $P_3$'') in \cite{kulikov-focal}; there the
regression edge of the Hessian developable is called the focal curve,
and ``points of type $P_3$'' are the cusps of this curve, hence
correspond to the flexes of $C = \dual{\Sigma_\He}$.

Moreover, \cite{kulikov-calculus} provides some invariants of the
flecnodal curve that we have not considered here.
``Points $H_3$'' are the ordinary double points of the flecnodal curve;
they are the points $q\in S$ such that both local branches at $q$
of the tangent section $\T_qS\cap S$ have a flex at $q$.
``Points $H_4$'' are the points where the flecnodal curve is tangent
to an asymptotic tangent line of $S$;
they are the points $q\in S$ such that the tangent section $\T_qS\cap
S$ has a branch at $q$ with a higher order inflection point.
Kulikov obtains:
\begin{mycpctitem}
\item $\#H_3 = 5n(7n^2-28n+30)$;
\item $\#H_4 = 5n(n-4)(7n-12)$.
\end{mycpctitem}
These numbers are given by Salmon as well, at 
\cite[\S 604]{salmon2}.






\subsection{Ordinary double edges of the polar cone}
\label{s:ord-dble-edges}



In this section we consider the same setup as in Section
\ref{s:polcone-cusps}, and use the notation introduced there. In
particular, we let $X$ be a degree $n$ surface in $\P^3$ with d-ordinary
singularities, and call $B$ and $C$ its ordinary and cuspidal double
curves. We consider a general point $p \in \P^3$, and denote by
$\cD^pX$ the polar cone of $X$ with respect to $p$, and by $\appbnd p
X$ the apparent boundary.


\paragraph{Ordinary double edges of the polar cone}
\label{p:dble-edg-polar-cone}
In this section we study the ordinary double edges of the polar cone
$\cD^pX$;
they are the lines passing through $p$ and
%bitangent to the surface $X$
intersecting $X$ with multiplicity $2$ in two distinct points.
The locus of points $q \in S$ such that the line
$\vect {p,q}$ verifies this condition is cut out on
$X\cap \polar p X$ 
by a degree $(n-2)(n-3)$ hypersurface $R^pX$:
this has been proved by Salmon,
and his construction is explained in
\cite[Section \tref{s:bitg-lines}]{16.th+l-redres}.
This hypersurface has been invoked in 
% \ref{s:double-curves}
\ref{sp:nodes-Bp}
already.

We shall conduct our study of ordinary double edges by analyzing the
various kinds of intersection points of this hypersurface $R^pX$ with
the curve $X\cap \polar p X$.
This strategy is similar to that followed in
Section \ref{s:polcone-cusps},
with the hypersurface $R^pX$ playing the role that the second polar
$\polar {p^2} X$ played there.


\begin{definition}
The \emph{number of apparent double points} of a curve in $\P^3$ 
is the number of double points of its projection from a general
point. 

The \emph{number of apparent only double points} of two curves $Y,Y'$
in $\P^3$ is
the number of intersection points of their projections from a general
point that do not come from an actual
intersection point of $Y$ and $Y'$.
We denote it by $[Y,Y']^\zero$.
\end{definition}


\paragraph{Notation}
\label{not:ord-edg-polar-cone}
We add the following notation to that introduced in Section
\ref{s:polcone-cusps}: 
\begin{mycpctitem}
\item $\delta$ is the number of ordinary double edges of the
  circumscribed cone $\cC_p X$ (these are the honest bitangent lines
  to $X$);
\item $k$ is the number of apparent double points of the ordinary double
  curve $B$ of $X$;
\item $h$ is the number of apparent double points of the cuspidal double
  curve $C$ of $X$;
\item $i$ is the number of intersection points of $B$ and $C$ smooth for
  both curves
(when $X=\dual S$ for a smooth $S$, this number vanishes).
\end{mycpctitem}


% Let $C$ and $C'$ be two curves in $\P^3$.
% Their \emph{number of apparent intersection points}, $[C\cdot C']$,
% is the intersection number of their plane projections $\pi_p(C)$ and
% $\pi_p(C')$ from a general point $p\in\P^3$; this is merely given by
% \[
% [C\cdot C'] = \deg(C)\cdot \deg(C').
% \]
% On the other hand, we define the \emph{number of \emph{only} apparent
%   intersection points} of $C$ and $C'$, denoted by
% $[C\cdot C'] ^\zero$, to be the number of intersection points of
% $\pi_p(C)$ and $\pi_p(C')$ that do not come from an actual
% intersection point of $C$ and $C'$.

% By abuse of notation, we also allow the same definition when $C$ or
% $C'$ is a cone over a curve with vertex at $p$.

% {\color{red}comme {\c c}a {\c c}a ne va pas, faire une d{\'e}finition ad hoc pour ce
% qui nous int{\'e}resse}

\medskip
The following formulae,
given by Salmon without any comment,
describe the intersection of the hypersurface $R^pX$ mentioned in
\ref{p:dble-edg-polar-cone} above with the various components of the
curve 
\[
  X\cap \polar p X = \appbnd p X + 2B +3C,
\]
of total degree $n(n-1)(n-2)(n-3)$.
Recall that $a,b,c$ denote the degrees of the curves
$\appbnd p X, B,C$
(called $A,B,C$ by Salmon), respectively.


\newcommand{\hieroB}[1]
{\smash{\raisebox{.6mm}{\pmglyph{\HMviii}}
\kern -6mm \raisebox{-1.1mm}{\pmglyph{\HDxlvii}}
\kern -1mm \raisebox{-1.15mm}{\pmglyph{\HMxvii}}
#1}}
\newcommand{\refSalmonBi}{(\hieroB {\pmglyph{\HZi}})}%
\newcommand{\refSalmonBii}{(\hieroB {\pmglyph{\HZiv}})}%
\newcommand{\refSalmonBiii}{(\hieroB {\pmglyph{\HZii}})}%

\begin{lemma}
The following relations hold:
\begin{align}
%\label{eq:B0}
\tag{\hieroB {\pmglyph{\HZi}}}
a(n-2)(n-3) &= 2\delta + 2[\appbnd p X \cdot B]^\zero
+ 3[\appbnd p X \cdot C]^\zero~;\\
\tag{\hieroB {\pmglyph{\HZiv}}}
b(n-2)(n-3) &= 4k + [\appbnd p X \cdot B]^\zero + 3[B \cdot C]^\zero~;\\
\tag{\hieroB {\pmglyph{\HZii}}}
c(n-2)(n-3) &= 6h + [\appbnd p X \cdot C]^\zero + 2[B \cdot C]^\zero.
\end{align}
\end{lemma}

\begin{proof}
Let $Y,Y'$ be two curves (possibly the same) among $\appbnd p X,B,C$,
and denote by
$m_Y, m_{Y'}$ their multiplicities in the cycle $X\cap \polar p X$.
An intersection point between two local branches of the projections
$\pi_p(Y)$ and $\pi_p(Y')$ gives a double
edge of the polar cone with multiplicity $m_Y m_{Y'}$, hence two
contact points $y \in Y$ and $y'\in Y'$ with $X$,
each of which should contribute with the same multiplicity
$m_Y m_{Y'}$ to the intersection
$X\cap \polar p X \cap R^pX$.
Taking into account the multplicities of $Y$ and $Y'$ in $X \cap
\polar p X$, one finds that $R^pX$ should intersect $Y$ with
multiplicity 
$m_{Y'}$ at $y$ and $Y'$ with multiplicity $m_Y$ at $y'$.
This explains all the coefficients in the formulae.
\end{proof}

Some claims in the above proof arguably deserve a more
rigorous treatment, but let me not try to fix this here.
Note that
the actual intersection points of $\appbnd p X,B,C$ do not contribute
to the intersection $X \cap \polar p X \cap R^pX$, as they give
rise to cuspidal double edges of the polar cone instead of ordinary
double edges.

For two curves $Y$ and $Y'$ in $\P^3$, 
the total number of intersection points of the projections $\pi_p(Y)$
and $\pi_p(Y')$ is $\deg(Y) \deg(Y')$.
The following set of formulae,
yet again given cold-bloodedly by Salmon,
indicates the quantities to be subtracted
from $\deg(Y) \deg(Y')$ to obtain $[Y,Y']^\zero$,
in the case when $Y$ and $Y'$ are two components of
$X\cap \polar p X$.


\newcommand{\refAOIPi}{(\smash{\pmglyph{\HFi \HZi}})}%
\newcommand{\refAOIPii}{(\smash{\pmglyph{\HFi \HZiv}})}%
\newcommand{\refAOIPiii}{(\smash{\pmglyph{\HFi \HZii}})}%

\begin{theorem}
\label{t:ord-edges}
The following relations hold:
\begin{align}
%\label{eq:apparent-inteprs}
\tag{\smash{\pmglyph{\HFi \HZi}}}
[\appbnd p X \cdot B]^\zero &= ab-2\rho \ ;\\
\tag{\smash{\pmglyph{\HFi \HZiv}}}
[\appbnd p X \cdot C]^\zero &= ac-3\sigma \ ;\\
\tag{\smash{\pmglyph{\HFi \HZii}}}
[B \cdot C]^\zero &= bc-3\beta-2\gamma-i.
\end{align}
\end{theorem}

\begin{proof}
In our setup, every actual intersection point of two curves among
$\appbnd p X,B,C$ is of one of the types $\rho,\sigma,\beta,\gamma,i$,
so only 
the coefficients are to be explained. 
The latter are the intersection multiplicities at the corresponding
points 
of the projections from $p$ of the two curves under consideration.
For points of type $i$, it is $1$ by the generality of $p$. The rest
of the proof consists in examining one by one the other possible
types. 

\medskip
\subparagraph{Points of type $\rho$}
\label{p:ord-edg-rho}
These are the points $q \in \appbnd p X \cap B$. At such a point, the surface
$X$ has two smooth local sheets $X'_q$ and $X''_q$, $B=X'_q \cap
X''_q$ and 
the circumscribed curve $\appbnd p X$ is contained in one of them, say
$X'_q$,  
and transverse to $B$. The curve $\appbnd p X$ is the ramification
curve of the 
projection of $X'_q$, hence the projections of $\appbnd p X$ and $B$
are tangent 
at the projection of $q$, and thus intersect with multiplicity $2$.

\medskip
\subparagraph{Points of type $\sigma$}
These are the points $q \in \appbnd p X \cap C$. At such a point, the
surface $X$ has one cuspidal local sheet $X_q$, and $C= \Sing (X_q)$. 
We have seen in \ref{p:sigma-cusp} that $\appbnd p X$ and $C$ are
smooth and tangent at $q$, and it follows from the same argument as
in \ref{p:ord-edg-rho} that their projections from $p$ are tangent.
But the claim is that, in fact, the two projections intersect with
multiplicity $3$.

It should be possible to prove this with a local computation, using the
setup of \ref{p:sigma-cusp}, but I have not been able to do it in
general. The difficulty is that,
while the curve defined by the two equations $f$ and $\polar p f$
splits as $\appbnd p X + 3C$ locally at $q$
(in the notation of \ref{p:sigma-cusp}), neither of the two
summands is a Cartier divisor on $X$, and therefore it is difficult to
find their equations.
It is however doable in practice for an arbitrary, explicit, choice of
the polynomials $g_2$ and $h_2$, using one's favourite computer
algebra system;
I have done it for several randomly chosen polynomials, using
Macaulay2; I recommend to do this over a finite field.
Finally, once one knows equations for $C$ and $\appbnd p X$, one finds
equations for their projections by eliminating the variable $x$
(because $p=(1:0:0:0)$), and it only remains to check with one's own
eyes that the intersection multiplicity at the projection of $q$ is
indeed $3$.

In any event,
the number $[\appbnd p X\cdot C]^\zero$ occurs only in 
\refSalmonBi{} and \refSalmonBiii{}, in which we already
know all the other numbers involved.
One may therefore use them to find $[\appbnd p X\cdot C]^\zero$,
and thus obtain an indirect proof of Formula \refAOIPii{}.


\medskip
\subparagraph{Points of type $\beta$}
These are the swallowtail singularities of $X$. At these points $B$ is
smooth and $C$ is cuspidal, and we can see on the local model in
\ref{p:swallowtail} that they have the same reduced tangent cone.
It follows that after projection they intersect with multiplicity $3$
at these points.

\medskip
\subparagraph{Points of type $\gamma$}
These are the points at which $X$ has two transverse local sheets, one
smooth: $X_q^\rs$, and the other cuspidal: $X_q^\rc$.
There $C$ is smooth and $B$ is cuspidal, and these two curves have
transverse reduced tangent cones. It follows  that after projection
they intersect with multiplicity $2$ at these points.

\medskip\noindent
Theorem~\ref{t:ord-edges} is now proved.
\end{proof}

% \begin{figure}
% \centering
% \includegraphics[height=25mm]{BC-gamma}
% %\captionof{figure}
% \caption{Local picture of $X$ at a point of type $\gamma$}
% \end{figure}


\noindent
Finally, putting together formulas 
(\hieroB {}\kern -1.7mm) and 
(\pmglyph{\HFi}\kern -.6mm) gives the following.
\newcommand{\hieroBi}[1]
{\smash{\raisebox{.6mm}{\pmglyph{\HMviii}}
\kern -6mm \raisebox{-1.1mm}{\pmglyph{\HDxlvii}}
\kern -1mm \raisebox{-1.15mm}{\pmglyph{\HPWii}}
#1}}


\paragraph{Corollary} 
\label{c:ord-dble-edg}
\begin{align}
%\label{eq:B0}
\tag{\hieroBi {\pmglyph{\HZi}}}
a(n-2)(n-3) &= 2\delta + 2ab+3ac-4\rho-9\sigma
\ ;\\
\tag{\hieroBi {\pmglyph{\HZiv}}}
b(n-2)(n-3) &= 4k + ab+3bc-9\beta-6\gamma-3i-2\rho
\ ;\\
\tag{\hieroBi {\pmglyph{\HZii}}}
c(n-2)(n-3) &= 6h+ac+2bc-6\beta-4\gamma-2i-3\sigma.
\end{align}



\subsection{Application to the case when $X=S^\vee$}%$X=\dual S$}
\label{s:chars-dev-dual}

We now proceed as in Section~\ref{s:app-dual-tritg},
\ie
we let $X$ be the dual of a smooth, sufficiently general,
degree $n$ surface $S \subset
\P^3$, and apply the formulas of
Section~\ref{s:ord-dble-edges} above to $X$.
We maintain the setup and notation introduced
in Section~\ref{s:app-dual-tritg}.


\paragraph{}
As in \ref{p:checkA}, the circumscribed cone $\cC ^{\check p}(\dual
S)$ is the dual in $\check \P^3$ of the plane curve $\orth {\check p}
\cap S$. The number $\check \delta$ of ordinary edges of this cone is
therefore the number of bitangents of the plane curve $\orth {\check p}
\cap S$, which by \ref{p:pluecker-sm-plane} is:
\begin{mycpctitem}
\item $\check \delta = 
\frac 1 2 n(n-2)(n-3)(n+3)$.
\end{mycpctitem}

% The number $\check \delta$ counts those lines $\ell \subset \check
% \P^3$ passing through the point $\check p$ and tangent to $\dual S$ at
% two points $q_1$ and $q_2$. Equivalently, the line $\orth \ell \subset
% \P^3$ should be contained in the general plane $H_{\check p} := \orth
% {\check p}$, and in two planes $\orth {q_1}$ and $\orth {q_2}$ both
% tangent to $S$. In turn, this is equivalent to the line $\orth \ell
% \subset H_p$ being a bitangent of the proj

\paragraph{}
The numbers $\check h$ and $\check k$ are the invariants $g$ 
(introduced in \ref{p:not-char-dev-II}) of the Hessian and node-couple
developables respectively. The former has been computed in
\ref{p:H-dev-num}
and the latter we don't know yet:
\begin{mycpctitem}
\item $\check h=g_\He =
  2 n (n - 2) (4 n^4  - 16 n^3  + 20 n^2  - 27 n + 39)$~;
\item $\check k=g_\Kn$.
\end{mycpctitem}


\paragraph{Examination of formulae
  ({\protect\hieroBi{\hspace{-.4em}}})
}
\label{p:g_Kn}
The numbers $\check n, \check a, \check b, \check c$ have been given
in Section \ref{s:app-dual-tritg},
and the numbers $\check \rho, \check \sigma, \check \beta, \check
\gamma$ have already been computed.
As we mentioned earlier, the number $\check \imath$ vanishes.
One may thus check by a direct computation that the first and third
identities of \ref{c:ord-dble-edg} indeed hold.
The second one, on the other hand, gives the formula:
\begin{mycpctitem}
\item $\check k= \frac 1 8
n (n - 2) (n^{10} - 6 n^9  + 16 n^8  - 54 n^7  + 164 n^6  - 288 n^5  +
547 n^4  - 1058 n^3 + 1068 n^2  - 1214 n + 1464)$.
\end{mycpctitem}



\paragraph{Numerical characters of the node-couple developable}
At this point, we know the following three numerical characters of the
node-couple developable:
$n_\Kn=\check b$, the degree of the curve $\check B \subset \check
\P^3$, 
$g_\Kn = \check k$, the number of apparent double points of $\check
B$,
and $\alpha_\Kn=\check \gamma$, the number of cusps of $\check B$.
We may therefore
derive all the others using the formulas of
Section~\ref{s:plucker-dev};
however, these ought to be suitably modified in order to take
into account the presence of $\check t$ ordinary triple points on the
curve $C_\Kn = \check B$.
This may be taken care of in various
ways, but the idea is always the same, namely that an ordinary triple
point counts exactly as three nodes.

For instance, let us adapt the formula
$r=n(n-1)-2g-3\alpha$ from
\ref{p:plucker-devI}
in order to compute the rank $r_\Kn$ of the node-couple developable.
The adapted formula is
\begin{align*}
r_\Kn &= n_\Kn (n_\Kn-1)-2\bigl(g_\Kn+3\#(\text{triple points})\bigr)
-3\alpha_\Kn \\
&= \check b (\check b -1) - 2\check k -6 \check t - 3\check \gamma,
\end{align*}
and it gives
\begin{mycpctitem}
\item $r_\Kn = 
n (n - 2) (n - 3) (n^2  + 2 n - 4)$.
\end{mycpctitem}
We leave this task for the remaining numerical characters an exercise
to the not-exhausted-yet reader. 


\bigskip
Finally, I would like to mention the article
\cite{corvaja-zucconi}, in which the authors perform an interesting
study of the family of bitangent lines of a very general quartic
surface, which involves in particular the node-couple developable.




\section{Formulae for surfaces projected in $\P^3$}
\label{S:enriques}

In this section, we prove formulae for the enumeration of
curves with prescribed singularities in a possibly incomplete linear
system of dimension $r \leq 3$ on a smooth surface;
this will take the form of enumerating curves on a surface in $\P^3$
with ordinary singularities, see \ref{p:setup-enr-dim3}.
These formulae are from a different age with respect to those
of Salmon, and involve invariants of a different nature, \eg
the arithmetic genus;
by the way, beware the difference in notation with respect to the
previous sections. The material presented here is taken from
\cite[Capitolo V]{enriques}.



\paragraph{Setup}
\label{p:enr-setup}
We consider a linear system $|V|$ of dimension $r \leq 3$ on a smooth
surface $S$.
We will usually make some transversality assumptions on $|V|$, which
are typically granted
if $|V|$ is a general subsystem of a very
ample linear system.
In particular, we always assume that the general member of $|V|$ is
smooth and irreducible. 
We set:
\begin{mycpctitem}
\item $C$ the linear equivalence class of divisors in $|V|$ (and
  sometimes a member of $|V|$ by abuse of notation)~;
\item $n$ the degree of $|V|$, \ie $n=C^2$~;
\item $\pi$ the common arithmetic genus of all members of $|V|$.
\end{mycpctitem}
We have the following first identity,
given by the adjunction formula:
\begin{equation}
\label{KC-adj}
K_S \cdot C = 2\pi-2-n.
\end{equation}


\paragraph{Warm up: the $1$-dimensional case}
\label{p:enr-1dim}
Let $r=1$, and assume that $|V|$ has $n$ simple
base points, and all its singular members are $1$-nodal curves.
In this context, we define
the class $\check n$ of $|V|$ as the number of its
singular members.
In this case, the topological formula
discussed in details in
\cite[Section \tref{s:pencil}]{10.th-panoramico}
gives:
\begin{mycpctitem}
\item
$\check n = e(S)+n-e(C)\cdot e(\P^1)
= c_2(S)+n+4\pi-4$.
\end{mycpctitem}

\bigskip 
Next we treat the case $r=3$.
For $r=2$ we shall only consider a cheap version in which we assume
that $|V|$ is a subsystem of a linear system of dimension at least
$3$. 


\subsection{The $3$-dimensional case: surfaces with ordinary
  singularities}
\label{s:enr-dim3}

In this section we let $r=3$, and make the following assumption,
granted by 
the general projection theorem,
see \cite{gruson-peskine}, 
if $|V|$ is a general subssytem of a very ample linear system.

\paragraph{}
\label{p:setup-enr-dim3}
We assume that the map defined by $|V|$ is a
birational morphism from $S$ to a degree $n$ surface $S^\flat \subset
\P^3$ with \emph{ordinary singularities} (in the usual sense), \ie
$S^\flat$ is smooth except for an ordinary
double curve $D$ with $\tau$ pinch points and $t$ triple points:
locally at a pinch point $S^\flat$ has a Whitney umbrella singularity,
\ie it looks like the hypersurface $x^2-zy^2=0$
in the affine space with coordinates $x,y,z$;
locally at a triple point it looks like the hypersurface $xyz=0$, so
these points are non-planar triple points for $D$;
locally at all other points of $D$, $S^\flat$ looks like the
hypersurface $xy=0$;
in particular, $D$ is smooth except for the triple points.
For simplicity, 
we assume moreover that $D$ is irreducible.



The morphism $\nu:S \to S^\flat$ is the normalization map. We let $\Delta
\subset S$ be the pre-image of $D \subset S^\flat$; there is a double
cover $\Delta \to D$, which ramifies exactly over the $\tau$ pinch
points. 
By adjunction theory
(see, \eg \cite[Exer.~II.8.5]{hartshorne-13}
and \cite[Section \tref{E:S:cond}]{02.edoardo}), one has
$\omega_S \cong \O_S(-\Delta) \otimes \nu^* \omega_{S^\flat}$, and 
$\nu_* \omega_S = \restr {\cI_D} {S^\flat}$, where $\cI_D$ is the
sheaf of ideals defining $D$ in $\P^3$.
Being $S^\flat$ a divisor in $\P^3$, we have
$\omega_{S^\flat} \cong 
\restr {\omega_{\P^3}(S^\flat)} {S^\flat}
= \O_{S^\flat}(n-4)$
by the standard adjunction formula.

\paragraph{}
In addition to the already introduced notation
(see also \ref{p:enr-setup}), we let:
\begin{mycpctitem}
\item $\tau$ be the number of pinch points of $S^\flat$~; 
\item $t$ be the number of triple points of $S^\flat$~; 
\item $d$ be the degree of the double curve $D \subset \P^3$~;
\item $\rho$ be the geometric genus of $D$~;
\item $\Pi$ be the geometric genus of $\Delta \subset S$.
\end{mycpctitem}


\paragraph{}
The curves $C$ are represented in $\P^3$ as hyperplane sections of
$S^\flat$, hence as degree $n$ plane curves with $d$ nodes. Therefore
one has
\begin{equation}
\label{enriq3}
\pi = \binom {n-1} 2 -d.
\end{equation}


\paragraph{Effective degree of first polars}
\label{p:enr-1st-polars}
We compute the class $\check n$ of $S^\flat$, that is the number of
singular curves in a general subpencil of $|V|$, following the
method explained in \ref{p:-deg-dual-polars}.

For a general point $p \in \P^3$, the first polar $\polar p {S^\flat}$
is a degree $n-1$ hypersurface passing simply through $D$,
and we define the apparent boundary 
$\appbnd p S^\flat$
as the Zariski closure of $(\polar p {S^\flat} \cap S^\flat)-D$,
as in \ref{p:polar-cones}.
The curve $\appbnd p S^\flat$ passes through all pinch points:
this follows from a local computation, which we reckon the reader who
has survived this far can make on his own.

Therefore, for a general pair of points $p,q\in\P^3$ the intersection
of the two curves
$\appbnd p S^\flat$
and $\appbnd q S^\flat$
consists of the $\tau$ pinch
points of $S^\flat$ plus the $\check n$ points $a$ such that 
$p,q \in \T_aS$. To compute this intersection number $\tau+\check n$,
we pull-back the curves to the normalization $S$.
They are sections of 
\[
\cI_D \otimes \O_{S^\flat}(n-1) \cong 
\cI_D \otimes \omega_{S^\flat} \otimes \O_{S^\flat}(3),
\]
hence pull-back to curves in the class $K_S+3C$.
We thus find the identity
\begin{equation}
\label{enriq2}
\check n + \tau 
= (K_S+3C)^2
= K_S^2 +3n +12\pi -12,
\end{equation}
using \eqref{KC-adj} to substitute the intersection number $K_S\cdot
C$. 


\paragraph{Genus of the curve of neutral pairs of $|V|$}
One first observes that the curve $\Delta$ has three nodes above each
triple point of $S^\flat$, as is best understood looking at 
Figure \ref{fig:n-triple}.
\begin{figure}
\centering
\includegraphics[height=30mm]{dble-curve.eps}
\caption{Normalization of $S^\flat$ at a triple point}
\label{fig:n-triple}
\end{figure}
Since it is otherwise smooth, its
arithmetic genus is
$p_a(\Delta)=p_g(\Delta)+3t = \Pi+3t$.
On the other hand, 
using the already seen identity $K_S = (n-4)C-\Delta$,
the adjunction formula gives
\begin{equation*}
2(\Pi+3t)-2 =
2p_a(\Delta)-2 = (K_S+\Delta)\cdot \Delta
=(n-4)C\cdot \Delta = 2(n-4)d.
\end{equation*}
Therefore,
\begin{equation}
\label{enriq4}
p_a(\Delta)= \Pi + 3t = (n-4)d+1.
\end{equation}
% \begin{equation}
% \label{genusDelta}
% p_a(\Delta)= (n-4)d+1.
% \end{equation}

On the other hand, the map $\Delta \to D$ lifts to a
$2:1$ covering $\bar\Delta \to \bar D$ between the normalizations of
$\Delta$ and $D$. It is ramified
at $\tau$ points, so the Riemann--Hurwitz formula gives
\begin{equation}
\label{enriq5}
2\Pi-2 = 2(2\rho-2)+\tau.
\end{equation}


\paragraph{Intersections of apparent boundaries with the double curve}
Let $p \in \P^3$ be a general point. We consider the apparent boundary 
$\appbnd p S^\flat$
and its intersection with 
the double curve $D$.
To see the situation clearly, it is best to work on the
normalization $S$. 
One has
\begin{equation*}
\nu^*\appbnd p S^\flat \cdot \Delta
= (K_S+3C)\cdot \bigl( (n-4)C-K_S \bigr)
= -K_S^2 +2\pi(n-7) +2n^2 -7n +14.
\end{equation*}
Geometrically this intersection amounts to the $\tau$ pinch points
plus the points $q\in D$ such that the tangent plane to one of the two
local sheets of $S^\flat$ at $q$ passes through $p$. Let $a$ be the
number of the latter points. It may be computed by considering the
intersection of the second polar $\polar {p^2} S^\flat$ with $D$. 
It follows from Theorem \ref{t:polars-tglines} that this intersection
consists of the $a$ points we are interested in plus the $t$ triples
points, and since those are triple for $D$ one finds
\begin{equation*}
a+3t= (n-2)d.
\end{equation*}
Finally, we end up with 
\begin{equation}
\label{enriq6}
\tau + [ (n-2)d -3t
]
= -K_S^2 +2\pi(n-7) +2n^2 -7n +14.
\footnotemark
\end{equation}
\footnotetext{There is a typo in \cite[Formula (6), p.~175]{enriques},
but the final formulas on p.~176 agree with ours in
\ref{enr-formulas}.} 


\paragraph{Postulation formula}
We shall also use the following formula for the arithmetic genus of
$S$, which we shall discuss in Section \ref{s:postulation}:
\begin{equation}
\label{postulazione}
p_a( S) = 
\binom {n-1} 3 - (n-4)d + \rho + 2t -1.
\end{equation}


\paragraph{Conclusion}
\label{enr-formulas}
We may now express the quantities 
$\check n$, $\tau$, $t$, $d$, $\rho$, $\Pi$ in terms of the four
invariants $n$, $\pi$, $p_a(S)$, $K_S^2$.
The formula for $d$ is readily given by \eqref{enriq3}; we use it so
substitute for $d$ in the five equations
\eqref{enriq2},
\eqref{enriq4},
\eqref{enriq5},
\eqref{enriq6},
\eqref{postulazione},
thus obtaining
\[
\begin{pmatrix}
1 &&&& 1 \\
 & 2 & 6 \\
& 2 & 0 & -4 & -1 \\
&& -3 & 0 & 1 \\
&& -2 & -1 & 0
\end{pmatrix}
\begin{pmatrix}
\check n \\ \Pi \\ t \\ \rho \\ \tau
\end{pmatrix}
= \begin{pmatrix}
3n +12\pi +K_S^2 -12 \\
(n-4)(n-1)(n-2)-2(n-4)\pi +2 \\
-2 \\
-\frac 1 2 n^3+\frac 9 2 n^2-11n+16
-K_S^2+\pi(3n-16) \\
\frac 1 6 (n-1)(n-2)(-2n+9) + \pi(n-4)-p_a( S) 
-1
\end{pmatrix}.
\]
This finally gives:
\begin{mycpctitem}
\setlength{\itemsep}{1mm}
\item $\check n
= n  + 4 \pi + 12 p_a(S) - K_S^2 + 8$~;
\item $d=
\frac 1 2 (n-1)(n-2) - \pi$~;
\item $\rho=
\frac 1 2 (n^2-7n)+ \pi(n - 12) + 9 p_a(S) - 2 K_S^2 +22$~;
\item $\Pi=
n^2-6n + 2\pi(n-10) + 12 p_a(S) - 3 K_S^2+33$~;
\item $t=
\frac 1 6 (n^3 - 9 n^2  + 26 n)
-\pi (n - 8) - 4 p_a(S) + K_S^2-12 $~;
\item $\tau=
2 n + 8 \pi - 12 p_a(S) +2 K_S^2- 20$.
\end{mycpctitem}

\paragraph{Choice of four independent invariants}
I have chosen to follow Enriques' notation for ease of reference. I
have however substituted the old-fashioned \emph{linear genus}
$p^{(1)}(S)$ with $K_S^2$.
Indeed, $p^{(1)}(S)$ is defined as the \emph{virtual} genus of canonical
sections of $S$, that is the genus of the curves in $|K_S|$ obtained
from the adjunction formula, even though $|K_S|$ may in fact be
empty. 
In other words $p^{(1)}$ is defined by the formula
\[
2p^{(1)}-2=(K_S+K_S)\cdot K_S,
\]
hence $p^{(1)} = K_S^2+1$.

Nowadays the custom is to use $C^2$, $K_S\cdot C$, $K_S^2$, $c_2(S)$
rather than $n$, $\pi$, $p_a(S)$, $K_S^2$.
To obtain the above formulas in this form, simply use
\begin{equation}
\label{noether}
C^2=n;\qquad
K_S\cdot C+C^2=2\pi-2;\qquad
1+p_a(S)=\frac 1 {12} \bigl(K_S^2+c_2(S)\bigr).
\end{equation}
The former two relations we have already encountered, and the latter
is the well-known Noether formula (see, \eg
\cite[Example A.4.1.2]{hartshorne-13};
a modern proof in classical spirit is given in \cite{piene-noether};
we shall prove it in \ref{p:enr-class}).


\subsection{The postulation formula}
\label{s:postulation}

In this section we discuss the postulation formula
\eqref{postulazione}, which gives an expression for the arithmetic
genus $p_a(S)$ in terms of the projection $S^\flat$ in $\P^3$.
Here, we give a first simple proof of the formula,
and then explain the classical definition of the arithmetic genus
and why it coincides with the modern definition, which gives another
simple proof of the formula.
The postulation formula is discussed in \cite{piene-noether} as well.
The interested reader may also wish to consult
\cite[Chap.~III]{zariski-mumford},
in addition to \cite[Cap.~IV]{enriques}.


\begin{definition}
\label{p:genera-defs}
Let $X$ be a variety.
The \emph{arithmetic genus} of $X$ is
\[
p_a(X):=(-1)^{\dim X} \bigl(\chi(\O_X)-1\bigr).
\]
If $X$ is smooth, its \emph{geometric genus} is
\[
p_g(X):=h^0(X,\omega_X).
\]
\end{definition}

\noindent
If $X$ is a degree $n$ hypersurface in $\P^N$, one finds
\begin{equation}
\label{eq:pa-deg-n}
  p_a(X)=h^0(\O_{\P^N}(n-N-1))=\binom {n-1} N.
\end{equation}


\paragraph{Arithmetic and geometric genera of a curve}
\label{p:pa-pg-curves}
For a smooth curve there is no
difference between the arithmetic and geometric genera; it is
important to note that the same does not hold in higher dimension.
One defines the geometric genus of an arbitrary reduced curve as the
genus of its normalization.
The arithmetic and geometric genera of a curve $X$
may be related by means of the exact sequence
\begin{equation}
\label{exseq-norm-curv}
0 \to \O_{X} \to \nu_* \O_{\bar X} \to 
\textstyle {\bigoplus_{p\in \Sing(X)}} (\C_p)^{\oplus \delta(p)}
\to 0,
\end{equation}
where $\nu:\bar X \to X$ is the normalization map, and the third
term is a skyscraper sheaf supported on the singular locus of $X$,
with $\delta(p)$ an integer depending on the type of singularity,
see \cite[Section \tref{E:S:cond}]{02.edoardo}.
Taking Euler characteristics in \eqref{exseq-norm-curv}, one obtains
\[
p_g(X) = p_a(X)-
\textstyle {\sum_{p\in \Sing(X)} \delta(p)}.
\]
\subparagraph{Example}
\label{sp:delta-sp-triple}
Locally at a space triple point, the exact sequence
\eqref{exseq-norm-curv} looks like
\begin{equation*}
\begin{matrix}
0 \to \C[x,y,z]/(xy,xz,yz)
\to &\C[x]\oplus \C[y] \oplus \C[z]
&\to &\C^2 &\to 0
\\
&(P,Q,R) &\mapsto &\bigl(P(0)-Q(0),Q(0)-R(0) \bigr)
\end{matrix}
\end{equation*}
so that a space triple point makes the genus drop by $2$.


\paragraph{Proof of the postulation formula, I}
\label{p:paS-exctseq}
Let us apply the ideas of \ref{p:pa-pg-curves}
in order to compute
the arithmetic genus of a smooth surface $S$
in terms of a general projection $S^\flat$ in $\P^3$.
Thus, $S^\flat$ has ordinary singularities as described in
\ref{p:setup-enr-dim3}, and we shall use the same notation as in
Section \ref{s:enr-dim3}.
There is an exact sequence
\begin{equation*}
\label{succ-esatta-corr}
\begin{matrix}
0 \to \O_{S ^\flat} \to \nu_*\O_{S} \to 
&\nu_* \O_{\Delta}
&\to &\O_D &\to 0,
\\
& (f_1,f_2) & \mapsto & f_1 - f_2
\end{matrix}
\end{equation*}
and it gives, taking Euler characteristics:
\begin{equation}
\label{eq:postul-pf}
p_a(S) =
p_a(S ^\flat) - p_a(\Delta) + p_a(D).
\end{equation}
Now, the arithmetic genus of $S^\flat$ is that of a degree $n$
hypersurface in $\P^3$, see \eqref{eq:pa-deg-n}, that of $\Delta$ is
$(n-4)d+1$ by \eqref{enriq4},
%{genusDelta},
and that of $D$ is $\rho+2t$ by \ref{sp:delta-sp-triple}, 
so the relation \eqref{eq:postul-pf}
gives the postulation formula \eqref{postulazione}.
\qed


\bigskip
To explain the classical definition of the arithmetic genus of a
surface, we will use the following lemma.

\begin{lemma}
\label{l:agg}
For all $i=0,1,2$, one has
$H^i(S, \omega_S)
\cong H^i(S^{\flat}, \O_{S^{\flat}}(n-4)\otimes \cI_D)$.
% \[
% H^i\bigl(S, \O_S(n-4)\otimes \cI_D\bigr)
% \cong H^i\bigl(\bar S, K_{\bar S}).
% \]
\end{lemma}

\begin{proof}
We use the relations
between the canonical line bundles of $S$, $S^\flat$, and $\P^3$, 
see \ref{p:setup-enr-dim3}. 
By the projection formula, we have
\begin{equation}
\label{proj}
\nu_* \omega_{S}
= \nu_* \bigl(
\nu^* \O_{S ^\flat}(n-4)\otimes \O_{S} (-\Delta) \bigr)
= \O_{S ^\flat}(n-4)\otimes \cI_D.
\end{equation}
Moreover one has $R^i\nu_*(\omega_{S})=0$ for all $i=1,2$,
because $\nu$ is finite,
so
$H^i(S, \omega_S) \cong H^i(S^\flat, \nu_* \omega_S)$ for all $i=0,1,2$
by Leray's spectral sequence (or merely
\cite[Exer.~III.8.1]{hartshorne-13}), and the result follows.
\end{proof}


\paragraph{Classical definition of the arithmetic genus of a surface}
\label{p:pa-classic}
Let $S$ be a smooth surface, and $S^\flat$ be a general projection of
$S$ in $\P^3$, as in \ref{p:paS-exctseq}.
By Lemma~\ref{l:agg}, one has
\begin{equation*}
p_g(S) =  
h^0(\P^3, \O_{\P^3}(n-4)\otimes \cI_D),
\end{equation*}
\ie the geometric genus of $S$ is the number of independent degree
$n-4$ hypersurfaces containing $D$; in classical words, the latter are
called degree $n-4$ hypersurfaces adjoint to $S^\flat$.
To compute this number, one may consider the restriction exact
sequence 
\begin{equation}
\label{pa-restr}
0 \to \O_{\P^3}(n-4) \otimes \cI_D
\to \O_{\P^3}(n-4)
\to \O_D(n-4) \to 0.
\end{equation}
If the linear series cut out on $D$ by $|\O_{\P^3}(n-4)|$ is complete
and non-special, one finds that
$h^0(\P^3, \O_{\P^3}(n-4)\otimes \cI_D)$ 
equals 
\begin{align}
%h^0 \bigl( \O_{\P^3}(n-4) \otimes \cI_D \bigr)
\notag
h^0 \bigl( \O_{\P^3}(n-4)\bigr) - h^0\bigl(
\O_D(n-4) \bigr)
&\textstyle = \binom {n-3} 3 
-\bigl( 1-p_a(D)+\deg \O_D(n-4)
\bigr)
\\
\label{postulation}
&= \textstyle \binom {n-3} 3 
-1 + (\rho+2t)+(n-4)d
\end{align}
(the first equality is given by the Riemann--Roch theorem, and the
second one by the computation of $p_a(D)$ in \ref{p:paS-exctseq}).
One recognizes in \eqref{postulation}
the right-hand-side of the postulation formula \eqref{postulazione}.

Classically, the arithmetic genus of $S$ is defined as the
\emph{virtual number} of independent degree
$n-4$ hypersurfaces  adjoint to $S^\flat$,
\ie the value that $h^0(\P^3, \O_{\P^3}(n-4)\otimes \cI_D)$
would assume if the linear series cut out on $D$ by
$|\O_{\P^3}(n-4)|$ were complete and non-special.\footnote
{or ``under the postulation that the linear series cut out on $D$ by
$|\O_{\P^3}(n-4)|$ is complete and non-special'',
hence the name ``postulation formula''.}
Thus, in the classical definition, the postulation formula
\eqref{postulazione} is taken as the \emph{definition}
of the arithmetic genus.

\paragraph{Equivalence of the definitions:
  proof of the postulation formula, II}
We shall now prove that the definition of the arithmetic genus given
in \ref{p:genera-defs}
is equivalent to the classical definition given above.
The matter is to prove the postulation formula, which we have already
done; we shall give another proof, based on the considerations of
\ref{p:pa-classic}.
The exact sequence \eqref{pa-restr} gives
\begin{align*}
\chi \bigl( \O_{\P^3}(n-4) \otimes \cI_D \bigr)
&= \chi \bigl( \O_{\P^3}(n-4)\bigr) - \chi \bigl(
\O_D(n-4) \bigr)
\\
&= \textstyle \binom {n-3} 3 
-1 + \rho+2t+(n-4)d,
% &= \binom {n-3} 3 
% -\bigl( 1-p_a(D)+\deg \O_D(n-4)
% \bigr)
\end{align*}
regardless of any assumption on the linear series cut out on $D$ by
$|\O_{\P^3}(n-4)|$.
Now, I claim that
\begin{equation*}
\chi \bigl( \O_{\P^3}(n-4) \otimes \cI_D \bigr)=\chi(\O_S)-1,
\end{equation*}
which will prove the equivalence of the classical and cohomological
definitions of the arithmetic genus.

To prove the claim, consider the exact sequence
\begin{equation*}
%\label{pa-restr2}
0 \to 
\omega_{\P^3} \cong \O_{\P^3}(n-4) \otimes \cI_{S ^\flat}
\to \O_{\P^3}(n-4) \otimes \cI_D
\to \O_{S ^\flat}(n-4) \otimes \cI_D \to 0,
\end{equation*}
with $\cI_{S ^\flat}$ the sheaf of ideals defining $S^\flat$ in
$\P^3$.
It implies
\begin{align*}
\chi \bigl( \O_{\P^3}(n-4) \otimes \cI_D \bigr)
% &= \chi \bigl (K_{\P^3} \bigr) + \chi \bigl( \O_S(n-4) \otimes \cI_D
% \bigr)
% \\
&= -1 + \chi \bigl( \O_S(n-4) \otimes \cI_D
\bigr).
\end{align*}
Now, one has
$\chi (S^\flat, \O_{S^\flat}(n-4) \otimes \cI_D)
= \chi( S, \omega_S)$
by Lemma \ref{l:agg}, and moreover
$\chi( S, \omega_S)
= \chi(S, \O_S)$ by Serre duality:
this proves the claim.
\qed






\subsection{The $2$-dimensional case: multiple planes}
\label{s:enriques-2dim}


In this section we consider a linear system $|V|$ on a smooth surface
$S$, of dimension $r=1$ or $2$, and we assume that
$|V|$ is a general linear subsystem of a $3$-dimensional linear system
$|V^\sharp|$ satisfying the conditions of \ref{p:setup-enr-dim3}.
In particular, this is the case if $|V|$ is a general linear subsystem
of a very ample linear system.

We shall apply the results obtained in Section \ref{s:enr-dim3} to 
$|V^\sharp|$.
We will use the notation introduced there, by taking
$S^\flat \subset \P^3$ to be
the surface defined by $|V^\sharp|$.

% For any $r \leq 3$, given the way we have set up the
% situation in \ref{p:enr-setup} we may assume that $|V|$ is a linear
% subspace of the space of hyperplane sections of a surface $S^\flat
% \subset \P^3$ as in \ref{p:setup-enr-dim3}. Equivalently, the morphism
% $S\to \P^r$ given by $|V|$ is the projection of $S^\flat$ from a
% $(3-r)$-dimensional linear subspace of $\P^3$.
% We shall thus deduce our formulas from the study carried out in
% Subsection \ref{s:enr-dim3}.

\paragraph{One-dimensional systems: proof of the Noether formula}
\label{p:enr-class}
Let $r=1$. 
We have computed the class of $|V|$ in \ref{p:enr-1dim}.
On the other hand, 
the discriminant of $|V|$ is merely the section of that of
$|V^\sharp|$ by the line $|V|$, hence the class of $|V|$ equals that of
$|V^\sharp|$, which is given in \ref{enr-formulas}.
Equating these two expressions for $\check n$, one finds
\[
c_2(S)+n+4\pi-4
= n  + 4 \pi + 12 p_a(S) - K_S^2 + 8,
\]
which is equivalent to the Noether formula, stated in \eqref{noether}.
\qed


\paragraph{}
We now let $r=2$ for the rest of this section.
Then $|V|$ defines an
$n:1$ covering $S \to \P^2$ with branch curve $B \subset \P^2$, which
may be incarnated as the projection of $S^\flat \subset \P^3$ from a
general point
$p$. 
We consider:
\begin{mycpctitem}
\item $N$ the degree of the branch curve $B \subset \P^2$~;
\item $P$ the geometric genus of $B$~;
\item $\kappa$ the number of points $q\in S$ such that there exist
  $C,C' \in |V|$ intersecting with multiplicity $\geq 3$ at $q$~;
\item $\iota$ the number of cuspidal members of $|V|$~;
\item $\delta$ the number of unordered pairs $q,q'\in S$ such that
  there exist $C,C' \in |V|$ tangent at both $q$ and $q'$~;
\item $\beta$ the number of $2$-nodal members of $|V|$.
\end{mycpctitem}
The dual of $B$ is the discriminant of $|V|$, so the class
of $B$ is $\check n$, which assumes the same value as in
\ref{p:enr-1dim} and \ref{enr-formulas}, see \ref{p:enr-class}.
Moreover, $\delta$, $\kappa$, $\beta$, $\iota$ are respectively the
numbers of nodes, cusps, bitangents, flexes of $B$.
We take once again for granted that $B$ and its dual have no other
singularities by our generality assumption.


\paragraph{Characters of the apparent boundary of $S^\flat$}
The branch curve $B$ is the image of the apparent boundary
$\appbnd p S^\flat$ by the map 
$S^\flat \to \P^2$, and in fact $\appbnd p S^\flat$ is the normalization of
$B$. 
This implies that $N$ and $P$ are respectively the degree and
genus of $\appbnd p S^\flat$, and since we have computed that its class in
$S$ is $K_S+3C$ one finds:
\begin{mycpctitem}
\item $N=(K_S+3C)\cdot C
= 2n+2\pi-2$~;
\item $P=9\pi+K_S^2-8$.
\end{mycpctitem}


\paragraph{Conclusion}
Since we know in addition the class $\check n$ of $B$, we may derive
all remaining numerical characters by applying the Pl{\"u}cker
formulae of Section \ref{s:pluecker} to $B$.
One finds:
\begin{mycpctitem}
\setlength{\itemsep}{1mm}
\item $\delta=
2\bigl[ (n+\pi)^2-5n-17\pi -2K_S^2+6p_a(S)+22
\bigr]$~;
\item $\kappa=
3 (n + 6 \pi + K_S^2 - 4 p_a(S)- 10)$~;
\item $\beta=
\frac 1 2 \bigl[
(n+4\pi-K_S^2+12p_a(S)-1)^2
+ 15 n- 6 \pi-17 K_S^2  + 132 p_a(S)  + 57
\bigr]$~;
\item $\iota=
24(\pi+p_a(S))$.
\end{mycpctitem}


\paragraph{Number of cuspidal curves in a net}
\label{p:Enriques-cusps}
It is interesting to derive the quantity $\iota$ directly by projective
methods. We end this section by sketching how this goes.
\par The parabolic curve of $S^\flat$ and the apparent boundary
$\appbnd p {S^\flat}$
intersect at the pinch points, and 
at those points $q$ on the parabolic curve such that the tangent plane
at $q$ contains $p$; 
the quantity $\iota$ is the number of points of the latter kind.

To find the intersection number of these two curves we compute
the class of the pull-back of the parabolic curve to $S$. 
The degree of the Hessian is $4(n-2)$, and a local computation shows
that its intersection with $S^\flat$
contains the double curve $D$ with multiplicity $4$.
Thus, arguing as in \ref{p:enr-1st-polars},
one finds that the pull-back of the parabolic curve has
class $4K_S+8C$.
The class of the pull-back of $\appbnd p {S^\flat}$ has been computed
in \ref{p:enr-1st-polars}.

On the other hand, we claim that the two curves intersect with
multiplicity $2$ at each pinch point. Indeed, if $q$ is a pinch point
with preimage $q' \in S$, then the members of $|V|$ passing through $q'$
form a pencil of curves which are all singular at $q'$. The condition to be
cuspidal in such a pencil is that the determinant of the $2\times 2$
matrix of second derivatives vanishes, which is a degree $2$
condition. We thus 
find $2$ cuspidal curves at $q'$ in $|V|$, hence the claim.
\par Finally, we have
\begin{equation}
(K_S+3C)\cdot(4K_S+8C)=\iota +2\tau,
\end{equation}
which indeed gives $\iota=24(\pi+p_a)$ with the expression for $\tau$
in \ref{enr-formulas}.



%\appendix
\setcounter{section}{0}
\renewcommand{\thesection}{\Alph{section}}
\renewcommand{\theparagraph}{(\Alph{section}.\arabic{paragraph})}
\renewcommand{\thesubparagraph}
{(\Alph{section}.\arabic{paragraph}.\arabic{subparagraph})}
\renewcommand{\theequation}
{\Alph{section}.\arabic{paragraph}.\arabic{subparagraph}}

\section{Polynomial calculus}
\label{S:calculus}


We give here a brief recap on polarity, together with a few facts
about the Hessian, so that the reader unfamiliar
with this may conveniently consult the relevant material. 
We refer the reader to \cite[Chapter~1]{dolgachev} and 
\cite[\S~5.4 and 5.6]{italEMS} for more details;
see also \cite{fischer}.

\subsection{Polarity}
\label{S:polarity}

\paragraph{Notation and plea for the notation}
\label{notation:polarity}
Let $\k$ be a field of characteristic zero, and let
$F \in \k[X_0,\ldots,X_n]$ be a homogeneous degree $d$ polynomial in
$n+1$ indeterminates.

For all
$\bx = (x_0,\ldots,x_n)$ and
$\by = (y_0,\ldots,y_n)$
in $\k^{n+1}$, we write
$\dD_{\bx} F$ for the differential of $F$ at the point $\bx$
(which is a linear functional on $\k^{n+1}$), and
$\dD_{\bx} F (\by)$ for the value of the latter at the vector $\by$, so
that
\begin{equation}
\label{eq:diff-2vars}
  \dD_{\bx} F (\by)
  = y_0 \, \partial_0 F (\bx) + \cdots y_n \, \partial_n F (\bx),
\end{equation}
where $\partial_i F$ is the polynomial $\partial F / \partial X_i$ for
all $i=0,\ldots,n$.

The quantity \eqref{eq:diff-2vars} is a function in the two variables
$\bx$ and $\by$, and somehow a main point in polarity theory is to
consider it as a function of the variable $\bx$ depending on the
parameter $\by$.
With this in mind we introduce the following alternative notation:
\begin{equation}
\label{eq:notation:polarity}
  \bigl( \dD^{\by} F \bigr) (\bx)
  = \bigl( \dD_{\bx} F \bigr) (\by)
  = y_0 \, \partial_0 F (\bx) + \cdots y_n \, \partial_n F (\bx).
\end{equation}
Although it may be disturbing at first,
as I have witnessed on various occasions, we shall see
that it is both meaningful and useful.
% Of course we will use the lighter
% $\dD^{\by} F (\bx)$ and
% $\dD_{\bx} F (\by)$
% instead of
% $\bigl( \dD^{\by} F \bigr) (\bx)$
% and $\bigl( \dD_{\bx} F \bigr) (\by)$
% respectively.
One could be tempted at this point to introduce $\dD _\bx ^\by F$ as
well, but let me refrain from doing this.



\paragraph{The polar pairing}
In the notation of \ref{notation:polarity} above,
for all $\bx = (x_0,\ldots,x_n) \in \k^{n+1}$,
\begin{equation}
\label{def:polar}
\dD ^\bx F =
x_0\, \partial_0 F + \cdots x_n\, \partial_n F
\in \k[X_0,\ldots,X_n]
\end{equation}
is a homogeneous polynomial of degree $d-1$ (if nonzero),
which depends linearly on $\bx$
(note that the $X_i$ are indeterminates whereas the $x_i$ are scalars).
Considering this polynomial as $(\dD^\bx) (F)$, where $\dD^\bx$
denotes the differential operator
\[
  \dD ^\bx =
  x_0 \partial_0 + \cdots x_n \partial_n,
\]
for all $\bx_1, \ldots, \bx_k \in \k^{n+1}$, we set
\begin{equation}
\label{def:polar2}
\polar {\bx_1 \cdots \bx_k} =
\polar {\bx_1} \circ \cdots \circ \polar {\bx_k}.
\end{equation}
Extending \eqref{def:polar2} by $\k$-linearity, one obtains a perfect
bilinear pairing
\begin{align*}
\Polar: \Sym^k (\k^{n+1}) \otimes \Sym^d (\check \k^{n+1})
&\longrightarrow \Sym ^{d-k} (\check \k^{n+1})
\\
\sum\nolimits_{i,j} \Xi_i \otimes F_j 
&\longmapsto
\sum\nolimits_{i,j} \polar {\Xi_i} F_j
\end{align*}
extending the natural pairing between $\k^{n+1}$ and
its dual $\check \k^{n+1}$.


\paragraph{The Taylor--Newton formula}
\label{p:Taylor-Newton}
In the formalism of polarity it has the following pleasant
incarnation.
Let $\bx = (x_0,\ldots,x_n)$ and
$\by = (y_0,\ldots,y_n)$ be in $\k^{n+1}$. As above, $F$ is a degree
$d$ polynomial.
One has:
\begin{align*}
  F(\bx+\by)
  &= \sum _{k=0} ^d \ 
    \sum_{k_0 + \cdots + k_n = k} \,
    \frac 1 {k_0! \cdots k_n!} \,
    y_0^{k_0} \cdots y_n ^{k_n} \,
    \biggl(
    \frac {\partial^{k_0}} {\partial X_0^{k_0}}
    \cdots
    \frac {\partial^{k_n}} {\partial X_n^{k_n}}
    F
    \biggr)
    (\bx)
  \\
  &= \sum _{k=0} ^d \,
    \frac 1 {k!} \,
    \biggl(
    \Bigl(
    y_0\, \frac {\partial} {\partial X_0}
    + \cdots +
    y_n\, \frac {\partial} {\partial X_n}
    \Bigr) ^k
    F
    \biggr)
    (\bx)
  \\
  &= \sum _{k=0} ^d \,
    \frac 1 {k!} \,
    \polar {\by^k} F (\bx).
\end{align*}


\paragraph{Polar hypersurfaces}
Consider the hypersurface $Z = V(F) \subset \P^n$.
For $\hat a=(a_0,\ldots,a_n)$
and $\bx = (x_0,\ldots,x_n)$ in $\k^{n+1}$, and $k\in \N$, 
\[
\polar {\hat a^k} F (\bx) = 
\bigl( ( a_0 \partial_0 + \cdots + a_n \partial_n )^k F \bigr) (\bx)
\]
is a bihomogeneous polynomial of bidegree $(k,d-k)$
in the variables $(a_0,\ldots,a_n)$ and $(x_0,\ldots,x_n)$. 
The hypersurface $V(\polar {\hat a^k} F)$
depends only on $Z$ and the point $a= (a_0:\ldots:a_n)\in \P^n$,
see \cite[Thm.~5.4.2]{italEMS}: we
call it the \emph{$k$-th polar of $Z$ with respect to $a$}, and denote
it by $\polar {a^k} Z$.
It is a degree $d-k$ hypersurface.
We will often abuse notation and omit the distinction between $\hat a$
and $a$.
In addition, we will call $V(\polar {\hat a^k} F)$ a hypersurface even
when $\polar {\hat a^k} F = 0$, and thus $V(\polar {\hat a^k} F) = \P^n$.

We shall also use the following notion:
the \emph{polar $k$-ic of $Z$ at $a$},
denoted by $\dD _{a^k} Z$,
is the degree $k$ hypersurface defined by the polynomial
\[
\dD ^{\bx^k} F(\hat a) =
\bigl( ( x_0 \partial_0 + \cdots + x_n \partial_n )^k F \bigr) (\hat a)
\]
in the variables $(x_0,\ldots, x_n)$.\footnote
{to avoid possible confusion, let me take the risk of being pedantic:
  consider $F$ as a polynomial in the indeterminates $Y_0,\ldots,Y_n$,
  and let $X_0,\ldots,X_n$ be a second set of indeterminates;
  then, specializing the polynomial
  $\bigl(
  X_0\, \frac {\partial} {\partial Y_0}
  + \cdots +
  X_n\, \frac {\partial} {\partial Y_n}
  \bigr)^k F(Y_0,\ldots,Y_n)$
  by specializing $Y_i$ to $a_i$ for all $i$,
  one obtains a polynomial in the indeterminates  $X_0,\ldots,X_n$:
  this is the defining equation of $\dD _{a^k} Z$.
}
In other words, we interchange the roles of $\hat a$ and $\bx$ when we
pass from  
$\polar {a^k} Z$ to $\dD _{a^k} Z$;
thus, by definition, for all $a,b \in \P^n$,
\begin{equation}
\label{kth-polar-vs-polar-kic}
  b\in \dD_{a^{k}}Z
  \quad \iff
  \quad
  a \in \dD^{b^k}Z.
\end{equation}

\begin{proposition}[polar symmetry]
Consider a degree $d$ hypersurface $Z \subset \P^n$.
Let $a, b \in \P^n$, and $k \in \intint 1 {d-1}$.
One has the equivalence:
\[
a\in \polar {b^{k}} Z
\ \iff \
b\in \polar {a^{d-k}} Z.
\]
%\negvcorr
\end{proposition}
%\vspace{\mnegvcorr}


\noindent
In particular this says that the polar $k$-ic at $a$
(\ie $\dD _{a^k} Z$)
coincides with
the $d-k$-th polar with respect to $a$
(\ie $\polar {a^{d-k}} Z$).

\begin{proof}
Let $F$ be a homogeneous polynomial defining the hypersurface $Z$.
Consider two sets of $n+1$ indeterminates $\bX = (X_0,\ldots,X_n)$
and $\bY=(Y_0,\ldots,Y_n)$.
By the Taylor--Newton Formula we have
\begin{equation*}
  F(\bX+\bY)
  = \sum _{k=0} ^d \,
  \frac 1 {k!} \,
    \bigl( \polar {\bY^k} F \bigr) (\bX)
  \quad
  = \quad
  F(\bY+\bX)
  = \sum _{k=0} ^d \,
  \frac 1 {k!} \,
  \bigl( \polar {\bX^k} F \bigr) (\bY).
\end{equation*}
Identifying the degree $k$ pieces in the indeterminates $\bX$, we find
\begin{equation*}
  \frac 1 {(d-k)!} \polar {\bY^{d-k}} F (\bX)
  \ =\  \frac 1 {k!} \polar {\bX^k} F (\bY),
\end{equation*}
which gives the result at once.
\end{proof}



% It follows from the Euler formula that if $a \in Z$, then $a \in \polar
% {a^k} Z$ for all $k \geq 1$. Also the converse holds, as follows.
% an elementary
% computation shows (see \cite[Prop.~5.4.3]{italEMS}.

\begin{proposition}
\label{p:polar-self-conjug}
Let $Z$ be a degree $d$ hypersurface in $\P^n$.
For all $a \in \P^n$ and
$k=1,\ldots,d-1$, one has:
\[
a \in Z
\iff
a \in \polar {a^k} Z.
\]
\end{proposition}
%\negvcorr\negvcorr

\begin{proof}
Let $F$ be an equation of $Z$.
One has
$\polar {a^k}F(a)= d(d-1)\cdots (d-k+1) F(a)$
by the Euler formula.
\end{proof}


\paragraph{}
If $b \in Z=V(F)$ is a smooth point, then 
$\bigl(\dD_b F\bigr)(\bX) = \bigl(\dD^{\bX} F\bigr)(b)$
is a linear homogeneous polynomial
defining the tangent hyperplane to $Z$
at $b$,
hence polar hyperplane $D_bZ$ is the tangent hyperplane to
$Z$ at $b$, and moreover, for all $a \in \P^n$,
\begin{equation*}
Z_\sm \cap \polar a Z =
\{ b\in Z_\sm : \T_bZ \ni a \},
\end{equation*}
where $Z_\sm$ denotes the smooth locus of $Z$.
This generalizes to the following fundamental property.

For all hypersurfaces $Z \subset \P^n$ and lines $\ell \subset \P^n$,
and for all $p \in \ell$, we let $i(Z,\ell)_p$ be the multiplicity with
which $p$ appears in $Z \cap \ell$.

\begin{theorem}
\label{t:polars-tglines}
% [Dolgachev, (1.19) p.13
% pas besoin que a soit un point non-singulier
Let $Z$ be a degree $d$ hypersurface, $a \in Z$,
and $b \in \P^n$. For all integer $s\geq 0$, one has
\begin{align*}
i \bigl( Z,\vect{a,b} \bigr)_a \geqslant s+1 \quad
& \iff \quad \forall k=1,\ldots, s,\quad b\in \dD_{a^{k}}Z \\
& \iff \quad \forall k=1,\ldots, s,\quad a\in \dD^{b^{k}}Z.
\end{align*}
\end{theorem}

\begin{proof}
Let $F$ be a homogeneous equation for $Z$, and let
$\hat a, \hat b \in \k^{n+1}$.
Consider an indeterminate $T$. We have
\[
  F(\hat a+T \hat b)
  = \sum _{k=0} ^d \,
  \frac 1 {k!} \,
  \bigl( \polar {(T\hat b)^k} F \bigr) (\hat a)
  = \sum _{k=0} ^d \,
  \frac 1 {k!} \,
  \bigl( \polar {\hat b^k} F \bigr) (\hat a)\cdot T^k
\]
by the Taylor--Newton formula.
This gives the result since, by definition,
$i \bigl( Z,\vect{a,b} \bigr)_a \geqslant s+1$
if and only if
$T^{s+1}$ divides $F(\hat a+T \hat b)$
(note that $\polar {\hat b^0} F (\hat a) = F(\hat a) = 0$ by
hypothesis). 
\end{proof}

It turns out that for $a \in Z$, all polars of $Z$ with respect to $a$
(equivalently, all polar hypersurfaces $\dD _{a^k} Z$ at $a$)
are tangent at $a$. Actually, $Z$ and its polar $k$-ic at $a$, 
$\dD _{a^k} Z$ have the same polar $s$-ics at $a$ for all $s\leq k$,
as the following identities show.
Let $d=\deg (Z)$. Using polar symmetry repeatedly, one finds
\[
\dD _{a^s} \bigl(\dD_{a^k}Z \bigr)
= \polar {a^{k-s}} \bigl(\dD _{a^k} Z \bigr)
= \polar {a^{k-s}} \bigl( \polar {a^{d-k}} Z \bigr)
= \polar {a^{d-s}} Z
= \dD _{a^s} Z.
\]
This has the following remarkable consequence.

\begin{corollary}
\label{c:inters-polars}
Let $Z$ be a hypersurface in $\P^n$, and $a$ be a point of $Z$.
The $n$ hypersurfaces 
$\dD _{a} Z, \ldots, \dD _{a^n} Z$
intersect with multiplicity at least $n!$ at $a$
(with the convention that the multiplicity is infinite if the
intersection is positive dimensional at $a$).
\end{corollary}

\begin{proof}
We consider only the case in which $\dD _{a} Z, \ldots, \dD _{a^n} Z$
define a local complete intersection at $a$,
otherwise the result is trivial.
Then the intersection $\dD _{a} Z, \ldots, \dD _{a^{n-1}} Z$
consists of $(n-1)!$ lines each intersecting $Z$ with multiplicity at
least $n$ at $a$, as follows from Theorem~\ref{t:polars-tglines}.
Since the polar $k$-ics at $a$ of $\dD _{a^{n}} Z$ are the same as those
of $Z$, as indicated above, each of these lines also intersect
$\dD _{a^{n}} Z$ with multiplicity at least $n$ at $a$, 
and the result follows.
\end{proof}


The polar hyperplane $\dD _{a} Z$ is indeed a hyperplane only if $a$
is a smooth point of $Z$, and then it is properly the tangent
hyperplane to $Z$ at $a$,
otherwise $\dD _{a} Z$ is the whole $\P^n$.
The following result generalizes this:
by \ref{t:pol-sing1}, if $Z$ has multiplicity exactly $m$ at $a$,
then $\dD _{a^m} Z$ coincides with the tangent cone $\TC_a (Z)$.


\begin{theorem}
\label{t:pol-sing}
% [Dolgachev, Prop. 1.1.7 p.8]
Let $Z$ be a degree $d$ hypersurface, and $a$ be a
point of $Z$ of multiplicity $m$. Consider an integer
$r\leq d$.
\subparagraph{}\label{t:pol-sing1}
The polar $r$-ic at $a$,
$\dD_{a^r}Z$,
is the whole $\P^n$
if and only if $r < m$.
If $r \geq m$, then $\dD_{a^r}Z$
has multiplicity $m$ at $a$, 
and it has the same tangent cone as $Z$ at $a$:
$\TC_a (\dD_{a^r}Z) = \TC_a (Z)$.
\subparagraph{}\label{t:pol-sing2}
Let $b \in \P^n -\{a\}$.
If $r < m$,
the $r$-th polar with respect to $b$,
$\polar {b^r} Z$, has multiplicity at least
$m-r$ at $a$;
the multiplicity is exactly $m-r$ if $b$ is general, and in
this case
the tangent cone of $\polar {b^r} Z$ at $a$ 
equals the
$r$-th polar with respect to $b$ of the tangent cone
$\TC_a(Z)$:
$\TC_a\bigl(\polar {b^r} Z \bigr)
= \polar {b^r} {\bigl(\TC_a(Z)\bigr)}$.
% \[
% \TC_a\bigl(\polar {b^r} Z \bigr)
% = \polar {b^r} {\bigl(\TC_a(Z)\bigr)}.
% \] 
%\negvcorr
\end{theorem}
%\vspace{\mnegvcorr}

\noindent
Note that
\ref{t:pol-sing2} tells us that
$\polar {b^r} Z$ contains $a$ if $r \leqslant m-1$, and is
singular at $a$ if $r \leqslant m-2$.

% Also the following holds. Let $k, l$ be positive integers such that 
% $k+l < d$.
% If $a$ is a point of multiplicity $\geq d-k-l+1$ of 
% $\polar {b^l} Z$, then $b$ is a point of multiplicity $\geq d-k-l+1$
% of $\polar {a^k} Z$.

% The proof consists of an elementary calculation, see
% \cite[Proposition~1.1.7]{dolgachev}.

\begin{proof}
Let us assume, without loss of generality, that
$a=(1\:0\! :\ldots :\!0)$. Then
\[
  F = X_0^{d-m} F_m(X_1,\ldots,X_n)
  + \cdots + F_d(X_1,\ldots,X_n)
\]
where each $F_k$ is homogeneous of degree $k$,
and $F_m$ is non-zero.
One has $\dD_{a^r}Z = \polar {a^{d-r}} Z$ by polar symmetry, and
$\dD ^{a^{d-r}} = (\partial/\partial X_0)^{{d-r}}$,
hence $\dD_{a^r}Z$ is defined by the equation
\[
  \bigl( \tfrac {\partial} {\partial X_0} \bigr)^{{d-r}} F
  = \tfrac {(d-m)!} {(r-m)!} X_0^{r-m} F_m
  + \cdots +
  \tfrac {(d-r)!} {0!}  F_r;
\]
it is zero if and only if $r<m$, and if $r\geq m$ we see that
$\dD_{a^r}Z$ has multiplicity $m$ at $a$ with tangent cone defined by
$F_m$, which proves \ref{t:pol-sing1}.

Now let $b=(b_0,b_1,\ldots,b_n)$ be such that the corresponding point in
$\P^n$ is distinct from $a$. We set $b^\natural = (0,b_1,\ldots,b_n)$
(it is non-zero because $b$ and $a$ are distinct in $\P^n$),
and $b^r = (b^\natural)^r + \Xi$.
Then $\dD^{b^r} = \dD^{(b^\natural)^r} + \dD^\Xi$, where $\dD^{(b^\natural)^r}$ is
a polynomial in $\partial/\partial X_1,\ldots,\partial/\partial X_n$
only, while $\dD^\Xi$ is a polynomial in $\partial/\partial X_0,
\partial/\partial X_1,\ldots,\partial/\partial X_n$ in which all terms
involve $\partial/\partial X_0$ with a positive exponent.
Therefore, the piece of $\dD^{b^r}F$ with the highest degree in $X_0$
is
\[
  \dD^{(b^\natural)^r}(X_0^{d-m}F_m)
  = X_0^{d-m}\, \dD^{(b^\natural)^r}(F_m)
  = X_0^{d-m}\, \dD^{b^r}(F_m).
\]
It follows that $\dD^{b^r} Z$ has multiplicity at least
$m-r$ at $a$; this multiplicity is exactly $m-r$ if and only if 
$\dD^{b^r}(F_m)$ is non-zero, and in this case $\dD^{b^r}(F_m)$
defines the tangent cone of $\dD^{b^r} Z$ at $a$, so that the latter
equals $\polar {b^r} {(\TC_a(Z))}$.
Now $\dD^{b^r} (F_m) = \dD^{(b^\natural)^r} (F_m)$ is non-zero for
general $b$, and \ref{t:pol-sing2} is proven.
\end{proof}


\subsection{Hessian and second fundamental form}
\label{app:hess}


Let $Z$ be a hypersurface in $\P^n$, defined by the homogeneous
polynomial $F \in \k[X_0,\ldots,X_n]$. 


\paragraph{Hessian of a hypersurface}
\label{p:hessian}
The \emph{Hessian hypersurface} of $Z$ is
the hypersurface $\Hess(Z)$ defined by the homogeneous polynomial
\[
\Hess(F) = \det \bigl( \d i \d j F \bigr)
_{0 \leq i,j \leq n}.
\]
It has degree $(n+1)(n-2)$ (if non-zero).

Using the Euler formula and the standard properties of determinants,
one may obtain the alternative expression
\begin{equation}
\label{eq:hess-alt}
\Hess(F)=
\textstyle{\frac{(d-1)^2}{X_0^2}}
%\left| \begin{array}{cccc}
\begin{vmatrix}
\frac{d}{d-1}\cdot F & \partial_{1} F & \cdots & \partial_{n} F \\
\partial_{1} F & \partial_{1}^2 F & \cdots
& \partial_{1} \partial_{n} F \\ 
\vdots & \vdots & \ddots & \vdots \\
\partial_{n} F & \partial_{1} \partial_{n} F & \cdots
& \partial_{n}^2 F
\end{vmatrix},
%\end{array} \right|.
\end{equation}
which is useful to study the intersection of $Z$ and $\Hess(Z)$.



\paragraph{Second fundamental form}
\label{p:IIform}
Let $p$ be a smooth point of $Z$.
The \emph{second fundamental form} of $Z$ at $p$, denoted by
$\II_p$, is a quadric
in the tangent space $T_pZ$ which is defined as follows.
Analytically locally around $p$, and in an affine chart
in which we identify $p$ with $(0,\ldots,0)$ and
$T_pZ$ with $\A^{n-1}\times\0$,
$Z$ is the image of a map
\[
  \varphi:
  (u_1,\ldots,u_{n-1}) \mapsto
  \bigl(
  u_1,\ldots,u_{n-1},\varphi(u_1,\ldots,u_{n-1})
  \bigr)
\]
defined on a neighbourhood of the origin in the tangent
space $T_pZ$, such that the order $0$ and order $1$ terms in the Taylor
expansion of $\varphi$ vanish.
The second fundamental form is the order $2$ term of the Taylor
expansion of $\varphi$ modulo multiplication by a non-zero scalar;
it does not depend on the choice of the
parametrization.


\paragraph{Local forms}
\label{p:Hess-II}
Assume $F$ is in the form
\[
  X_0^{d-1}X_n
  +X_0^{d-2} \Bigl(
  \sum_{1\leq i,j \leq n} a_{ij}X_iX_j
  \Bigr)
  + O(3),
\]
so that $p=(1:0:\ldots:0) \in Z$, and $\T_pZ = \{X_n=0\}$.
We assume that the matrix $(a_{ij})_{1\leq i,j \leq n}$ is symmetric.
By computing the first terms of the Taylor expansion of
\[
  F\bigl(
  1,u_1,\ldots,u_{n-1},\varphi(u_1,\ldots,u_{n-1})
  \bigr),
\]
one sees that the second fundamental form of $Z$ at $p$ is the
quadratic form on $T_pZ \simeq \C^{n-1}$ defined by the symmetric
matrix  $(a_{ij})_{1\leq i,j \leq n-1}$, modulo scalar multiplication.

Now let us show the relation between the determinant of this matrix
and the Hessian determinant. We will assume $n=3$ in order to have
smaller matrices, but it is straightforward to do the same computation
for arbitrary $n$.
By direct computation, one finds that the Hessian determinant of $F$
at $p=(1:0:0:0)$
is
\[
  \begin{vmatrix}
    0 & 0 & 0 & d-1 \\
    0 & 2a_{11} & 2a_{12} & 2a_{13} \\
    0 & 2a_{12} & 2a_{22} & 2a_{23} \\
    d-1 & 2a_{13} & 2a_{23} & 2a_{33}
  \end{vmatrix}
  =
  \begin{vmatrix}
    0 & d-1 \\
    d-1 & 2a_{33}
  \end{vmatrix}
  \cdot
  \begin{vmatrix}
    2a_{11} & 2a_{12} \\
    2a_{12} & 2a_{22} 
  \end{vmatrix}.
\]

\begin{corollary}
The second fundamental form at $p$ is non-degenerate if and only if
the Hessian determinant is non-zero.
\end{corollary}


\paragraph{Second fundamental form and polar quadric}
Still in the notation of \ref{p:Hess-II} above, the polar quadric of
$Z$ at $p$, $\dD_{p^2}Z$, is defined by the equation
\[
  \dD^{p^{d-2}} F
  = \bigl( \tfrac{\partial}{\partial X_0} \bigr)^{d-2} F
  \,=\, \tfrac {(d-1)!}{1!} X_0X_n
  + \tfrac {(d-2)!}{0!}\,
  \Bigl(
  \sum_{1\leq i,j \leq n} a_{ij}X_iX_j
  \Bigr).
\]
We thus see that the intersection of the polar quadric $\dD_{p^2}Z$
with the projective tangent hyperplane $\T_pZ = V(X_n)$ is the projective
completion of the second fundamental form $\II_p$.

Note that $\II_p$ is an affine quadric in $T_pZ$ which is defined by a
homogenous degree $2$ polynomial, hence it is singular at the
origin, \ie at $p$. On the other hand, we have seen
in Theorem \ref{t:pol-sing}
that $\T_pZ = \T_p (\dD_{p^2}Z)$,
which explains why  $\dD_{p^2}Z \cap \T_pZ$ is singular at $p$.


\section{Developable surfaces}
\label{ap:dev}

In this appendix we review the basic theory of developable surfaces in
the projective space of dimension $3$,
following
the beautiful \cite[Chap.~V]{edge}.

\subsection{Synthetic description}
\label{s:dev-synth}

\paragraph{Definition}
A \emph{developable surface} $S \subset \P^3$ is a ruled surface such that
the tangent plane to $S$ is constant along the lines of the
ruling. In other words, for all lines $\Lambda$ of the ruling, and for
all $p,p' \in \Lambda$, one has $\T_pS = \T _{p'} S$.
An important aspect of developable surfaces is that they are the
surfaces that can be unfolded into the plane with no distortion; we
will however not consider this idea any farther in this text.
\par
In classical terminology, if $S$ is a ruled surface, the lines of the
rulings are called 
\emph{generators}, and a generator $\Lambda$ is said 
to be \emph{torsal} if the tangent plane to $S$ is constant along
$\Lambda$. Thus developable surfaces are those ruled surfaces for
which all generators are torsal.

\paragraph{}
\label{p:devel-defect}
Developable surfaces in $\P^3$ are exactly those 
surfaces in $\P^3$ that have their dual which is not a hypersurface,
see \cite[Thm.~1.18]{tevelev}.
It therefore follows from biduality that any non-degenerate
developable surface is projective dual to a curve $C$ in $\check\P^3$.
In particular it has an ordinary double curve, corresponding to
bitangent planes to $C$, and a cuspidal double curve, corresponding to
osculating planes to $C$
(unless $C$ is degenerate, in which case $S$ is a cone).
% \par
% (We say that a plane $H$ is bitangent [resp.\ osculating] to $C$ if
% the intersection cycle $H\cap C$ contains a subcycle of the form
% $2p+2q$ [resp.\ $3p$], $p,q \in C$).
\par
This description may be refined as follows.


\paragraph{}
\label{p:devel-bidual}
The following fact refines the description of \ref{p:devel-defect};
for a proof,
see \cite[Section 0.5]{fischer-piontkowski},
or \cite[5.8.14]{italEMS}.
Also \cite[\S 30]{anschau} is very enlightening.
Let $S$ be a developable surface in $\P^3$.
On every generator there is a
singular point at which $S$ does not have a well-defined
tangent plane
(beware that there are other singular points as well, see
Proposition \ref{c:deg-double-curv-dev}). 
If $S$ is not a cone, the locus of the singular
points on the various generators is a curve $\Gamma$, called
the \emph{regression edge}, which is none other than the cuspidal
double curve of $\dual C$ mentioned in \ref{p:devel-defect}.
At a general point $p \in \Gamma$, the tangent line
$\T_p\Gamma$ is the generator of $S$ through $p$, and the osculating
plane 
$\Osc_p\Gamma$ is the plane tangent to $S$ along the generator
$\T_p\Gamma$. 

This tells us that $S$ is the \emph{tangential surface} of $\Gamma$,
namely 
\[
S 
= \Tan (\Gamma) 
:= \overline{
\bigcup\nolimits _{p \in \Gamma_\sm} \T_p\Gamma
}.
\]
Moreover, the curve $C=\dual S \subset \check\P^3$ is what I call the
\emph{oscdual}\footnote
{Piene has introduced, more generally, the concept of $m$-dual
varieties in \cite{piene-higherorder}; in her notation, the oscdual of
$\Gamma$ is the $2$-dual variety $\dual \Gamma_2$.
See also Pohl's \cite{pohl}.}
curve of $\Gamma \subset \P^3$, namely
\[
C=
\overline{
\bigcup\nolimits _{p \in \Gamma^\zero} \orth {(\Osc_p\Gamma)}
},
\]
where $\Gamma^\zero$ denotes the open subset of $\Gamma$ of points $p$ such
that $\Osc_p\Gamma$ is a plane, \ie $\Gamma$ and $\T_p\Gamma$
intersect with multiplicity exactly $2$ at $p$.

The dual of $\Gamma$ is a developable surface in $\check \P^3$, the
generators of which are the lines
$\orth {\T_p\Gamma}$ for all smooth points $p \in \Gamma$.
It follows from biduality and the above description that this is the
tangential surface of the curve $C$.
In particular, $\Gamma$ is the oscdual curve of $C$: this is a
reflexivity statement for oscduality.


\paragraph{}
While we shall not prove here that a developable surface in $\P^3$ is
either a cone or the tangential surface $\Tan(\Gamma)$ of a curve, it
is easy and instructive to see why tangential surfaces are
developable.  Assume $\Gamma$ is parametrized locally by a map
$\phi: u \mapsto \smash{\bigl(\alpha(u), \beta(u), \gamma(u) \bigr)}$
in some affine chart of $\P^3$.
Then $\Tan(\Gamma)$ is parametrized locally by
\[
  \Phi:
  (u,s) \,\longmapsto\,
  \begin{pmatrix}
    \alpha(u) \\ \beta(u) \\ \gamma(u)
  \end{pmatrix}
  + s
  \begin{pmatrix}
    \alpha'(u) \\ \beta'(u) \\ \gamma'(u)
  \end{pmatrix},
\]
and the differential of this parametrization at the point $(u_0,s_0)$ is
determined by
\[
  \frac {\partial}{\partial u} \,\longmapsto\,
  \begin{pmatrix}
    \alpha'(u_0) \\ \beta'(u_0) \\ \gamma'(u_0)
  \end{pmatrix}
  + s_0
  \begin{pmatrix}
    \alpha''(u_0) \\ \beta''(u_0) \\ \gamma''(u_0)
  \end{pmatrix}
  \Et
  \frac {\partial}{\partial s} \,\longmapsto\,
  \begin{pmatrix}
    \alpha'(u_0) \\ \beta'(u_0) \\ \gamma'(u_0)
  \end{pmatrix}.
\]
We thus see that,
if $\Gamma$ doesn't have an inflectionary behaviour at the point
$\phi(u_0)$, the differential of $\Phi$ fails to be of maximal rank if
and only if $s_0=0$, and otherwise its image is constant as $s_0$
moves, equal to the plane spanned by $\phi'(u_0)$ and $\phi''(u_0)$.
The upshot is that the tangent plane to $\Tan(\Gamma)$ is constant
along its generator $\T_{\phi(u_0)}\Gamma$, equal to the osculating
plane $\Osc_{\phi(u_0)}\Gamma$, except at the very point $\phi(u_0)$
where it is not well-defined, and thus $\Gamma$ is a cuspidal curve of
$\Tan(\Gamma)$.


\paragraph{}
\label{p:hess-dev}
Finally, although we shall not use it,
note that developable surfaces are characterized by the property that
they are contained in the zero locus of their associated Hessian
determinant. 
This is an instance of a result valid for hypersurfaces of any
dimension, which has been proved by B.~Segre
\cite{bsegre-bertiniforms}; see also
\cite[Lemma 7.2.7]{russo} for a proof attributed to Koll\'ar by the
author.



\subsection{Analysis of contacts}
\label{s:edge}

We carry on our analysis of developable surfaces, building upon the
description given in the previous section, and following the
general philosophy of biduality.
Recall that
$S = \Tan(\Gamma) \subset \P^3$ is the tangential surface of the curve
$\Gamma \subset \P^3$, and $C= \dual S \subset \P^3$ is the dual curve
of the developable surface $S$, as well as the oscdual of $\Gamma$.
We leave aside for the moment the
peculiar behaviour that the curve $\Gamma \subset \P^3$ may have at
isolated points in some special situations.

\paragraph{Characteristic numbers, I}
\label{p:not-char-dev-I}
We let:
\begin{mycpctitem}
\item $m = \deg \Gamma$~;
\item $n= \deg C$~;
\item $r= \deg  \bigl(\Tan (\Gamma)\bigr)$.
\end{mycpctitem}
\par
Classically, developable surfaces were considered as systems
packaging together three $1$-dimensional families in $\P^3$ of planes,
points, and lines respectively;
these are the planes para\-met\-rized by points of $C$, the points of
$\Gamma$, and the tangent lines of $\Gamma$.
In this perspective, $m$
is the number of points
of the system
contained in a general plane of $\P^3$,
$n$ is the number of planes of the system passing through a general
point of $\P^3$,
and $r$ is the number of lines of the system meeting a general line of
$\P^3$. 
The integers $m,n,r$ are called respectively the order, class, and
rank of the system.

\paragraph{}
\label{p:inters-infnear-planes}
Knowing the family of planes given by $C \subset \check \P^3$, one may
find the generators of the developable surface $\Tan(\Gamma) \subset
\P^3$ by taking the intersections in $\P^3$ of pairs of infinitely
near members of $C$.
\par
Indeed, the generators of $\Tan(\Gamma)$ are the orthogonals of the
tangent lines of $C$. Now for $p,q \in C$, the orthogonal of the line
$\vect{p,q} \subset \check \P^3$ is the intersection of the two planes 
$\orth p$ and $\orth q$ in $\P^3$. Letting $q$ tend to $p$ yields the
asserted statement.


\paragraph{}
Let $o$ and $H$ be a general point and a general plane in $\P^3$. The
duality between projections and hyperplanes sections (see
Proposition \ref{prop:dual-sec-proj})
% \cite[Thm.~1.21]{tevelev}
tells us that the projection
of $\Gamma$ from $o$ is dual as a plane curve to the hyperplane
section of $\dual \Gamma = \Tan(C)$ by $\orth o$ and,
dually, that the section of $S=\Tan(\Gamma)$ by $H$ is dual to the
projection of $C$ from the point $\orth H$.
This may be established using the following elementary statement,
see Proposition \ref{pr:proj-sec}.

\begin{lemma}
\label{l:proj-spcurv}
Let $o \in \P^3$ be a point off $\Gamma$, and consider the
projection 
$\pi_o: \P^3 \dashrightarrow \P^3/o$.
Let $p\in \Gamma$ be a smooth point
such that the line $\vect {o,p}$ intersects $\Gamma$
only at $p$.
\setlength{\parindent}{0mm}
\begin{asparaenum}[\normalfont (i)]
\item 
If the line $\vect {o,p}$ is tangent to $\Gamma$ at $p$,
then the projected curve $\pi_o(\Gamma)$ has a cusp at
$\pi_o(p)$.
\item
If the line $\vect {o,p}$ is not tangent to $\Gamma$ at $p$,
there is a unique plane $H$ containing $o$ and tangent to $\Gamma$ at
$p$, and its projection $\pi_o(H)$ is the tangent line to
$\pi_o(\Gamma)$ at $\pi_o(p)$.
If $H$ osculates $\Gamma$ to the order at least $3$, then 
$\pi_o(H)$ is a flex tangent.
\end{asparaenum}
\end{lemma}

This lemma
is pretty clear from the differential point of view, given that
the kernel of the differential of $\pi_o$ at the point $p$ is the
tangent direction of the line $\vect {o,p}$.

Another interesting interpretation of this result is in terms of
intersection multiplicities. Call $\Gamma'=\pi_o(\Gamma)$,
$p'=\pi_o(p)$, and
$H'=\pi_o(H)$, assuming that $H$ is a hyperplane in $\P^3$ containing
$p$, so that $H'$ is a line in $\P^2$.
Then, for local intersection multiplicities at $p$ and $p'$, the
projection formula tells us that
\[
  (H\cdot \Gamma)_p
  = (H'\cdot \Gamma')_{p'}.
\]
Thus, if $H$ is an ordinary (resp. osculating) tangent plane of
$\Gamma$ at $p$, then $H'$ is an ordinary (resp. flex) tangent of
$\Gamma'$ at $p'$.
Moreover, if the line $\vect{o,p}$ is tangent to $\Gamma$ at $p$,
then for all planes $H$ passing through $o$ and $p$ one has 
$(H\cdot \Gamma)_p >1$, hence $(H'\cdot \Gamma')_{p'}>1$ for all lines
passing through $p'$: this implies that $\Gamma'$ is singular at $p'$,
and it has a cusp there because it is unibranch, as follows from our
assumption that $\vect {o,p}$ intersects $\Gamma$
only at $p$.

Finally, the lemma may also be proved by local computations. Let me
now give a sample of these.
Assume $p=(1:0:0:0)$ and $\Gamma$ is parametrized locally at $p$ by
$t \mapsto (1:t:t^2:t^{3+k})$ for some non-negative integer $k$.
Let $o=(a:b:c:d)$, and assume that $b\neq 0$
(the other possibilities may be considered analogously).
Then the projection from $o$ writes
\[
  (x:y:z:w) \mapsto
  (x-\tfrac a b y: z-\tfrac c b y: w -\tfrac d b y),
\]
so that $\Gamma' = \pi_o(\Gamma)$ is locally parametrized at
$p'=\pi_o(p)$ by
\[
  t \mapsto
  \Bigl(1:
  \frac {t^2-\tfrac c b t} {1-\tfrac a b t}:
  \frac {t^{3+k} -\tfrac d b t} {1-\tfrac a b t}
  \Bigr).
\]
If $d=0$,
then $o$ sits on the osculating plane of $\Gamma$ at $p$.
If moreover $c\neq 0$, then $\Gamma'$ has a local parametrization at
$p'$ of the form
$t \mapsto (1:-\tfrac c b t + \sum_{m\geq 2} \alpha_m t^m:
t^{3+k} + \sum_{m\geq 4+k} \beta_m t^m)$,
hence it has a flex at $p'$.
If $d=c=0$,
then $o$ sits on the tangent line to $\Gamma$ at $p$, and the local
parametrization shows that $\Gamma'$ has cusp at $p'$:
an ordinary cusp (\ie an $A_2$ double point) if $k=0$,
a ramphoid cusp (\ie an $A_4$ double point) if $k=1$,
and so on.

% Part (i) tells us that when we project from a point $o$ off
% $\Tan(\Gamma)$, the number of flex points of $\pi_o(\Gamma)$ is the
% degree $n$ of the osc-dual curve $C$, or equivalently the class of the
% developable surface $\Tan(\Gamma)$.

\paragraph{}
\label{com:proj-spcurv}
If we project a smooth curve $\Gamma \subset \P^3$ from a general
point $o$, its image is a plane nodal curve $\Gamma'$, and the nodes
correspond to the finitely many secant lines of $\Gamma$
(\ie lines of the form $\vect {p,q}$ with $p,q\in \Gamma$)
passing through $o$.\footnote
{see \cite[IV, Theorem 3.10]{hartshorne-13} for a complete proof,
and \cite{gruson-peskine} for a vast generalization.}
The projection $\Gamma'$ has moreover finitely
many flexes (in addition to the original flexes of $\Gamma$),
corresponding to the finitely many osculating hyperplanes of $\Gamma$
passing through $o$
(\ie to the finitely intersection points of the oscdual curve
$C = \dual {\Tan(\Gamma)}$ with the hyperplane $\orth o$).

Assume now that we project from a general point $o$ of the tangential
surface $\Tan(\Gamma)$.
Then the projection $\Gamma'$ has one cusp, corresponding to the
unique generator of $\Tan(\Gamma)$ passing through $o$,
and one less node than in the general situation, because the geometric
genus of $\Gamma'$ must always be the same as that of $\Gamma$
(another interpretation of this is that one of the secant lines
of $\Gamma$ in the general situation has become a tangent line in the
present situation).
This implies in particular that the class of the plane curve $\Gamma'$
in the present situation is one less than in the general situation,
by the Plücker formula $(P_1)$, see \ref{p:classic-Pluecker}.

Moreover, the projection $\Gamma'$ from a point $o \in \Tan(\Gamma)$
has two less flexes than the projection from a general point.
This follows from the Plücker formula $(P_2)$, arguing once again
that a node has become a cusp.
From a more geometric point of view, we have seen in
\ref{p:inters-infnear-planes} that the generators of
$\Tan(\Gamma)$ are the intersections of two infinitely near osculating
planes of $\Gamma$; these are the two osculating planes of $\Gamma$
through $o$ that no longer give flexes of $\Gamma'$.
Note that these two infinitely near osculating
planes of $\Gamma$ correspond to the tangency point of the oscdual
curve $C = \dual {\Tan(\Gamma)}$ with the plane $\orth o$.


\begin{proposition}
\label{pr:proj-sec}
The section of $\Tan(\Gamma)$ by a plane $H$ is the dual curve of the
plane curve $\pi_{\orth H} (C)$.
\end{proposition}

\begin{proof}
For all $p \in \Tan(\Gamma) \cap H$, there is a point
$q \in \Gamma$ such that
$p= H \cap \T_q\Gamma$.
By duality, the orthogonal line $\orth
{(\T_q\Gamma)}$ is the tangent to $C$ at the point $\orth
{(\Osc_q\Gamma)}$.
It follows that the plane $\orth p$ is tangent to $C$
at $\orth {(\Osc_q\Gamma)}$, as it contains
$\orth {(\T_q\Gamma)}$;
moreover, as it passes through the point $\orth H$, its projection
from $\orth H$ is a tangent line of $\pi_{\orth H} (C)$.
Conversely, all tangent lines to $\pi_{\orth H} (C)$ are obtained in
this way.
\end{proof}

As an illustration of the proposition, note that
the plane curve $H \cap \Tan(\Gamma)$ has cusps at the points where
$H$ meets the cuspidal edge of $\Tan(\Gamma)$, \ie $\Gamma$
itself, while the dual plane curve $\pi_{\orth H} (C)$
correspondingly has flex points
given by the osculating planes to $C$ passing through $\orth H$, \ie
the planes $\orth q$ for $q \in H \cap \Gamma$.

\begin{proposition}
\label{pr:tans-samedeg}
The two tangential surfaces $\Tan(\Gamma)$ and $\Tan(C)$ have the same
degree. 
\end{proposition}

\begin{proof}
As we have seen in \ref{p:not-char-dev-I},
the degree of $\Tan(\Gamma)$ is the number of lines
$\T_p\Gamma$ meeting a given, general, line $\Lambda \subset \P^3$.
Since the orthogonal $\orth [\T_p\Gamma]$ is the tangent line to $C$
at the point $\orth [\Osc_p\Gamma]$,
this is also the number of lines $\T_{p'}C$ meeting the line $\orth
\Lambda$, \ie the degree of $\Tan(C)$.
\end{proof}

% \begin{proof}
% Let $p \in \P^3$ be a point off $\Tan(\Gamma)$. The projected curve 
% $\pi_p(\Gamma)$ is the plane dual of the hyperplane section 
% $\orth p \cap \dual \Gamma = \Tan(C)$, so the degree of $\Tan(C)$ is
% the number of lines tangent to $\pi_p(\Gamma)$ passing through a fixed
% point $q \in \P^3/p$, equivalently the number of planes tangent to
% $\Gamma$ containing the line $\vect{p,q} \subset \P^3$. Now the planes
% tangent to $\Gamma$ are those containing a generator of
% $\Tan(\Gamma)$. Hence the number of planes tangent to $\Gamma$ and
% containing $\vect{p,q}$ equals the number of generators of
% $\Tan(\Gamma)$ meeting $\vect{p,q}$, which is none other than the
% degree of $\Tan(\Gamma)$.
% \end{proof}


\subparagraph{Remark}
Proposition~\ref{pr:tans-samedeg} is a twisted version of the fact
that the class of a (non-developable) ruled surface equals its
degree.
\par
To compare the two situations, let's recall the proof. Let $S \subset
\P^3$ be a 
ruled surface, and assume $\check S$ is a surface. The class of $S$ is
the number of tangent planes of $S$ containing a given, general,
line $\Lambda \subset \P^3$. Since $\check S$ is a surface, the planes
tangent to $S$ are exactly the planes that contain a ruling of $S$. It
follows that the class of $S$ is the number of rulings of $S$ that
meet $\Lambda$. But the latter number also equals the degree of $S$.
\par
If $S$ is developable, it is no longer true that its tangent planes
are those containing a ruling (indeed there is only one tangent plane
per ruling), and the number of planes tangent to $S$ containing a line
$\Lambda$ is zero, as $\dual S$ actually has codimension $2$ in
$\check \P^3$.

\bigskip
It is useful to analyze the sections of the developable surface by
planes containing a generator.

\begin{lemma}
\label{l:sec-dev-gen-i}
Let the hyperplane $H \subset \P^3$ contain the line $\T_p\Gamma$ for
some $p \in \Gamma$, and write $H\cap \Tan(\Gamma)$ as
$\T_p\Gamma + R$. In general, the residual section $R$ has one more
flex and two less cusps than the general plane section of
$\Tan(\Gamma)$. The extra flex point is $p$, and $\T_p R =
\T_p\Gamma$. 
\end{lemma}

\begin{proof}
The point $\orth H \in \check \P^3$ sits on the line
$\orth {(\T_p\Gamma)}$ which is
tangent to $C$ at the point $\orth {(\Osc_p \Gamma)}$, so the curve
$\pi_{\orth H} (C)$ has one more cusp and 
two less flexes than the projection of $C$ from a general point,
as explained in Paragraph \ref{com:proj-spcurv}.
Dually, this gives the first assertion about $R$.
In addition, note that the class of $\pi_{\orth H} (C)$ is one less
than that of a general projection, agreeing with the fact that
$\deg(R) = \deg (\Tan\, \Gamma)-1$.

The tangent cone to $\pi_{\orth H} (C)$ at its extra cusp is
the projection from $\orth H$ of the plane 
$\Osc _{\orth {(\Osc_p \Gamma)}} C$; its orthogonal is the extra flex
point of 
$R$, and it is the point $p$.
Moreover, the tangent line to $R$ at $p$ is the orthogonal of the
cuspidal point of $\pi_{\orth H} (C)$; the latter is the projection
from $\orth H$ of the line $\orth {(\T_p\Gamma)}$, hence $\T_pR$ equals
$\T_p\Gamma$. 
\end{proof}

We may now prove the following. Before we start, note that
being $\Tan(\Gamma)$ ruled, its double points lie on two generators:
if they are distinct then the double point is on the ordinary double
curve, otherwise it is on the cuspidal edge.
Given a generator $\T_p\Gamma$, $p$ is the only point of $\T_p\Gamma$
lying on the cuspidal edge, unless $\T_p\Gamma$ is tangent to $\Gamma$
at some other point.

\begin{proposition}
\label{c:deg-double-curv-dev}
The degree
of the ordinary double curve of $\Tan(\Gamma)$ equals $r-4$.
\end{proposition}

\begin{proof}
Consider the section of $\Tan(\Gamma)$ by a plane $H$ containing a
generator $\T_p\Gamma$ as in Lemma~\ref{l:sec-dev-gen-i}: it consists
of the line line $\T_p\Gamma$ and a residual curve $R$ of degree
$r-1$. They meet with multiplicity $3$ at $p$, and at $r-4$ further
points $p_1,\ldots,p_{r-4}$,
which are the intersection points of $\T_p\Gamma$ and the ordinary
double curve of $\Tan(\Gamma)$.
\end{proof}

% \subparagraph{}
% \label{c:deg-double-curv-dev:com}
Note that, in the notation of the above proof,
since $p_1,\ldots,p_{r-4}$ are the intersection points of $\T_p\Gamma$
and the ordinary double curve, they are independent of the choice of
$H$ in the pencil of planes containing $\T_p\Gamma$.

For all $i=1,\ldots,r-4$, there is a point $q_i \in \Gamma$ such that 
$p_i = \T_p \Gamma \cap \T_{q_i} \Gamma$.
It follows that the plane $\orth {p_i} \subset \check \P^3$ is tangent
to $C$ at the two points $\orth {(\Osc_p \Gamma)}$ and 
$\orth {(\Osc_{q_i} \Gamma)}$, which explains why it should be an
ordinary double point of the surface $\Tan(\Gamma)=\dual C$ according
to the general principles of duality.


% It is interesting to explain this following the principles of
% biduality. 
% Let us prove that the points $x_1,\ldots,x_{r-4}$ lie on $r-4$
% generators $\Lambda_1,\ldots,\Lambda_{r-4}$ respectively, all distinct
% from $\T_x\Gamma$. 

% The residual $R$ is the plane dual of $\pi _{\orth H} (C)$, and
% $\T_x\Gamma$ is the orthogonal of its cusp $k=\pi _{\orth H} \bigl(
% \orth {(\T_x\Gamma)} \bigr)$. It follows that the points $x_i$
% correspond to the tangent lines of $\pi _{\orth H} (C)$ passing
% through $k$. 
% In turn, these tangent lines are the projections of the planes in
% $\check\P^3$ passing through $\orth H$ and tangent to $C$.

\begin{lemma}
\label{l:sec-dev-tg}
Let $p\in \Gamma$.
The section of $\Tan(\Gamma)$ by its tangent plane
$\Osc_p (\Gamma)$
decomposes
as $2\T_p\Gamma+R$, where the curve $R$ is
tangent to $\T_p\Gamma$ at $p$,
and passes through all the ordinary
double points $p_1,\ldots,p_{r-4}$ of $Tan(\Gamma)$ lying on
$\T_p\Gamma$.
\end{lemma}

\begin{remark}
The pencil of curves
cut out on $\Tan(\Gamma)$ by the planes containing $\Lambda =
\T_p\Gamma$ is a 
family of plane curves with prescribed contact 
$3p+p_1+\cdots+p_{r-4}$ 
with $\Lambda$,
which degenerates to a curve containing $\Lambda$
itself when the plane tends to the tangent plane $\Osc_p(\Gamma)$.
This is exactly the situation considered by Caporaso and
Harris in \cite{ch-13} and studied in the first half of this volume.
\end{remark}

\begin{proof}[Proof of Lemma \ref{l:sec-dev-tg}]
Let $H=\Osc_p\Gamma$.
The section $H \cap \Tan(\Gamma)$ must decompose as
$2\T_x\Gamma+R$, with $R$ the
plane dual of the projected curve $\pi_{\orth H}(C)$.
This time the point $\orth H \in \check \P^3$ sits on the curve $C$,
and the projection $\pi_{\orth H}(C)$
is smooth at the point image of $\orth H$,
namely $\pi_{\orth H} (\T_{\orth H} C)$, with tangent line
$\pi_{\orth H} (\Osc_{\orth H} C)$ there.
It follows that $p = \orth {(\Osc_{\orth H} C)}$ is on the plane dual
$R$, with tangent
$\T_p R = \orth{(\T_{\orth H} C)} = \T_{p} \Gamma$. This proves the
first assertion.

For the second,
letting once again $p_i = \T_p \Gamma \cap \T_{q_i} \Gamma$,
we have seen that the plane $\orth {p_i}$ 
is tangent to $C$ at the two points $\orth H$ and
$\orth {(\Osc_{q_i} \Gamma)}$. Thus
$\pi _{\orth H} (\orth {p_i})$ is the tangent line to $\pi _{\orth H}
(C)$ at 
$\pi _{\orth H} (\orth {(\Osc_{q_i} \Gamma)})$, 
hence $p_i \in R$ since the latter is the plane dual of 
$\pi _{\orth H} (C)$.
\end{proof}


Finally, let us check by duality that the degree of $R$ is indeed
$r-2$ in the above context.
Let $g$ be the genus of $C$. The projection of $C$ from a
general point of $\check \P^3$ is a nodal degree $n$ plane curve of
genus $g$, 
which thus has $\delta= \frac 1 2 (n-1)(n-2)-g$ nodes, hence class
$r=n(n-1)-2\delta$.
If however it gets projected from a general point on itself,
it still gives a genus $g$ nodal curve, but with degree $n-1$, so that
the number of nodes becomes 
$\delta'=\frac 1 2 (n-2)(n-3)-g=\delta -(n-2)$.
The class of this curve is then
$(n-1)(n-2)-2\delta'$, which is $r-2$ as required.



\subsection{Pl{\"u}cker formulae}
\label{s:plucker-dev}

We now explain how the Pl{\"u}cker formulae for plane curves may be used
to derive relations between the numerical characters of a developable
surface, following Cayley \cite{cayley-memoir}.
As for plane curves, it turns out to be appropriate
to let the curves $\Gamma$ and $C$ have various
kinds of singularities which are stable under oscduality.
We thus consider a slightly more general
situation than what we did in Subsection~\ref{s:edge}, by allowing the
stationary behaviours indicated below.

\paragraph{Characteristic numbers, II}
\label{p:not-char-dev-II}
In addition to the quantities introduced in \ref{p:not-char-dev-I}, we
let 
\begin{mycpctitem}
\item $\alpha$ the number of ordinary cusps of $C$,
\ie points at which $C$ has a local parametrization of the form 
$t \mapsto (t^2,t^3,t^4)$~;
\item $\beta$ the number of ordinary cusps of $\Gamma$~;
\item $x$ the degree of the ordinary double curve of $\Tan(\Gamma)$;
\item $y$ the degree of the ordinary double curve of $\Tan(C)$;
\item $g$ the number of apparent double points of $C$;
\item $h$ the number of apparent double points of $\Gamma$.
\end{mycpctitem}
The quantities $\alpha$ and $\beta$ are classically referred to 
as the
number of stationary planes and points of the system.
The quantity $x$ is the number of points in a general plane $H\subset
\P^3$ that lie on two distinct
tangent lines of $\Gamma$, see Proposition \ref{c:deg-double-curv-dev}
and the comment before it; 
dually, $y$ is the number of planes passing through a general point,
and containing two distinct tangent lines of $\Gamma$.
The quantity $h$ is the number of lines meeting $\Gamma$ in two points
(\ie secants of $\Gamma$)
passing through a general point of $\P^3$;
dually,
$g$ is the number of lines lying in a general plane $H
\subset \P^3$ that are contained in two osculating planes of $\Gamma$.

\begin{lemma}
\label{lem:osc-Gauss-exch}
Consider the osculatory Gauss map $\Gamma \to C$, mapping a general
point $p\in\Gamma$ to the point $\orth{(\Osc_p \Gamma)} \in \check
\P^3$. 
It sends a point where $\Gamma$ has a local parametrization of
the form $t \mapsto (t,t^2,t^4)$
(resp.\ $t \mapsto (t^2,t^3,t^4)$)
to a point where $C$ has a local parametrization of
the form $t \mapsto (t^2,t^3,t^4)$
(resp.\ $t \mapsto (t,t^2,t^4)$).
\end{lemma}

\medskip
The upshot is that the osculatory Gauss map turns points of types
$\alpha$ and $\beta$ of $\Gamma$ to points of types
$\beta$ and $\alpha$ of $C$, respectively.

%\medskip
\begin{proof}
This is a local computation: 
to a local branch of $\Gamma$ parametrized by
$t\in \C \mapsto f(t)\in \C^4$, the osculatory Gauss maps associates
the local branch of $C$ parametrized by
$t\in \C \mapsto \bigl( f \wedge \partial_tf \wedge \partial_t^2 f
\bigr)(t)
\in \bigwedge ^3 \C^4 \cong \check \C^4$.
In the former case, the result follows from the identity
\[\small
\begin{pmatrix}
1 \\ t \\ t^2 \\ t^4
\end{pmatrix}
\wedge \begin{pmatrix}
0 \\ 1 \\ 2t \\ 4t^3
\end{pmatrix}
\wedge \begin{pmatrix}
0 \\ 0 \\ 2 \\ 12t^2
\end{pmatrix}
=
\begin{pmatrix}
-6t^4 & 16 t^3 & -12 t^2 & 2
\end{pmatrix}.
\]
We leave the computation in the latter case to the reader.
\end{proof}


\paragraph{}
\label{p:plucker-devI}
Let us apply the Pl{\"u}cker formulae to a general hyperplane section 
$H \cap \Tan(\Gamma)$; as a plane curve, it is dual to
$\pi_{\orth H} (C)$.
The former is a curve of degree $r$, with $x$ nodes and $m$ cusps,
and the latter has degree $n$ and $g$ nodes; for general $H$, its only
cusps come from cusps of $C$, which are in the number $\alpha$.
% by Lemma \ref{lem:osc-Gauss-exch}. 
We thus get the following identities:
\begin{alignat*}{2}
n &= r(r-1)-2x - 3m;
\hspace{1cm} & r &= n(n -1)-2g-3\alpha; \\
\alpha &= 3r(r-2) -6x -8m;
& m &= 3n(n-2) -6g -8\alpha,
\end{alignat*}
hence
\begin{alignat*}{2}
\alpha - m &= 3(n-r);
&\hspace{1cm} 2(g-x) &= (n -r)(n + r-9).
\end{alignat*}

\paragraph{}
\label{p:plucker-devII}
Dually, one may apply the Pl{\"u}cker formulae to the pair of dual plane
curves $\pi_o(\Gamma)$ and $\orth o \cap \Tan(C)$ for a general point
$o \in \P^3$.
This gives:
\begin{alignat*}{2}
r &= m(m-1)-2h - 3\beta;
\hspace{1cm}& m &= r(r -1)-2y-3n; \\
n &= 3m(m-2) -6h -8\beta;
& \beta &= 3r(r-2) -6y -8n,
\end{alignat*}
hence
\begin{alignat*}{2}
n - \beta &= 3(r-m)
\hspace{1cm}& 2(y-h) &= (r -m)(r + m-9).
\end{alignat*}

\paragraph{}
\label{p:plucker-devI+II}
Eventually, one may combine the identities from \ref{p:plucker-devI}
and \ref{p:plucker-devII} to obtain:
\begin{gather*}
\alpha - \beta = 2(n-m), \qquad
x-y=n-m, \\
2(g-h) = (n-m)(n+m-7).
\end{gather*}


\paragraph{}
\label{s:stat-lines}
It seems natural to allow the system to have stationary lines as well,
\ie the curve $\Gamma$ to have points at which it is locally
parametrized by $t\mapsto (t,t^3,t^4)$.
I have chosen not to do it from the start, in order to give a more
straightforward application of the Pl{\"u}cker formulae for plane
curves. Let me now add two statements with which it is possible
to adapt the above arguments in
order take the possibility of stationary lines in consideration, which
I will leave to the reader.

First,
a local computation as in the proof of \ref{lem:osc-Gauss-exch} shows
that the osculatory Gauss map sends a point at which $\Gamma$ has a
stationary tangent line to a point at which $C$ has a stationary
tangent line.
The second statement is the following.

\begin{lemma}
The stationary lines of the system give cuspidal lines to both
tangential surfaces $\Tan(\Gamma)$ and $\Tan(C)$.
\end{lemma}

\begin{proof}
Let $p \in \Gamma$ be a point at which $\Gamma$ is locally
parametrized by $t\mapsto (t,t^3,t^4)$, and $\Lambda= \T_p\Gamma$ be
the corresponding (stationary) generator. We shall prove that for a
general plane $H \subset \P^3$, the section $H \cap \Tan(\Gamma)$ has
a cusp at the point $H \cap \Lambda$, or equivalently the curve
$\pi _{\orth H}(C)$ has a flex at
$\pi _{\orth H}\bigl( \orth{(\Osc_p\Gamma)} \bigr)$ along the line
$\pi _{\orth H}(\orth \Lambda)$.

As we have seen, the curve $C$ has a local parametrization of the form
$t\mapsto (t,t^3,t^4)$ at the point $\orth{(\Osc_p\Gamma)}$.
Thus after projection from the general point $\orth H$, the curve $\pi
_{\orth H}(C)$ has a local parametrization of the form
$t \mapsto (t,t^3)$. The result follows since $\orth \Lambda$ is the
tangent line to $C$ at $\orth{(\Osc_p\Gamma)}$.
\end{proof}


\subsection{Generalized Pl{\"u}cker formulae}

In this section I outline the generalization of the previous
formulae to curves in a projective space of arbitrary dimension,
which is due to Piene \cite{piene-duality}.
This is not used in the course of the text, but it would be a pity not
to mention it.
Note that there also exists a duality between the $i$-th ranks of an
arbitrary variety in projective space and those of its dual, which is
due to Urabe \cite{urabe-duality}, see also
\cite{kleiman-aarhus},
and \cite{aluffi-involution},
but this I will be reasonable and not talk
about it here.

\paragraph{}
\label{p:dev-genus}
So far we have only considered extrinsic invariants of the curve
$\Gamma \subset \P^3$. 
% Among those, let us add (see \ref{s:stat-lines})
% \begin{mycpctitem}
% \item $\nu$ the number of stationary tangent lines of $\Gamma$.
% \end{mycpctitem}
Adding its geometric genus $p_g$ in the picture,
one finds:
\begin{equation}
\label{eq:deg-tan}
r=2m+2p_g-2-\beta
\end{equation}
(recall the notation from \ref{p:not-char-dev-I}
and \ref{p:not-char-dev-II}).

\begin{proof}
Let $\Lambda \subset \P^3$ be a general line. We want to compute the
number of tangent lines to $\Gamma$ meeting $\Lambda$, or equivalently
the number of planes tangent to $\Gamma$ and containing $\Lambda$. To
this end we consider the projection from $\Lambda$;
it induces a degree $m$ covering $\bar \Gamma \to \P^1$,
where $\bar \Gamma$ is the normalization of $\Gamma$.
By the Riemann--Hurwitz formula, it has $2m+2p_g-2$ ramification points,
of which $\beta$ come from the ramification points of the
normalization map of $\Gamma$. The other ones correspond to planes
tangent to $\Gamma$ and containing $\Lambda$.
\end{proof}

\bigskip
\subparagraph{Remark}
The same reasoning may be applied to the curve $C$; one gets in this
way the identity
\begin{equation*}
r= 2n+2p_g-2-\alpha.  
\end{equation*}
Indeed, the osculatory Gauss map gives a birationality between
$\Gamma$ and $C$, so these two curves have the same geometric genus,
and $r$ is the degree of both $\Tan(C)$ and $\Tan(\Gamma)$ by
Proposition~\ref{pr:tans-samedeg}.
\par
Putting the two identities together, one finds the formula
$2(n-m)=\alpha-\beta$ 
which we have already gotten in \ref{p:plucker-devI+II}.



\paragraph{New setup}
\label{p:newsetup}
From now on, we consider a curve $\Gamma \subset \P^N$ of degree $m$
and geometric genus $p_g$. 
Let $\bar \Gamma \to \Gamma$ be its normalization, and $f: \bar \Gamma
\to \P^N$ its composition with $\Gamma \hookrightarrow \P^N$.
For all $p \in \Gamma$ one may
choose a local parameter $t$ at $p$ on $\bar \Gamma$ and a system of
homogeneous coordinates $(x_0:x_1:\ldots:x_N)$ on $\P^N$ such that $f:
\bar \Gamma \to \P^N$ 
is given locally by
% in the affine chart $x_0=1$ by 
\[
t \mapsto \bigl(1:
t^{1+s_1}:\ldots:
t^{N+s_1+\cdots+s_N} \bigr)
\]
up to higher order terms
(\ie the $i$-th coordinate of $f$ is a formal power series in $t$
whose leading term is $t^{i+s_1+\cdots+s_i}$),
and $s_1,\ldots,s_N$ are non-negative integers depending only on
$p$.
The point $p$ is \emph{ordinary} if $s_1=\cdots=s_N=0$, and 
\emph{stationary} or \emph{hyperosculating} otherwise.

For all $i=0,\ldots,N-1$, the $i$-th osculating subspace of $\Gamma$
at $p \in \bar \Gamma$,
denoted $\Osc^i _p (\Gamma)$,
is the $(N-i)$-plane in $\P^N$ defined by the
equations 
$x_N=\cdots=x_{N-i+1}=0$ in a system of homogeneous coordinates as
above.
We shall consider the $i$-th \emph{osculating variety} of $\Gamma$,
denoted by $\Osc^i(\Gamma)$,
that is the union of the $i$-th osculating subspaces of $\Gamma$ at
all the points of $\bar \Gamma$.
For $i=0$ this is $\Gamma$ itself, for $i=1$ this is the tangential
surface of $\Gamma$ that we have considered in the previous
subsections; for $i=N-1$ this fills the whole $\P^N$, hence it is best
seen as a curve $C \subset \check \P^N$ which I call the
\emph{osc-dual} curve of $\Gamma$.

\paragraph{The $i$-th ranks}
\label{p:i-th-rks}
For all $i=0,\ldots,N-1$,
let $r_i$ be the degree of the
$i$-th osculating variety of $\Gamma$;
it is called the \emph{$i$-th rank} of $\Gamma$.
For $i=N-1$, this is by definition the
degree of the osc-dual curve $C \subset \check \P^N$.
We define integers $k_i$ by 
\begin{equation*}
k_i := \sum\nolimits_{p \in \Gamma} s_i(p),
\end{equation*}
where $s_i(p)$ is defined as in \ref{p:newsetup}.

A standard computation on the Chern classes of the bundles of
principal parts of the embedding of $\bar\Gamma$ in $\P^N$,
see \cite[Prop.~10.4.13]{dolgachev}, gives the following formulae:
\begin{gather}
\label{i-th-rk}
r_i = (i+1)\bigl(m + i(p_g-1)\bigr) 
-\sum\nolimits_{j=1}^i \bigl(
(i-j+1)k_j
\bigr)
\qquad \text{for all}\ i=0,\ldots,N-1 \\
\label{tot-ramif}
\sum\nolimits_{j=1}^N \bigl(
(N-j+1)k_j
\bigr) =
(N+1)\bigl(m + N(p_g-1)\bigr).
\end{gather}

Formula~\eqref{i-th-rk} for $i=0$ is trivial, as $r_0=\deg(\Gamma)=m$
by definition.
Formula \eqref{tot-ramif} has to be understood as the incarnation
for $i=N$ of formula \eqref{i-th-rk}, setting $r_N=0$. 
For $i=1$, one gets a formula which is exactly \eqref{eq:deg-tan}.
Eventually, note that formula \eqref{tot-ramif} may be interpreted as
counting the stationary points of $\Gamma$, with the multiplicity
\[
s_N+2s_{N-1}+\cdots+(N-1)s_2+Ns_1.
\]


\paragraph{Generalized Pl{\"u}cker formulae}
As a straightforward corollary of the formulas in \ref{p:i-th-rks},
one has 
\begin{equation}
\label{gnlzd-plucker}
r_{i-1} -2r_i + r_{i+1} = 2p_g-2 -k_{i+1},
\qquad \text{for all}\ i=0,\ldots,N-1,
\end{equation}
with the convention that $r_N=r_{-1}=0$.

\bigskip
\subparagraph{Plane curves} For $N=2$, we are considering a plane
curve $\Gamma$ of degree $m$. The number $k_1$ (resp.\ $k_2$) counts, with
multiplicities, the cusps (resp.\ the flexes) of $\Gamma$, so we will
call it $\kappa$ (resp.\ $\iota$) as usual. 
Formula \eqref{gnlzd-plucker} gives the two identities
\begin{alignat*}{2}
-2m+\check m &= 2p_g-2 -\kappa~;
&\hspace{15mm} 
m-2\check m &= 2p_g-2 - \iota.
\end{alignat*}
The second formula is merely the first applied to
$C$, which in this case is the plain dual of $\Gamma$.
Assuming $\Gamma$ has only $\delta$ nodes and $\kappa$
(ordinary) cusps as
singularities, these may be recovered from the usual formulae
\begin{alignat*}{2}
\check m&=m(m-1)-2\delta-3\kappa~;
&\hspace{15mm} 
2p_g-2 &= m(m-3)-2\delta -2\kappa
\end{alignat*}
(the first one is the computation of the class using polars for a
singular curve as in \ref{p:classic-Pluecker}, and the second one is
the adjunction formula for a (possibly) singular plane curve.
One gets the first formula by writing
\begin{equation*}
\check m -2m 
= m(m-1)-2\delta-3\kappa -2m
= m(m-3)-2\delta-3\kappa 
= 2p_g-2 - \kappa.
\end{equation*}

\bigskip
\subparagraph{Space curves}
For $N=3$ we are considering a space curve $\Gamma \subset \P^3$ as in
the previous subsections. In the notation therein, the ranks
$r_0,r_1,r_2$ are respectively the degree $m$, the rank $r$, and the
class $n$. On the other hand, $k_1,k_2,k_3$ are respectively the
number $\beta$ of cusps of $\Gamma$, the number of stationary lines
(let us call it $\gamma$), and the number $\alpha$ of cusps of $C$.
Formula \eqref{gnlzd-plucker} gives the three identities
\\[\abovedisplayskip]
$\phantom.
\hfill
-2m+ r = 2p_g-2 -\beta~;
\hfill
m-2r + n = 2p_g-2 - \gamma~;
\hfill
r -2 n = 2p_g-2 - \alpha.
\hfill
$


\paragraph{Piene duality
{\normalfont \cite[Thm.~5.1]{piene-duality}}}
\label{p:P-dual}
{\itshape
Let $\Gamma \subset \P^N$ be a curve, and $C \subset \check \P^N$ its
osc-dual curve. The osc-dual curve of $C$ is $\Gamma$, and the
following relations hold
for all $i=0,\ldots,N-1$:
\begin{align}
\label{P-dual1}
r_i (C) &= r_{N-i-1} (\Gamma) \\
\label{P-dual2}
k_i (C) &= k_{N-i-1} (\Gamma).
\end{align}
}

Formula \eqref{P-dual1} generalizes the fact that for $N=3$ the two
tangential surfaces $\Tan(\Gamma)$ and $\Tan(C)$ have the same degree,
see Proposition~\ref{pr:tans-samedeg},
and
Formula \eqref{P-dual2} the fact that the osc-Gauss map turns
stationary planes, lines and points of $\Gamma$ into stationary
points, lines, and planes of $C$ respectively, see Lemma
\ref{lem:osc-Gauss-exch}. 

\paragraph{Interpretation as strata of the dual hypersurface}
\label{:P-bidual}
Underlying the merely numerical relations of \ref{p:P-dual} is the
following geometric duality, which generalizes \ref{p:devel-bidual}.

\def\idual#1#2{{#1}^{\vee_{#2}}}
For all $i>0$, we say that a hyperplane $H \subset \P^N$ is
\emph{$i$-osculating} to $\Gamma$ at $p\in \bar\Gamma$ if 
it contains $\Osc^i_p(\Gamma)$.
If $p\in \bar\Gamma$ is an ordinary point of $\Gamma$,
this is equivalent to the divisor 
$f^*H-(i+1)p$ on $\bar\Gamma$ being effective.
We let 
$\idual \Gamma i$
be the closed subset
parametrizing hyperplanes $i$-osculating to $\Gamma$ at some point on
$\bar \Gamma$; thus $\idual \Gamma 1$ is the plain dual hypersurface
$\dual \Gamma$, and $\idual \Gamma {N-1}$ is the osc-dual curve $C$.

For all $i=0,\ldots,N-1$,
one has $\idual \Gamma i = \Osc^{N-1-i}(C)$,
and moreover $\dual {\Osc^i(\Gamma)} = \idual \Gamma {i+1}$.
In fact, for all $p\in \bar\Gamma$, the linear space
% the orthogonal of the $i$-th osculating space of $\Gamma$ at $p\in
% \bar \Gamma$
$\orth {\Osc^i_p(\Gamma)}$
 is the
$(N-1-i)$-th osculating space of $C$ at $p$
(note that the map $p\in \bar \Gamma \mapsto [\Osc^{N-1}_p(\Gamma)]
\in \check \P^N$
is the normalization of $C$). 

For all $i=0,\ldots, N-1$,
let $f_i: \bar \Gamma \to \G(\P^N,i)$ 
and $\idual f {i}: \bar \Gamma \to \G(\check \P^N,i)$)
be the maps
$p \mapsto \Osc^i_p(\Gamma)$
and $p \mapsto \Osc^i_p(C)$ respectively.
The map $\idual f {N-1-i}$ equals the composition of $f_i$ with the
orthogonality map 
$\Lambda \in \G(\P^N,i) \mapsto \orth \Lambda \in \G(\check
\P^N,N-1-i)$. 
It follows that the two curves $f_i(\bar\Gamma)$ and $\idual f {N-1-i}
(\bar\Gamma)$ have the same degree under the Pl{\"u}cker embeddings of
$\G(\P^N,i)$ and $\G(\check \P^N,N-1-i)$ respectively; these degrees are
$r_i(\Gamma)$ and $r_{N-1-i}(C)$ respectively
(see, \eg \cite[Example 19.11]{harris-13}), so we find
Formula \eqref{P-dual1}.


\subsection{De Jonqui{\`e}res' formula}
\label{s:deJonqu}


The next result is even more general than the previous ones. See
\cite[Chap.~VIII]{acgh} for a proof and pointers to the
literature. 


\begin{theorem}[de Jonqui{\`e}res formula]
\label{t:dJ}
Let $m$ be a positive integer, and $m_1,\ldots,m_a$ be
non--negative integers such that
$m=\sum _{1\leq s \leq a} s \cdot m_s$.
The virtual number of divisors having $m_s$ points of
multiplicity $s$ for all $s=1,\ldots,a$ 
in a given linear series of degree $m$ and dimension
$i=\sum _{1\leq s \leq a} (s-1)\cdot m_s$ 
on a smooth, genus $g$ curve
is the coefficient of the $t_1 ^{m_1} \cdots t_a ^{m_a}$ term in the
formal power series
\begin{equation*}
\bigl( 1+1^2t_1 + 2^2 t_2+ \cdots + a^2 t_a \bigr)^g
\cdot \bigl( 1+1\, t_1 + 2 t_2+ \cdots + a t_a \bigr)
^{m-i-g}.
\end{equation*}
\end{theorem}


\paragraph{Link with the $i$-th ranks}
We now show how the de Jonqui{\`e}res formula may be used to derive the
$i$-th ranks of a curve $\Gamma \subset \P^N$ of degree $m$ and
geometric genus $g$ as in \ref{p:newsetup}, thus recovering formula
\eqref{i-th-rk}. 

By definition,
$r_i(\Gamma)
= r_{N-1-i}(C)
= \deg (\Osc ^{i}(\Gamma))$
is the number of hyperplanes $i$-osculating to
$\Gamma$ in a general $i$-dimensional linear subsystem of
$|\O_\Gamma (1)|$. 
By de Jonqui{\`e}res' formula, the number of hyperplanes $H$ such that
$f^*H-(i+1)p$ is effective for some $p\in \bar\Gamma$ in a general
$i$-dimensional linear subsystem of $|\O_\Gamma (1)|$ 
is the coefficient of the monomial $t_1 ^{m-i-1} t_{i+1}$ in
% \[
% \bigl( 1+1^2t_1 + 2^2 t_2+ \cdots + (i+1)^2 t_{i+1} \bigr)^g
% \cdot \bigl( 1+1\, t_1 + 2 t_2+ \cdots + (i+1) t_{i+1} \bigr)
% ^{m-i-g}.
% \]
% This is also the coefficient of $t_1 ^{m-i-1} t_{i+1}$ in
\begin{multline*}
\bigl( 1+1^2t_1 + (i+1)^2 t_{i+1} \bigr)^g
\cdot \bigl( 1+1\, t_1 + (i+1) t_{i+1} \bigr)
^{m-i-g}\\
\begin{aligned}
&= 
\bigl( 1+1^2t_1 + [(i+1)+i(i+1)] t_{i+1} \bigr)^g
\cdot \bigl( 1+1\, t_1 + (i+1) t_{i+1} \bigr)
^{m-i-g}
\\
&=
\sum _{j=0} ^g \binom g j
\bigl( 1+ t_1 + (i+1) t_{i+1} \bigr)^{(g-j)+m-i-g}
\cdot \bigl(
i(i+1) t_{i+1}
\bigr) ^j,
\end{aligned}
\end{multline*}
which is also the coefficient of $t_1 ^{m-i-1} t_{i+1}$ in
\begin{equation*}
\bigl( 1+ t_1 + (i+1) t_{i+1} \bigr)^{m-i}
+ i(i+1) t_{i+1} \cdot g \bigl( 1+ t_1 + (i+1) t_{i+1} \bigr)^{m-i-1},
\end{equation*}
that is
\begin{equation}
\label{i-rk-dJ}
(m-i)(i+1)+ i(i+1) \cdot g
= (i+1) \bigl(m+(g-1)i \bigr).
\end{equation}

To obtain $r_i$ from the number \eqref{i-rk-dJ}, one ought to subtract
the excess contributions of the various stationary points of $\Gamma$.
For $i=1$ for instance, for all cusp $p$ of $\Gamma$
(\ie for all $p \in \bar\Gamma$ such that $s_1(p)>0$), the whole 
$\orth p \subset \check \P^N$ gives rise to hyperplanes contributing
to the number \eqref{i-rk-dJ}, so that the latter  actually is the degree
of the reducible hypersurface sum of $\idual \Gamma 1$ and the various
$\orth p$ for all cusps $p$ of $\Gamma$. 
Taking this into consideration, one recovers
Formula \ref{p:dev-genus} for $r_1$.

For $i=2$, also the points $p \in \bar\Gamma$ such that $s_1(p)=0$ and
$s_2(p)>0$ contribute to \eqref{i-rk-dJ}, to the effect that $\orth
{(\Osc^1_p (\Gamma))}$ occurs together with $\idual \Gamma 2$.
In general, all $p\in \bar\Gamma$ such that $s_j(p)>0$ for some $j
\leq i$ contribute to \eqref{i-rk-dJ}, and to conclude we need to show
that each contributes with the multiplicity 
\[
s_i + 2\,s_{i-1} + \cdots + i\,s_1
\]
in de Jonqui{\`e}res' formula. 
I have not found this particular computation in the literature, and
will leave this as an open exercise to the reader.


\section{Biduality for asymptotic tangent lines by
  enumerative means}
\label{S:asympt}

Let $\Lambda$ be an asymptotic tangent line to a surface
$S \subset \P^3$ at a
smooth point $p$. In this appendix, we show that the line 
$\orth \Lambda$ is an asymptotic tangent line to the dual surface
$\dual S$ at the point $\orth [\T_pS]$,
by computing the intersection multiplicity of $\orth \Lambda$ and
$\dual S$ at this point. We also prove several variants,
see Theorem \ref{T:bidual-tgline}.

To compute this intersection multiplicity,
we consider the pencil of hyperplane sections of $S$ parametrized by
$\orth \Lambda$,
and count its singular members with the topological formula involving
Euler numbers described in
\cite[Section~\tref{s:pencil}]{10.th-panoramico}.
The intersection multiplicity we are looking for is the multiplicity
of the tangent section $\T_pS \cap S$ as a singular member of this
pencil 
(indeed the singular members of $\orth\Lambda$ correspond to the
intersection points of $\orth \Lambda$ with $\dual S$).
The upshot is the following lemma.

\begin{lemma}
\label{l:pencil-13}
Let $S \subset \P^3$ be a smooth surface, 
$\Lambda$ be a line, and $H$ be a hyperplane containing $\Lambda$.
Let $\tilde S \to S$ be the minimal sequence of blow-ups at reduced
points such that the proper transform $\tilde \Lambda$ of the pencil
$\orth \Lambda$ is base-point-free. 
Let $\tilde C_H$ and $\tilde C_\gen$ be the members of $\tilde
\Lambda$ corresponding 
to $C_H= H\cap S$ and a general member $C_\gen$ of $\orth
\Lambda$, respectively.
The intersection multiplicity of $\orth \Lambda$ and $\dual S$ at
$\orth H$ equals the difference in Euler numbers
$e(\tilde C_H)-e(\tilde C_\gen)$.
\end{lemma}


The assumption that $S$ is smooth is only to simplify matters:
one may adapt the lemma to a surface with given singularities, using
the same method.
The lemma follows from a direct application of 
\cite[Lemma~\tref{l:pencil}]{10.th-panoramico}
to the morphism $\tilde S \to \P^1$ given by $\tilde \Lambda$.
The same idea appears in \cite{parunsinski}
and \cite{aluffi-cukierman}.
With this tool at hand, we may now prove the following biduality
statement. 

\begin{theorem}
\label{T:bidual-tgline}
Let $S \subset \P^3$ be a smooth surface, and $p \in S$. The
orthogonal line to 
\begin{mycpctenum}[(a)]
\item a tangent at $p$,
\item one of the two asymptotic tangents at a non-parabolic $p$,
\item the asymptotic tangent at a general parabolic point $p$,
\item the asymptotic tangent at a parabolic point $p$ of type $\beta$,
\end{mycpctenum}
respectively, is
\begin{mycpctenum}[(a)]
\item a tangent at $\orth [\T_pS]$,
\item one of the two asymptotic tangents at $\orth [\T_pS]$,
\item the tangent at $\orth [\T_pS]$ of the cuspidal double curve of
  $\dual S$,
\item the common reduced tangent cone at $\orth [\T_pS]$ of both the
ordinary and cuspidal double curves of $\dual S$.
\end{mycpctenum}
\end{theorem}

\begin{proof}
We proceed with a case by case analysis, and apply Lemma
\ref{l:pencil-13} in all cases.
We use similar notation (and abuse of notation) in all cases, which we
introduce in the first case, and then use freely in the others.

(a) Let $\Lambda$ be a general tangent line to $S$, and call $p$ the
contact point.  Then all members of $\orth \Lambda$ are tangent at
$p$, and we have to blow-up twice at $p$ to remove the base points:
we let $\epsilon_1: S_1 \to S$ be the blow-up at $p$,
with exceptional divisor $E_1$,
and $\epsilon_2: S_2 \to S_1$ be the blow-up at the point $p_1 \in E_1$
corresponding to the tangent direction at $p \in S$ defined by
$\Lambda$, with exceptional divisor $E_2$.

Locally over $p \in S$, the $\tilde S \to S$ of Lemma~\ref{l:pencil-13}
is $\epsilon=\epsilon_2 \,\epsilon_1: S_2 \to S$. 
Let $C$ be the hyperplane class on $S$. Forgetting about the base
points of $\orth \Lambda$ away from $p$, the base-point-free pencil
$\tilde \Lambda$ of Lemma~\ref{l:pencil-13} is the complete linear system
$|\epsilon^* C-\epsilon_2^* E_1 - E_2|$.
Our task now is to compute the transform $\tilde C_0$ of the curve 
$C_0 = S \cap \T_pS$ in this pencil.

Since $C_0 \subset S$ has a double point at $p$, we have
\[
\epsilon_1^* C_0 = C_0 + 2 E_1,
\]
where by abuse of notation $C_0$ also denotes the proper transform of
$C_0$ in $S_1$.
Next, one has
\[
\epsilon^* C_0 = \epsilon_2^* (C_0 + 2 E_1)
= C_0 + 2E_1 +2E_2
\]
with the same abuse of notation, this time for both $C_0$ and $E_1$.
Finally we find 
\[
\tilde C_0=
\epsilon^* C_0 -\epsilon_2^* E_1 - E_2
= \epsilon^* C_0 - (E_1+E_2) - E_2
= C_0 + E_1.
\]
This is a reduced curve with two ordinary double points, hence it
counts with multiplicity $2$ as a singular member of $\orth \Lambda$
(see \cite[subsec.~\tref{s:pencil}]{10.th-panoramico} for the details of the
computation). It follows that $\orth \Lambda$ is tangent to $\dual S$
at $\orth [\T_pS]$.
\begin{center}
\includegraphics[height=25mm]
{tg-line-gr.eps}
% original height 148,434
% 23 * 148,434 / 136,299

\captionof{figure}{Pencil with base locus an ordinary
  tangent line $\Lambda$}
\end{center}

(b) Let $\Lambda$ be an asymptotic tangent at a general point
$p$. Then the members of $\orth \Lambda$ are all osculating to the
order $3$ at $p$ (in fact, we know they all have a flex along
$\Lambda$), and we need to blow-up three times to remove the 
base points, with exceptional divisors $E_1,E_2,E_3$. The
base-point-free pencil $\tilde \Lambda$ is now
\[
|\epsilon^* C- \epsilon_3^* \epsilon_2^* E_1 - \epsilon_3^* E_2 -E_3|
%= |\epsilon^* C- \epsilon^* E_1 - \epsilon^* E_2 -E_3|
= |\epsilon^* C- E_1 - 2E_2 -3E_3|.
\]
% where we introduce yet another abuse of notation, to the effect that
% $\epsilon$ denotes whatever the appropriate composition of the various
% $\epsilon_i$'s is.
The curve $C_0 = S \cap \T_pS$ has an ordinary double point at
$p$, with one local branch simply tangent to $\Lambda$.
We thus have successively
\begin{align*}
\epsilon_1^* C_0 &= C_0 + 2 E_1 \\
\epsilon_2^*\epsilon_1^* C_0 &= C_0 + 2 E_1 +3E_2 \\
\epsilon_3^* \epsilon_2^*\epsilon_1^* C_0 &= C_0 + 2 E_1 +3E_2 +3E_3,
\end{align*}
hence the transform $\tilde C_0$ of $C_0 \subset S$ in $\tilde
\Lambda$ is
\[
\tilde C_0=
\epsilon^* C_0- E_1 - 2E_2 -3E_3
= C_0 + E_1 + E_2.
\]
It is reduced with $3$ nodes, hence counts with multiplicity $3$ as a
singular member of $\orth \Lambda$. This shows that $\orth \Lambda$ is
an asymptotic tangent to $\dual S$.
\begin{center}
\includegraphics[height=26.5mm]
{tg-asympt-gr.eps}
% original height 157,108 148,434
% 23 * 157,108 / 136,299
\captionof{figure}{Pencil with base locus an asymptotic
  tangent line $\Lambda$}
\end{center}

(c) Let $\Lambda$ be an asymptotic tangent at a general parabolic
point $p$. The situation is the same as in case (b), except that
the tangent section
$C_0 = S \cap \T_pS$ now has a cusp at
$p$, with tangent cone supported on $\Lambda$.
We have
\begin{align*}
\epsilon_1^* C_0 &= C_0 + 2 E_1 \\
\epsilon_2^*\epsilon_1^* C_0 &= C_0 + 2 E_1 +3E_2 \\
\epsilon_3^* \epsilon_2^*\epsilon_1^* C_0 &= C_0 + 2 E_1 +3E_2 +3E_3,
\end{align*}
and the transform of $C_0$ in the base-point-free pencil
$\tilde\Lambda$ is 
\[
\tilde C_0=
\epsilon^* C_0- E_1 - 2E_2 -3E_3
= C_0 + E_1 + E_2.
\]
It is reduced with a triple point, hence it counts with multiplicity
$4$ by \cite[Lemma~\tref{l:pencil-mult}]{10.th-panoramico}.
\begin{center}
\vspace{2mm}
\includegraphics[height=23mm]%original height 136,299
% reference height because widest picture
{para-asympt-gr.eps}
\captionof{figure}{Pencil with base locus the double asymptotic
  tangent $\Lambda$ at a parabolic point}
\end{center}

\noindent 
The point $\orth [\T_pS]$ lies on the cuspidal double curve of $\dual
S$. A general line through this point intersects $\dual S$ with
multiplicity $2$, a general line in the tangent cone of $\dual S$
with multiplicity $3$, and the tangent line of the cuspidal double
curve with multiplicity $4$. Hence  $\orth \Lambda$ is the latter
line. 

(d) Lastly, let $p$ be a point such that $C_0 = S \cap
\T_pS$ has a tacnode at $p$, and $\Lambda$ be the asymptotic tangent of
$S$ at $p$, which is also the support of the tangent cone of $C_0$ at
$p$. The base-point-free pencil is defined as in cases (b) and (c).
The computations now give
\begin{align*}
\epsilon_1^* C_0 &= C_0 + 2 E_1 \\
\epsilon_2^*\epsilon_1^* C_0 &= C_0 + 2 E_1 +4E_2 \\
\epsilon_3^* \epsilon_2^*\epsilon_1^* C_0 &= C_0 + 2 E_1 +4E_2 +4E_3
\end{align*}
so that
\[
\tilde C_0=
\epsilon^* C_0- E_1 - 2E_2 -3E_3
= C_0 + E_1 + 2E_2+E_3.
\]
This time the curve is not reduced. However this is not a reason for
the topological formula behind Lemma~\ref{l:pencil-13} to fail, and the
latter is still valid. The only caution is that the computation of
$e(\tilde C_0)$ is no longer liable to
\cite[Lemma~\tref{l:pencil-mult}]{10.th-panoramico}; we compute it directly as
the Euler number of $\tilde {C}_{0,\red}$, as indeed the topological
formula doesn't see multiplicities,
\ie $e(\tilde C_0) = e(\tilde {C}_{0,\red})$.
\begin{center}
\vspace{2mm}
\includegraphics[height=23mm]
% original height 136,406
% 23 * 136,406 / 136,299
{swal-asympt-gr.eps}
\captionof{figure}{Pencil with base locus the double asymptotic
  tangent $\Lambda$ at a swallowtail point}
\end{center}

Since the curve $C_0 \subset S$ has a tacnode, its proper transform in
$\tilde S$ has genus $g-2$, where $g$ stands for the genus of a
general member of $\orth \Lambda$.
It then follows from the additivity of the Euler number as in the
proof of \cite[Lemma~\tref{l:pencil-mult}]{10.th-panoramico}, that
\begin{align*}
e(C_0 + E_1 + E_2+E_3)
&=e(C_0) + e(E_1) + e(E_2)+e(E_3)-4
\\
&=\bigl(2-2(g-2)\bigr) + 2+2+2-4
= e(C_\gen)+6.
\end{align*}

One then argues as in case (c), remembering the local swallowtail
model of $\dual S$ at $\orth [\T_pS]$ given in \ref{p:swallowtail}.
The point $\orth [\T_pS]$ is triple for $\dual S$, and the only line
through this point intersecting $\dual S$ with multiplicity strictly
larger than $4$ is the common support of the respective tangent cones
of both double curves of $\dual S$ at $\orth [\T_pS]$.
\end{proof}


\subparagraph{Remark}
In the swallowtail model of \ref{p:swallowtail}, the support of the
tangent cones of the double curves of $\dual S$ is the line $b=c=0$,
which is downright contained in the discriminant hypersurface 
\eqref{eq:swallowtail}.
Of course it is not the case in general that, in the notation of (d),
the line $\orth \Lambda$ is contained $\dual S$.






\begin{references}

\setcounter{footnote}{0}
\renewcommand{\thefootnote}{\alph{footnote}}
\begin{thebibliography}[Chapters in this Volume\footnote
  {see \url{https://www.math.univ-toulouse.fr/~tdedieu/\#enumTV}}]{XIII}

\bibitem[II]{02.edoardo}
Th.~Dedieu and E.~Sernesi,
\emph{Deformations of curves on surfaces}.

\bibitem[XI]{10.th-panoramico}
Th.~Dedieu, \emph{Enumerative geometry of {$K3$} surfaces}.

\bibitem[C]{16.th+l-redres}%{chap-reddisc}
L.~Busé {\normalfont \smfandname} Th.~Dedieu, \emph{Generalized weight
  properties of resultants and discriminants, and applications to projective
  enumerative geometry}.

\bibitem[XIII]{14.th-vainsencher}
Th.~Dedieu,
\emph{Node polynomials for curves on surfaces}.

\end{thebibliography}


\begin{thebibliography}[External References]{99}

\bibitem{alexeev-engel}
V.~Alexeev {\normalfont \smfandname} P.~Engel, \emph{The flex divisor of a
  {{\(K3\)}} surface}, Int. Math. Res. Not. \textbf{2023} (2023), no.~10,
  8356--8370.

\bibitem{aluffi-involution}
P.~Aluffi, \emph{Projective duality and a {C}hern-{M}ather involution}, Trans.
  Amer. Math. Soc. \textbf{370} (2018), no.~3, 1803--1822.

\bibitem{aluffi-cukierman}
P.~Aluffi {\normalfont \smfandname} F.~Cukierman, \emph{Multiplicities of
  discriminants}, Manuscripta Math. \textbf{78} (1993), no.~3, 245--258.

\bibitem{acgh}
E.~Arbarello, M.~Cornalba, P.~A. Griffiths {\normalfont \smfandname} J.~Harris,
  \emph{Geometry of algebraic curves. {V}ol. {I}}, Grundlehren der
  Mathematischen Wissenschaften, vol.~267, Springer-Verlag, New York, 1985.

\bibitem{italEMS}
M.~Beltrametti, E.~Carletti, D.~Gallarati {\normalfont \smfandname} G.~{Monti
  Bragadin}, \emph{Lectures on curves, surfaces and projective varieties -- a
  classical view of algebraic geometry}, EMS Textbooks in Mathematics, European
Mathematical Society, 2009, Original version
(in italian) issued in 2003.

\bibitem{bruce}
J.~W. Bruce, \emph{The duals of generic hypersurfaces}, Math. Scand.
  \textbf{49} (1981), no.~1, 36--60.

\bibitem{BASW}
L.~Bus{\'e}, C.~D'Andrea, M.~Sombra {\normalfont \smfandname} M.~Weimann,
  \emph{The geometry of the flex locus of a hypersurface}, Pacific J. Math.
  \textbf{304} (2020), no.~2, 419--437.

\bibitem{ch-13}
L.~Caporaso {\normalfont \smfandname} J.~Harris, \emph{Counting plane curves of
  any genus}, Invent. Math. \textbf{131} (1998), no.~2, 345--392.

\bibitem{cayley-memoir}
A.~Cayley, \emph{Mémoire sur les courbes à double courbure et les surfaces
  développables}, Journal de mathématiques pures et appliquées 1re série
  \textbf{10} (1845), 245--250.

\bibitem{CF}
C.~Ciliberto {\normalfont \smfandname} F.~Flamini, \emph{On the branch curve of
  a general projection of a surface to a plane}, Trans. Amer. Math. Soc.
  \textbf{363} (2011), no.~7, 3457--3471.

\bibitem{corvaja-zucconi}
P.~Corvaja {\normalfont \smfandname} F.~Zucconi, \emph{The surface of gauss
  double points},
Eur. J. Math. \textbf{8} (2022), no. 3, 871--892.
%prepublication arXiv:2008.02012.

\bibitem{dimca}
A.~Dimca, \emph{Topics on real and complex singularities}, Advanced Lectures in
  Mathematics, Friedr. Vieweg \& Sohn, Braunschweig, 1987, An introduction.

\bibitem{dolgachev}
I.~V. Dolgachev, \emph{Classical algebraic geometry}, Cambridge University
  Press, Cambridge, 2012, A modern view.

\bibitem{edge}
W.~L. Edge, \emph{The theory of ruled surfaces}, Cambridge University Press,
  1931, \url{http://www.maths.ed.ac.uk/cheltsov/edge2013/read.html}.

\bibitem{enriques}
F.~{Enriques}, \emph{{Le superficie algebriche}}, {N.~Zanichelli, Bologna},
  1949.

\bibitem{fischer}
G.~Fischer, \emph{Plane algebraic curves}, Student Mathematical Library,
  vol.~15, American Mathematical Society, Providence, RI, 2001, Translated from
  the 1994 German original by Leslie Kay.

\bibitem{fischer-piontkowski}
G.~Fischer {\normalfont \smfandname} J.~Piontkowski, \emph{Ruled varieties},
  Advanced Lectures in Mathematics, Friedr. Vieweg \& Sohn, Braunschweig, 2001,
  An introduction to algebraic differential geometry.

\bibitem{teissier-afst}
A.~G. Flores {\normalfont \smfandname} B.~Teissier, \emph{Local polar varieties
  in the geometric study of singularities}, Ann. Fac. Sci. Toulouse Math. (6)
  \textbf{27} (2018), no.~4, 679--775.

\bibitem{GKZ}
I.~M. Gelfand, M.~M. Kapranov {\normalfont \smfandname} A.~V. Zelevinsky,
  \emph{Discriminants, resultants and multidimensional determinants}, Modern
  Birkh\"auser Classics, Birkh\"auser Boston, Inc., Boston, MA, 2008, Reprint
  of the 1994 edition.

\bibitem{gruson-peskine}
L.~Gruson {\normalfont \smfandname} C.~Peskine, \emph{On the smooth locus of
  aligned {H}ilbert schemes, the {$k$}-secant lemma and the general projection
  theorem}, Duke Math. J. \textbf{162} (2013), no.~3, 553--578.

\bibitem{harris-13}
J.~Harris, \emph{Algebraic geometry}, Graduate Texts in Mathematics, vol.~133,
  Springer-Verlag, New York, 1995, A first course.

\bibitem{hartshorne-13}
R.~Hartshorne, \emph{Algebraic geometry}, Springer-Verlag, New York-Heidelberg,
  1977, Graduate Texts in Mathematics, No.~52.

\bibitem{anschau}
D.~{Hilbert} {\normalfont \smfandname} S.~{Cohn-Vossen}, \emph{{Anschauliche
  Geometrie.}}, vol.~37, Springer, Berlin, 1932, engl.\ transl.\ available as
  {``}Geometry and the Imagination{''}.

\bibitem{iversen}
B.~Iversen, \emph{Numerical invariants and multiple planes}, Amer. J. Math.
  \textbf{92} (1970), 968--996.

\bibitem{katz}
N.~M. Katz, \emph{Pinceaux de Lefschetz: théorèmes d'existence}, SGA 7 II,
  Exposé XVII.

\bibitem{kleiman-aarhus}
S.~L. Kleiman, \emph{Concerning the dual variety}, in \emph{18th {S}candinavian
  {C}ongress of {M}athematicians ({A}arhus, 1980)}, Progr. Math., vol.~11,
  Birkh\"auser, Boston, MA, 1981, 386--396.

\bibitem{kollar-flecnodal}
J.~Koll{\'a}r, \emph{Szemer{\'e}di-{T}rotter-type theorems in dimension 3},
  Adv. Math. \textbf{271} (2015), 30--61.

\bibitem{kulikov-calculus}
Val.~S. Kulikov, \emph{Calculus of singularities of imbedding of a general
  algebraic surface in the projective space {${\bf P}\sp{3}$}}, Funktsional.
  Anal. i Prilozhen. \textbf{17} (1983), no.~3, 15--27.

\bibitem{kulikov-focal}
\bysame , \emph{The number of singular focal centers of projection of an
  algebraic surface}, Uspekhi Mat. Nauk \textbf{39} (1984), no.~5(239),
  245--246.

\bibitem{kulikov-kulikov}
Val.~S. Kulikov {\normalfont \smfandname} Vik.~S. Kulikov, \emph{Generic coverings
  of the plane with {$A$}-{$D$}-{$E$}-singularities}, Izv. Ross. Akad. Nauk
  Ser. Mat. \textbf{64} (2000), no.~6, 65--106.

\bibitem{kulikov-afst}
Vik.~S. Kulikov, \emph{A remark on classical {P}luecker's formulae}, Ann. Fac.
  Sci. Toulouse Math. (6) \textbf{25} (2016), no.~5, 959--967.

\bibitem{kulikov-shustin}
Vik.~S. Kulikov {\normalfont \smfandname} E.~Shustin, \emph{Duality of planar and
  spacial curves: new insight}, Eur. J. Math. \textbf{1} (2015), no.~3,
  462--482.

\bibitem{laumon}
G.~Laumon, \emph{Degr\'e{} de la vari\'et\'e{} duale d'une hypersurface \`a{}
  singularit\'es isol\'ees}, Bull. Soc. Math. France \textbf{104} (1976),
  no.~1, 51--63.

\bibitem{mccrory-shifrin}
C.~McCrory {\normalfont \smfandname} T.~Shifrin, \emph{Cusps of the projective
  {G}auss map}, J. Differential Geom. \textbf{19} (1984), no.~1, 257--276.

\bibitem{parunsinski}
A.~Parusi\'nski, \emph{Multiplicity of the dual variety}, Bull. London Math.
  Soc. \textbf{23} (1991), no.~5, 429--436.

\bibitem{piene-duality}
R.~Piene, \emph{Numerical characters of a curve in projective {$n$}-space}, in
  \emph{Real and complex singularities ({P}roc. {N}inth {N}ordic {S}ummer
  {S}chool/{NAVF} {S}ympos. {M}ath., {O}slo, 1976)}, 1977, 475--495.

\bibitem{piene-polars}
\bysame , \emph{Polar classes of singular varieties}, Ann. Sci. \'Ecole Norm.
  Sup. (4) \textbf{11} (1978), no.~2, 247--276.

\bibitem{piene-someformulas}
\bysame , \emph{Some formulas for a surface in {${\bf P}^{3}$}}, in
  \emph{Algebraic geometry ({P}roc. {S}ympos., {U}niv. {T}roms\o , {T}roms\o ,
  1977)}, Lecture Notes in Math., vol.~687, Springer, Berlin, 1978, 196--235.

\bibitem{piene-noether}
\bysame , \emph{A proof of {N}oether's formula for the arithmetic genus of an
  algebraic surface}, Compositio Math. \textbf{38} (1979), no.~1, 113--119.

\bibitem{piene-higherorder}
\bysame , \emph{A note on higher order dual varieties, with an application to
  scrolls}, in \emph{Singularities, {P}art 2 ({A}rcata, {C}alif., 1981)}, Proc.
  Sympos. Pure Math., vol.~40, Amer. Math. Soc., Providence, RI, 1983,
  335--342.

\bibitem{pohl}
W.~F. Pohl, \emph{Differential geometry of higher order}, Topology \textbf{1}
  (1962), 169--211.

\bibitem{ronga-13}
F.~Ronga, \emph{On the number of planes triply tangent to a surface in
  projective space}, in \emph{Proceedings of the 1984 {V}ancouver conference in
  algebraic geometry}, CMS Conf. Proc., vol.~6, Amer. Math. Soc., Providence,
  RI, 1986, 389--395.

\bibitem{ronga-transversality}
\bysame , \emph{On the singularities of the surface reciprocal to a generic
  surface in projective space}, J. Differ. Geom. \textbf{29} (1989), no.~1,
  105--112.

\bibitem{russo}
F.~Russo, \emph{On the geometry of some special projective varieties}, Lecture
  Notes of the Unione Matematica Italiana, vol.~18, Springer, Cham; Unione
  Matematica Italiana, Bologna, 2016.

\bibitem{salmon2}
G.~Salmon, \emph{{A Treatise on the Analytic Geometry of Three Dimensions,
  Vol.~II}}, Chelsea Publishing Company, New York, 1965, reprint of the fifth
  (latest) edition.

\bibitem{samuel}
P.~Samuel, \emph{G\'eom\'etrie projective}, Presses Universitaires de France,
  Paris, 1986, English translation available.

\bibitem{bsegre-bertiniforms}
B.~Segre, \emph{Bertini forms and {H}essian matrices}, J. London Math. Soc.
  \textbf{26} (1951), 164--176.

\bibitem{teissier-simultanee}
B.~Teissier, \emph{R{\'e}solution simultan{\'e}e {II}}, in \emph{S{\'e}minaire
  sur les singularit{\'e}s des surfaces}, Lect. Notes Math., vol.~777,
  Springer, 1980, 82--146.

\bibitem{tevelev}
E.~A. Tevelev, \emph{Projective duality and homogeneous spaces}, Encyclopaedia
  of Mathematical Sciences, vol.~133, Springer-Verlag, Berlin, 2005, Invariant
  Theory and Algebraic Transformation Groups, IV.

\bibitem{urabe-duality}
T.~Urabe, \emph{Duality of numerical characters of polar loci}, Publ. Res.
  Inst. Math. Sci. \textbf{17} (1981), 331--345.

\bibitem{urabe-pluecker}
\bysame , \emph{Generalized {Pluecker} formulae}, Publ. Res. Inst. Math. Sci.
  \textbf{17} (1981), 347--362.

\bibitem{claire}
C.~Voisin, \emph{Théorie de Hodge et géométrie algébrique complexe}, Cours
  spécialisés, vol.~10, Société Mathématique de France, 2002, English
  translation available.

\bibitem{witaszek}
J.~Witaszek, \emph{The geometry of smooth quartics}, MSc thesis Universit{\"a}t
  Bonn, 2014.

\bibitem{XuGeng}
Geng Xu, \emph{Subvarieties of general hypersurfaces in projective space}, J.
  Differential Geom. \textbf{39} (1994), no.~1, 139--172.

\bibitem{zariski-mumford}
O.~Zariski, \emph{Algebraic surfaces}, Classics in Mathematics,
  Springer-Verlag, Berlin, 1995, With appendices by S. S. Abhyankar, J. Lipman
  and D. Mumford, Preface to the appendices by Mumford, Reprint of the second
  (1971) edition.

\end{thebibliography}

% \bibliographystyle{mysmf-alpha}
% \bibliography{classic}

\end{references}




\stopcontents[13.th-classic]





%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main.tex"
%%% coding: utf-8
%%% End: 

